New Lower and Upper Bounds for the Grothendieck Constant

We establish new bounds on the Grothendieck constant $K_G$: \[ \frac{6\pi}{11} \le K_G \le \frac{\pi}{2\log(1+\sqrt2)} - 10^{-4}. \] Methodologically, our lower bound approach differs from previous works by establishing limitations on the asymptotically optimal Krivine schemes, rather than giving explicit constructions of gap instances. Our upper bound is obtained by proposing and analyzing the first asymptotic construction of rounding schemes, whereas previous works only consider low-dimensional schemes. Together, these bounds determine the previously unknown tenths digit of $K_G$ to be $7$. The bounds were discovered by a long-running collaborative effort of humans and a long-horizon AI research system that we engineered.

==> old/ai_section.tex <==
% ============================================================================
% AI SECTION -- draft to be merged into the main paper as a single section.
% No abstract and no title: the \section below is the section itself.
% Style: anton_style.md. Items needing author confirmation are marked %% TODO.
% ============================================================================


\hypersetup{
  colorlinks=true,
  linkcolor=blue!55!black,
  urlcolor=blue!55!black,
  citecolor=blue!55!black
}

\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}
\setlist[itemize]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}
\setlist[enumerate]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}

\section{AI methodology and analysis}
\label{sec:ai}

{\color{red}AX: Overall, the opening before Subsection 11.1 is too long. It suffices to just have 1-2 paragraphs at most.}

The results in this paper were obtained in collaboration with an autonomous
AI research system. The cubic--quintic
construction and its certificate (Theorem~\ref{thm:cubic-quintic-upper-bound})
predate the current system and was found through conversation with GPT-5.5-Pro. The lower bound $\KG\ge6\pi/11$ was
discovered and first proved by the system; we have since verified the
argument ourselves, and the proof in this paper is our revision of the
system's write-up. The system also produced further improvements on both
sides of the problem, which we report in Section~\ref{sec:ai-results} but do
not state as theorems, because their certificates have not yet been human-verified. This section documents the methodology
(Section~\ref{sec:ai-methodology}), quantifies the run and its outcomes
(Section~\ref{sec:ai-results}), reconstructs how the lower bound was found
(Section~\ref{sec:ai-case-study}), and discusses what the record shows about
the strengths and weaknesses of current AI systems as mathematical
collaborators (Sections~\ref{sec:ai-discussion} and~\ref{sec:ai-future}).
{\color{red}AX: The discussion of cut-off dates belongs in some split of the methodology/discussions.
If you had to keep one paragraph, it would be this.
}


Recent successes of AI in mathematics, including on open problems, are of
a different kind from the work reported here. Evaluator-guided search has
produced record constructions~\cite{funsearch,novikov2025alphaevolvecodingagentscientific, charton2024patternboostconstructionsmathematicslittle},
and formal provers have shown proficiency at solving olympiad-level problems \cite{novikov2025alphaevolvecodingagentscientific}. In the
months surrounding our run, frontier models went further: an internal reasoning
model at OpenAI has disproved the Erd\H{o}s unit-distance conjecture
\cite{openai2026planarpointsets}, a mathematician has found a counterexample to the Jacobian conjecture using Claude Fable 5
\cite{jacobian}, and OpenAI has announced solutions, with formally
checked proofs, to ten open problems in mathematics and theoretical
computer science \cite{openai2026ten}. Most of these results involved resolving a single well-posed statement by construction. Moreover, none explicitly required significant long horizon reasoning. Finally, all of the recent results with frontier models were found fully autonomously, without sustained human intervention.
{\color{red}AX: Move to discussion. Also I'm not a fan of the ``in the months surrounding our run'' --- I think it's too fancy here. Let's just make this more standard ``recent and concurrent work'' that's happened to us.}

Our work is a more realistic example of how humans and AI can collaborate on mathematical research. The problem is more open ended, requiring a research program where over the course of weeks intermediate results accumulate and directions are opened and abandoned. Moreover, humans were consistently steering the system and providing feedback. We hope that our experiences outlined in this section will be useful to future mathematicians and AI researchers alike.
{\color{red}AX: Also move to discussion. It's also risky to explicitly claim that this is a ``more realistic example'', it could be more like: ``Our work is an extensive case-study ...'' or something like that?}



\subsection{Methodology}
\label{sec:ai-methodology}

{\color{red}AX: This is too dense. Tell Fable to explicitly split into the following paragraph groups: (1) AI models and compute: here you describe what models you used and you can also remark on the cut-off dates so that future readers have context. You can also add 1-2 sentences describing the server setup that you used.
(2) Harness: you can describe the harness system here.
(3) Run configurations
(4) Human interaction.
}

{\color{red}AX: Continuing from above: the current structure is kind of this split. It's more or less slapping on an explicit paragraph tag. However, the writing should be tightened to focus more on its assigned topic.}


The system uses a harness that couples two frontier language
models in distinct roles. A reasoning model (OpenAI GPT-5.5-Pro at maximal
reasoning effort, later GPT-5.6-Sol) serves as the brain, where it selects
directions, develops arguments, specifies experiments, and audits the
resulting claims. A coding agent (Anthropic Claude Code, running Claude Opus
and later Claude Fable~5) serves as the executor, where it maintains the project
repository, implements and runs experiments, retrieves literature, and
drives the reasoning model through a scripted interface. The harness was also adjusted repeatedly over the
run in response to observed failures. We describe its final form, to the
extent needed to interpret the record.


Work is organized into \emph{sessions} of a few hours, of which two to
five run concurrently on mutually distinct directions. No model context survives from
one session to the next, and instead continuity is carried by a single summary file that serves as
working memory and into which finished work is merged, and append-only
transcripts and experiment logs. A session passes through fixed phases:
orientation from the problem statement and summary files, selection of a focus, a research loop in
which the reasoning model requests computations, literature, or further
reasoning time, and a closing audit that produces a calibrated summary in
which every claim is tagged as proven, numerically supported, conjectural,
or heuristic. We reserve the word theorem, here and in the rest
of the paper, for statements that we have additionally checked ourselves.

The run started from a substantial base of our prior work rather than from
the problem alone. By June 2026 we had worked on the constant for several
months, and the harness was initialized with the results: the cubic--quintic scheme, the coefficient formulas and certification machinery, our accumulated notes, and a
problem statement listing candidate directions for both bounds. In
particular, the search space the run explored is a generalization of teh cubic--quintic scheme, and the possibility of converting
obstructions into lower bounds was raised, as a suggestion, in the problem
statement. The system therefore operated downstream of the mathematical
framework it was given, a point quantified in
Section~\ref{sec:ai-case-study}.

A human operator (one of the authors) steered the run asynchronously through
text files read at the start of, and during, every session. Steering
consisted of priorities, targets, audits of the run's own claims, and
occasional mathematical pointers; about forty dated directives were issued
over the run. The operator contributed no proof steps through this channel.

\subsection{Results}
\label{sec:ai-results}

The run spanned June~16 to July~24, 2026, It comprised
roughly 240 research sessions. The reasoning model was called 2{,}091
times, consuming about 152 million tokens at an estimated \$5{,}400 in
API cost; the coding agent ran on a flat-rate subscription (Claude Max). Floating-point searches ran
on a four-GPU node, and every certified computation was redone in interval
arithmetic on CPU. Table~\ref{tab:run} collects these figures, and
Table~\ref{tab:timeline} gives the timeline of the bounds.

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}ll@{}}
\toprule
Duration & June 16 -- July 24, 2026 (main phase through July 4)\\
Research sessions & $\approx240$\\
Reasoning model & GPT-5.5-Pro, later GPT-5.6-Sol; maximal effort\\
Usage and cost & 2{,}091 calls; $\approx152$M tokens; $\approx\$5{,}400$\\
Coding agent & Claude Code (Opus, later Fable 5); subscription\\
Human steering & one operator; $\approx40$ dated directives\\
\bottomrule
\end{tabular}
\caption{\textbf{The run at a glance.} Aggregates computed from the harness
telemetry. Dollar figures are list-price estimates; coding-agent usage was
only partially metered.
}
\label{tab:run}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lp{0.76\textwidth}@{}}
\toprule
Sessions & Event\\
\midrule
1 & run begins from the interval $1.6769566742\le\KG\le1.7818666070$
(the upper end is the cubic--quintic bound of this paper)\\
18 & upper-bound search plateaus; the operator directs a pivot to the
lower bound\\
44 & numerical upper bound $1.7802243$ recorded (later withdrawn)\\
55--57 & affine reframe; $\KG\ge6\pi/11$ derived\\
58--64 & $6\pi/11$ proof machine-audited; first \LaTeX{} write-up\\
p92, p117 & lower bounds $27\pi/49\approx1.7311$ and
$51\pi/92\approx1.7415$ machine-verified\\
follow-up & the session-44 value found unsupported by internal audit and
withdrawn\\
follow-up & upper bound $1.781801841033$ machine-certified\\
follow-up & upper bound $1.7813319810625639$ machine-certified;
adversarial review passed\\
\bottomrule
\end{tabular}
\caption{\textbf{Timeline of the bounds produced during the run.}
Machine-verified means accepted by the verification protocol of
Section~\ref{sec:ai-methodology}. The last three events fall in the short
follow-up phases, whose sessions we do not cite individually. Of the
run's results, only $\KG\ge6\pi/11$ has additionally been verified by the
authors; it is the result stated as a theorem in this paper.}
\label{tab:timeline}
\end{table}

The run's principal outcome, and the one this paper states as a theorem,
is the lower bound $\KG\ge6\pi/11$, whose discovery
Section~\ref{sec:ai-case-study} reconstructs. Beyond it, the run produced
machine-certified upper bounds of $1.781801841033$ and then
$1.7813319810625639$, improving on the cubic--quintic value, together with
the two stronger lower bounds listed in Table~\ref{tab:timeline}. We
report these as machine-verified claims rather than theorems: each passed
the full internal protocol, but we have not yet verified their
certificates ourselves.
%% TODO: reconcile with the main paper's discussion of concurrent work
%% (e.g. Heilman's computer-assisted improvement of Krivine's bound,
%% arXiv:2606.00247).

\subsection{Case study: the lower bound}
\label{sec:ai-case-study}

The lower bound is the run's main discovery. We reconstruct it here in
outline, highlighting the three human interventions that shaped it, since
the weaknesses discussed in Section~\ref{sec:ai-discussion} refer back to
them; the full logs of the sessions involved will be released with the rest
of the record.
{\color{red}AX: You don't have to refer to to-be-released artifacts here.
Tell Fable to write this version as though we're *not* releasing additional artifacts.
If and when we release artifacts, we'll strategically insert a few footnotes where needed.
}

{\color{red}AX: As currently written, I think the current section will be hard to track for anyone *not* intimately involved in the paper.
Granted, this is hard because it is about exploring a lot of concepts ...
Is it possible to extract a general/high-level for a proof template/sketch/idea so that we can ``set the scene'' + provide context?
\\
Additionally, I think you could consider adding a brief ``Overview`` paragraph of sorts that someone *not* working on Grothendieck can easily skim and get the big picture. This could be a high-level summarization of the subsequent ``The plateau``, ``First intervention'', etc. paragraphs.
}

\paragraph{The plateau.}
The run began on the upper bound, searching the limiting-scheme space of our
preprint for schemes whose correlation function admits a large
inverse-majorant parameter $\gamma$, since an admissible $\gamma$ gives
$\KG\le\pi/(2\gamma)$. From the hyperplane value
$\gamma=\log(1+\sqrt2)\approx0.8814$ it reached $\gamma\approx0.882$, and
there it stalled: in sessions 12 through 17 it opened six {\color{red}mechanically
distinct escape routes}, and each failed against the same obstruction,
namely that cubic coefficient mass cannot be cancelled without also reducing
the linear coefficient. Each failure was recorded and tagged, and the run's
response was to begin a seventh variation of the same search.

\paragraph{First intervention: turn the failures into a theorem.}
The operator redirected the run in session 18. Instead of attempting another
escape, it was to synthesize the accumulated failures into a proof that no
scheme in the class does much better: a ceiling $\gamma\le\Gamma$ valid for
the full class, with mixtures and arbitrary dimension, converts through the
optimality theorem of Naor and Regev \cite{naor2014krivine} into the lower
bound $\KG\ge\pi/(2\Gamma)$. The intervention supplied no new mathematics:
the problem statement had suggested this dualization from the outset, and
the run had accumulated exactly the required evidence without making the
connection. Session 18 identified the Naor--Regev theorem as the correct
transfer, proved a first ingredient valid in every dimension, and located
the difficulty precisely: the ceilings it could prove covered too narrow a
class of schemes.

\paragraph{Progress in two dimensions.}
Within days the run had proved a cubic ceiling of strength
$\Gamma\approx0.8866$ for two-dimensional schemes, with the {\color{red}keystone (?)}
inequality certified in interval arithmetic, and had sharpened the
constant numerically to $\Gamma\approx0.8846$. The extension to arbitrary dimension and to mixtures, which the
duality requires, did not follow: fourteen sessions in the range 32--51
attacked it, each reducing the gap to a sub-lemma, proving the sub-lemma in
a restricted setting, and leaving the global assembly open, while the
restricted results accumulated in memory as apparent progress. Two useful
facts emerged alongside this loop: the run verified the normalization of the
Naor--Regev transfer against the original paper, and it computed that
improving the Davie--Reeds~\cite{Davie1984LowerBoundKG,Reeds1991LowerBoundKG} bound $1.6769566742$ requires a universal ceiling
only at $\Gamma\le0.93669$, far above the two-dimensional value, so a
general ceiling could be far from sharp and still give a new lower bound.

\paragraph{Second intervention: the general bound, through theory.}
The operator ended this loop with a second redirection, on two grounds:
refinements of the two-dimensional result were not the object of interest,
since only a ceiling for the full class dualizes; and the gap was
conceptual, so further implementation would not close it. The run was to
spend several sessions on theory alone. Session 55 mapped the dependency
structure of the preceding weeks and identified the recurring error,
restricted closures recorded as global progress. Session 56 then produced
the {\color{red}decisive (?)} reframe. Every failed transport had been nonlinear in
quantities that do not average when schemes are mixed; the Hermite
coefficients $(b_1,b_3)$ of the correlation function, by contrast, are
linear functionals of the scheme, so a constraint that is affine in
$(b_1,b_3)$ passes to mixtures and to coefficientwise limits with no further
argument. Choosing the constraint for transportability, and requiring
equality at the extremal hyperplane point $(b_1,b_3)=(1,\tfrac16)$, gives
the one-parameter family of affine constraints
\[
        b_3\;\ge\;(1+\lambda)\,b_1-\Bigl(\lambda+\tfrac56\Bigr),
        \qquad \lambda\ge\tfrac12 ,
\]
where $\lambda$ indexes the slope of the line through the hyperplane point.
Each member forces a barrier $\Gamma_\lambda=(\lambda+\frac56)/(1+\lambda)$
on the admissible parameter, hence a bound $\KG\ge\pi/(2\Gamma_\lambda)$
conditional on proving that member, and every $\Gamma_\lambda$ below
$0.93669$ improves on Davie--Reeds.

\paragraph{Third intervention: one certified {\color{red}rung} before a better one.}
The tangent member $\lambda=\tfrac12$, worth $\KG\ge9\pi/16\approx1.767$,
requires a sharp chaos inequality that remains open, and once the family
existed the run's inclination was to work toward its strongest provable
member. The operator set the priority differently: what mattered was to
establish that the method yields any new lower bound at all, so the run was
to select a rung whose proof closes, certify it completely, and write it up,
with improvements inside the family treated as secondary. At $\lambda=1$ the
proof collapses to elementary structure: session 57 found that the
decomposition $h=(f+g)/2$, $k=(f-g)/2$ reduces the constraint, fiber by
one-dimensional fiber, to the ternary inequality~\eqref{eq:fiber-inequality},
%% TODO: fix cross-reference to the fiber inequality of the lower-bound section
whose closing case analysis is short, giving $\Gamma_1=\tfrac{11}{12}$ and
\[
        \KG\;\ge\;\frac{6\pi}{11}\;\approx\;1.7136 .
\]
Sessions 58--64 then subjected the chain to adversarial review, which
found and repaired the one substantive gap (the passage from finitely many
schemes to measurable mixtures, closed by a weak-$*$ lemma), a Jensen
inequality applied in the wrong direction, and a small defect in the
interval certificate's coverage, after which the run produced the first
complete write-up, about a day after the reframe. The stronger rungs
$27\pi/49$ and $51\pi/92$ of Table~\ref{tab:timeline} followed within a week
by the same method at smaller values of $\lambda$.



\paragraph{Attribution.}
The operator contributed no proof step anywhere in the chain. The operator's
contributions were the starting context of
Section~\ref{sec:ai-methodology} and the three interventions above, each a
redirection of effort rather than a piece of mathematics. The system
contributed the mathematics: the identification and verification of the
transfer theorem, the headroom computation, the two-dimensional ceiling, the
observation that affine constraints survive mixing, the family of lines, the
fiber reduction, the closure lemma, the certificates, and the initial
write-up. One further observation matters for what follows: nothing in the
session-56 reframe depended on information unavailable at the pivot a week
earlier, since the affineness of coefficients under mixing is elementary and
the headroom computation is one line. The binding constraint appears to have
been the system's disposition to continue its current program, not a missing
capability.
{\color{red} Name this something like ``human involvement'' or somehting along those lines. Also move the operator contributions first, and describe why they were necessary. Only then do you state the AI involvement.}


\subsection{Discussion}
\label{sec:ai-discussion}

The record supports a consistent capability profile: strong technical
execution, with persistent failures in the judgement that directs it. We
summarize the strengths, then the weaknesses, stated in the terms that the
interventions of Section~\ref{sec:ai-case-study} make concrete, and close
with what the record shows about the division of labor.

\subsubsection{Strengths}

Three strengths carried the run. The first is technical range with effective
recall: given a one-word pointer to Naor's work, the system identified the
relevant theorem, verified its normalization against the paper, and computed
the slack available for a lossy transfer; given a plateau, it produced six
structurally distinct escape mechanisms in two days. The second is local
invention: the affine family, the fiber reduction, the closure lemma, and
the certificate architecture were machine products, several arriving within
hours once the question was well posed. The third is speed and reliability
of execution: from the reframe to a machine-audited, interval-certified
proof took about a day, and most individual technical errors were caught by
the system's own verification passes. In one representative episode
(sessions p44 and p49), a claimed bound of $\KG\ge1.7754518$
was refuted within five hours by an adversarial session that computed its
true margin to be approximately $-8\times10^{-8}$, and the record was
corrected to the defensible value.

\subsubsection{Weaknesses}

Each intervention of Section~\ref{sec:ai-case-study} was needed because a
specific capability was absent. The paragraphs below name these
capabilities and add further instances from the record.

{\color{red}
AX: Name these paragraphs more explicitly to reflect a negative,
e.g., "Poor judgment of what is interesting", "Lack of high-level research skills", etc.}

\paragraph{Judgement of interestingness.}
The system did not reliably rank work by mathematical interest. The second
and third interventions are the clearest cases: the run treated refinements
of the two-dimensional ceiling as progress when only the general bound
mattered, and, once the family of rungs existed, it valued improvements
within the family over establishing the first certified rung. The same
tendency appeared at smaller scales throughout, from sessions spent on
$10^{-5}$-sized improvements to mechanisms the run already understood, down
to reported values tuned to the edges of their enclosures. The implication
for collaboration is that the objective of the research cannot yet be
delegated. The operator's judgements of interest were few, but each
redirected weeks of machine effort, and between them the system optimized,
competently, whatever was in front of it. On a problem of this size the
space of possible intermediate constructions is unbounded, and a ranking by
expected interest is what makes the search tractable; supplying that
ranking was the human's principal ongoing contribution.

\paragraph{Research skills.}
The system managed individual arguments well and the research process
poorly: it did not decide when to persist, when to switch, or what a
sequence of failures implied. The first intervention is the sharpest case,
since the dualization of failures into a lower bound was suggested in the
problem statement the system re-read at every session, the six failures
were in its memory, and the step was taken only when ordered. The record
contains three further episodes of the same shape, of fourteen, roughly two
dozen, and about a dozen sessions respectively (the two-dimensional
extension, near-sharp variants of the lower bound, and the July
certification effort), in each of which the run circled a target without
progress until the operator ended the loop. The implication is that
autonomous running time does not by itself convert into progress. Once the
accessible directions were exhausted, additional sessions multiplied
execution, not judgement, and the run's rate of real progress was set by
the frequency of strategic correction; additional compute would not have
changed it. Oversight of such systems is accordingly most valuable at the
level of strategy, which is precisely the level at which the system did not
correct itself.

\paragraph{Memory.}
The harness's file-based memory preserved statements more reliably than
their qualifications. The withdrawn upper bound of Table~\ref{tab:timeline}
is the clearest case. In session 44 the run recorded a numerical upper
bound of $1.7802243$, with caveats attached; over the nineteen days the
value stood in working memory, re-summarization detached the caveats from
the headline number, and a note defending the value was written three days
before the internal audit that refuted it, finding the score inflated by a
finite truncation window and the underlying correlation profile
infeasible. A related failure occurred inside verification, where a
dedicated replay of the $51\pi/92$ certificate (session p95) passed it
because the replay inherited the framing of the argument it was checking;
the invalidating error was found the same day by a session that rebuilt the
argument from scratch (session p102). We attribute both failures to scale.
The run produced hundreds of sessions and tens of millions of tokens of
intermediate mathematics, and each new session could be shown only a small
distillate of it. What to retain, at what resolution, and with which
qualifications attached was itself decided by the models, through repeated
summarization, and repeated summarization is exactly where caveats detach
and inherited framings go unquestioned. Unlike the previous two weaknesses,
this one looks amenable to engineering: memory for such systems plausibly
needs more structure than prose summaries provide, for instance a graph of
claims carrying provenance and qualifications, so that important
information remains retrievable without being repeatedly re-serialized
through a model's context window.

\paragraph{Origins of the weaknesses.}
We believe these gaps have a common origin in how current systems are
produced. Models are trained and evaluated on problems selected for being
small enough to pose, sandbox, and score, and nothing in that regime
exercises the allocation of weeks of effort across an open-ended search.
The corpus they learn mathematics from is, moreover, made of finished
mathematics: the literature records definitions, theorems, and polished
proofs, while the process that produced them, the dead ends, the decisions
to abandon or reframe, the judgement of what was worth attempting, is
largely absent from the written record. A system trained this way can be
expected to acquire technique and the form of finished mathematics while
remaining weak at exactly the process skills described above, and that is
what we observe.

\subsubsection{Division of labor}

{\color{red}Name this subsection like human operator involvement or something, to emphasize the human involvement first.}

A useful summary of the collaboration is obtained by counting who caught
which errors. Errors in individual claims, such as wrong constants, broken
certificates, and invalid steps, were caught almost entirely by the system
itself. Failure patterns spanning many sessions, such as the three circling
episodes and the detachment of caveats from claims, were caught by the
operator in every recorded instance and by the system in none. The system
reliably falsifies a claim once the claim is specified; deciding which
claims to distrust remained a human function throughout. Consistent with
this, the operator's leverage came less from mathematical suggestions, most
of which the system correctly tested and discarded, than from calibration:
setting targets, ending loops, and auditing the run's own reporting. We also
note a regularity with design consequences: every overclaiming incident in
the record sits at a target with nearly zero margin, whereas the results
that survived verification all carry slack. This suggests that systems of
this kind are most productive when aimed at robust targets, with sharp
constants attempted only from a secured base.

\subsection{Future directions}
\label{sec:ai-future}

\paragraph{Mathematics.}
The immediate items are the machine-verified claims of
Table~\ref{tab:timeline}: human verification of the two certified upper
bounds and of the lower bounds $27\pi/49$ and $51\pi/92$ would upgrade each
to a theorem. Beyond them, the run's internal analysis identifies the
tangent case $\lambda=\tfrac12$ of the affine family, equivalent to a sharp
degree-three chaos inequality, as the natural boundary of the method and
worth $\KG\ge9\pi/16$ if resolved.
{\color{red}AX: If you're brave, conjecture that \(K_G = \sqrt{\pi}\)}

\paragraph{Toward AI systems for long-horizon research.}
If the diagnosis of Section~\ref{sec:ai-discussion} is right, the
requirements for progress follow from it. First, mathematical
interestingness needs to become an object of study in its own right: the
judgement that selects which questions, intermediate constructions, and
targets are worth pursuing was the most consequential input the human
supplied, and there is at present no training signal or benchmark that
rewards it. Second, the process of research mathematics needs data. What
mathematicians actually do between problem statement and finished paper,
how they allocate effort, learn from repeated failure, and decide to
reframe, is barely recorded anywhere; records of long runs such as ours,
which preserve every step including the unsuccessful ones, are one way to
begin creating such data, and we release ours in that spirit. Third,
evaluation must move to horizons where these capabilities matter, treating
a weeks-long research program rather than a single problem as the unit of
assessment, with memory and calibration measured alongside correctness.
These conclusions carry the usual caution that they derive from one run on
one problem; replications on other open problems, successful or not, would
be the most useful follow-up work.

\paragraph{Human--AI collaboration.}
The run also suggests where collaboration of this kind is heading. Within
it, the contributions that required a human were not technical: the system
supplied the arguments, the computations, the certificates, and the first
write-up, while the human supplied the problem, the taste, and the
strategic corrections. If the technical abilities of these systems continue
to improve, this division will sharpen, and the mathematician's role in
such collaborations will concentrate into choosing what to work on, judging
which objects and targets matter, and deciding what to trust: directing
research that one does not personally execute. A similar shift is already
under way in software engineering. We expect working modes of this kind to
become common in mathematics, and the run documented here, with its
weaknesses as much as its results, is an early picture of what they will
require of the mathematician.

\subsection*{Statement on AI use}
{\color{red}AX: Any specific reason for an entire subsection instead of just a paragraph?}

Large language models were used extensively in the research reported in
this paper, in the roles described in this section: GPT-5.5-Pro and
GPT-5.6-Sol (OpenAI) as the reasoning model, and Claude Opus and Claude
Fable~5 (Anthropic) as the coding agent. AI assistance was also used in
preparing parts of this manuscript. All results stated as theorems have been
verified by the authors independently of these systems, and the account of
the run given in this section reflects the authors' own reading of the
record. The authors take full responsibility for the contents of this
paper.



==> old/asymptotic_scheme_old.tex <==
\section{The Asymptotic Family}
\label{sec:scheme}

This section implements Section~\ref{sec:scheme} of the proof architecture.  There is one minor change in convention from this section onwards to keep in mind: any partition $F$ defined below corresponds to the partition $x\mapsto F(\sqrt2 x)$ in Definition~\ref{def:gaussian-correlation-function}.  This change of variables is harmless and keeps the Hermite covariance identity in its usual probabilist normalization.

\subsection{Hermite notation}

\begin{definition}[Orthonormal probabilist Hermite polynomials]\label{def:Hermite}
Let $(\He_n)_{n\ge0}$ denote the orthonormal probabilist Hermite polynomials.  Thus, for $Z\sim N(0,1)$,
\[
  \E[\He_m(Z)\He_n(Z)]=\delta_{mn}.
\]
In particular,
\[
  \He_0=1,
  \qquad \He_1(x)=x,
  \qquad \He_3(x)={x^3-3x\over\sqrt6},
  \qquad \He_5(x)={x^5-10x^3+15x\over\sqrt{120}}.
\]
If $(X,Y)$ are standard Gaussians with correlation $t$, then
\begin{equation}\label{eq:hermite-cov}
  \E[\He_m(X)\He_n(Y)]=\delta_{mn}t^n.
\end{equation}
We use this as our normalization throughout the coefficient computation.  Standard references for these identities include~\cite[Sec.~6.1]{AAR99}.
\end{definition}

\begin{definition}[Gaussianized Hermite-chaos average]\label{def:gaussianized-chaos}
Fix an odd integer $d\ge3$.  A length-$N$ \emph{Gaussianized degree-$d$ Hermite-chaos average} is the random variable
\[
  P_{d,N}=N^{-1/2}\sum_{j=1}^N \He_d(U_{d,j}),
\]
where the $U_{d,j}$ are independent standard Gaussians.  The word ``Gaussianized'' refers to the fact that, for fixed $d$, the variable $P_{d,N}$ converges in distribution to a Gaussian as $N\to\infty$, while paired copies retain the covariance power of the degree-$d$ Wiener chaos.  Specifically, if $(U_{d,j},U_{d,j}')$ are paired with correlation $t$, then \eqref{eq:hermite-cov} gives
\[
  \E[P_{d,N}P_{d,N}']=t^d.
\]
For background on Hermite polynomials and Wiener chaos, see Janson's book on Gaussian Hilbert spaces~\cite{Janson1997GaussianHilbertSpaces}.
\end{definition}

\subsection{Finite-dimensional schemes}\label{subsec:finite-schemes}

\begin{definition}[Finite Hermite-average family]\label{def:finite-family}
Let $D\subseteq\{3,5,7,9,\ldots\}$ be a finite set of odd degrees.  For each $d\in D$, fix a real weight $s_d$, and define the relative sign
\[
  \sigma_d=(-1)^{(d-1)/2}.
\]
% Thus $\sigma_3=-1$, $\sigma_5=+1$, $\sigma_7=-1$, and so on.

For length $N$, let
\[
  P_{d,N}=N^{-1/2}\sum_{j=1}^N \He_d(U_{d,j}),
\]
where all variables $Z,X,U_{d,j}$ are independent standard Gaussians.  The finite rounding functions are
\begin{align}
  f_N&=\sgn\biggl(Z+\eta \He_3(X)+\sum_{d\in D}s_dP_{d,N}\biggr),\label{eq:finite-f-general}\\
  g_N&=\sgn\biggl(Z-\eta \He_3(X)+\sum_{d\in D}\sigma_d s_dP_{d,N}\biggr).\label{eq:finite-g-general}
\end{align}
They are odd measurable functions on $\R^{2+|D|N}$.  
% The value of $\sgn(0)$ is immaterial, since every threshold event has probability zero.
\end{definition}

\begin{definition}[The third/fifth finite scheme]\label{def:finite-35}
The scheme used for the numerical certificate is the specialization of Definition~\ref{def:finite-family} with $D=\{3,5\}$ and
\begin{equation}\label{eq:params}
  \eta=0.136419125,
  \qquad
  s_3=0.34101124,
  \qquad
  s_5=0.05276111.
\end{equation}
Equivalently,
\begin{align}
  f_N&=\sgn\bigl(Z+\eta \He_3(X)+s_3P_{3,N}+s_5P_{5,N}\bigr),\label{eq:finite-f-35}\\
  g_N&=\sgn\bigl(Z-\eta \He_3(X)-s_3P_{3,N}+s_5P_{5,N}\bigr).\label{eq:finite-g-35}
\end{align}
Thus degree $3$ is anti-aligned between the two sides, while degree $5$ is aligned.
\end{definition}

\subsection{The limiting model}\label{subsec:limiting-model}

\begin{definition}[Limiting model]\label{def:limiting-model}
Let $D,\eta,(s_d)_{d\in D}$ be as in Definition~\ref{def:finite-family}.  Let $R_d$, $d\in D$, be independent standard Gaussians.  The limiting threshold pair is
\begin{align}
  f(z,x,(r_d))&=\sgn\biggl(z+\eta \He_3(x)+\sum_{d\in D}s_dr_d\biggr),\label{eq:lim-f-general}\\
  g(z,x,(r_d))&=\sgn\biggl(z-\eta \He_3(x)+\sum_{d\in D}\sigma_d s_dr_d\biggr).\label{eq:lim-g-general}
\end{align}
For the limiting correlation at parameter $t$, the paired coordinates satisfy
\[
  \rho_Z=t,
  \qquad \rho_X=t,
  \qquad \rho_d=t^d\quad(d\in D),
\]
and different coordinate pairs are independent.  The arcsine-normalized limiting correlation is
\begin{equation}\label{eq:lim-H}
  H(t)={\pi\over2}\E\bigl[f(Z,X,(R_d))g(Z',X',(R_d'))\bigr].
\end{equation}
\end{definition}

Because all degrees in the model are odd, $H$ is an odd function.  For $D=\{3,5\}$, Definition~\ref{def:limiting-model} implies that the extra coordinates have correlations $t^3$ and $t^5$, which come from the finite Hermite averages through \eqref{eq:hermite-cov}.


==> old/certification.tex <==
\section{New Certification Section}

Write
\[
H(t)
=
b_1t
+
\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}} b_m t^m,
\qquad
B_3^2
:=
\sum_{\substack{m\ge 1\\ m\ \mathrm{odd}}} m^6 b_m^2.
\]
The certificate reduces to a single comparison between the linear
coefficient and the total nonlinear coefficient mass.

\begin{proposition}[Head--tail inverse certificate]
\label{prop:head-tail-certificate}
Let \(N\) be odd. If
\begin{equation}
\gamma
+
\sum_{\substack{3\le m\le N\\m\ \mathrm{odd}}}|b_m|
+
\frac{B_3}{\sqrt{10N^5}}
<
b_1,
\label{eq:head-tail-condition}
\end{equation}
then the local inverse
\[
G(z)=H^{-1}(z)=\sum_{n\ge1}a_nz^n
\]
extends holomorphically to a neighborhood of
\(\gamma\overline{\mathbb D}\), maps this neighborhood into
\(\mathbb D\) after shrinking it if necessary, and satisfies
\[
\sum_{n\ge1}|a_n|\gamma^n<1.
\]
\end{proposition}

\begin{proof}
By Cauchy--Schwarz,
\[
\sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
\le
B_3
\left(
\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}
\right)^{1/2}.
\]
Since \(N\) is odd and \(x\mapsto x^{-6}\) is decreasing,
\[
\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}
\le
\frac12\int_N^\infty x^{-6}\,dx
=
\frac{1}{10N^5}.
\]
Consequently, if
\[
\eta:=\sum_{m\ge3}|b_m|,
\]
then \eqref{eq:head-tail-condition} implies
\[
\gamma+\eta<b_1.
\]

Set
\[
\widehat E(u):=\sum_{m\ge3}|b_m|u^m.
\]
Let
\[
G(z)=\sum_{n\ge1}a_nz^n
\]
be the formal inverse of \(H\), and let
\[
V(z)=\sum_{n\ge1}v_nz^n
\]
be the unique formal power series with nonnegative coefficients
satisfying
\[
b_1V(z)=z+\widehat E(V(z)).
\]
Comparing coefficients in
\[
b_1G(z)=z-E(G(z))
\]
and inducting on the degree gives
\[
|a_n|\le v_n
\qquad (n\ge1).
\]

Equivalently, \(V\) is obtained coefficientwise from the Picard
iteration
\[
V_0(z)=0,
\qquad
V_{k+1}(z)
=
\frac{z+\widehat E(V_k(z))}{b_1}.
\]
Put
\[
q:=\frac{\gamma+\eta}{b_1}<1.
\]
If \(V_k(\gamma)\le1\), then
\[
V_{k+1}(\gamma)
\le
\frac{\gamma+\widehat E(1)}{b_1}
=
q.
\]
Thus the iterates are bounded by \(q\), and monotone convergence gives
\[
\sum_{n\ge1}|a_n|\gamma^n
\le
V(\gamma)
\le q
<1.
\]

Since the inequality \(\gamma+\eta<b_1\) is strict, it remains true
with \(\gamma\) replaced by some
\(\widetilde\gamma>\gamma\). Repeating the argument at
\(\widetilde\gamma\) shows that \(G\) converges absolutely there and
satisfies
\[
\sup_{|z|\le\widetilde\gamma}|G(z)|<1.
\]
The formal identity \(H(G(z))=z\) therefore holds analytically on
\(\widetilde\gamma\mathbb D\), proving the claimed extension and
mapping property.
\end{proof}

\begin{proposition}[Certified numerical data]
\label{prop:certified-data}
For the cubic--quintic scheme and \(N=251\), interval arithmetic
certifies
\[
b_1\ge 0.881573822049,
\]
\[
\sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|
\le 1.1328860\cdot10^{-5},
\]
and
\[
B_3\le36.
\]
\end{proposition}

\begin{proof}
The coefficient-head computation and the certified Sobolev estimate
are proved in Appendix~\ref{app:numerical-certificate}.
\end{proof}

We now take
\[
\gamma=0.881545409.
\]
Proposition~\ref{prop:certified-data} gives
\[
\gamma
+
\sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|
+
\frac{B_3}{\sqrt{10\cdot251^5}}
\le
0.881568143462
<
0.881573822049
\le b_1.
\]
Hence Proposition~\ref{prop:head-tail-certificate} gives
\[
\sum_{n\ge1}|a_n|\gamma^n<1.
\]
The finite-dimensional transfer theorem and the classical Krivine
criterion therefore imply
\[
K_G
\le
\frac{\pi}{2\gamma}
\le
1.7818666069360661.
\]




\section{Certification}
\label{sec:certification}

This section contains the complete limiting certificate and the final proof of Theorem~\ref{thm:main}.  The analytic estimates are grouped with the interval-arithmetic quantities that certify them: the Wiener-algebra inverse criterion, the Sobolev tail bound, the bound on the Sobolev norm, the assembly of the numerical inequalities, the formal finite-dimensional proof, and the computational formulas used by the certificate.


\subsection{A Wiener-algebra certificate for the limiting inverse}\label{sec:wiener}

This subsection implements the inverse-majorant step of the proof architecture.  The point is that the nonlinear part of $H$ is small in the Wiener algebra, so the inverse majorant can be certified without computing a long inverse series.

\begin{definition}[Wiener-algebra data]\label{def:wiener-data}
Let $\calA$ be the Wiener algebra of absolutely convergent power series on the unit disk:
\[
  U(w)=\sum_{n\ge0}u_nw^n,
  \qquad
  \|U\|_1=\sum_{n\ge0}|u_n|<\infty.
\]
Then $\|UV\|_1\le\|U\|_1\|V\|_1$.  Write
\begin{equation}\label{eq:H-linear-nonlinear}
  H(t)=b_1t+E(t),
  \qquad
  E(t)=\sum_{m\ge3}b_mt^m,
\end{equation}
and define
\begin{equation}\label{eq:eta0eta1}
  \eta_0=\sum_{m\ge3}|b_m|,
  \qquad
  \eta_1=\sum_{m\ge3}m|b_m|.
\end{equation}
\end{definition}

On the unit ball of $\calA$, the nonlinear part is $\eta_1$-Lipschitz:
\begin{equation}\label{eq:E-lipschitz-simple}
  \|E(U)-E(V)\|_1\le \eta_1\|U-V\|_1,
  \qquad \|U\|_1,\|V\|_1\le1.
\end{equation}
This follows from $\|U^m-V^m\|_1\le m\|U-V\|_1$ on the unit ball.

\begin{theorem}[Wiener contraction certificate]\label{thm:simple-wiener}
Assume
\begin{equation}\label{eq:simple-wiener-cond}
  \eta_1<b_1,
  \qquad
  \gamma+\eta_0<b_1.
\end{equation}
Then $H^{-1}$ is holomorphic on the disk of radius $\gamma$ and
\[
  \sum_{n\ge1}|A_n|\gamma^n<1,
  \qquad H^{-1}(\zeta)=\sum_{n\ge1}A_n\zeta^n.
\]
Moreover the inverse branch is holomorphic on a neighborhood of $\gamma\overline\D$, and it maps $\gamma\D$ into $\D$.
\end{theorem}

\begin{proof}
We first construct the inverse branch as a fixed point in the Wiener algebra, rather than assuming it exists.  The equation $H(U)=\gamma w$ is equivalent, as an identity in $\calA$, to
\[
  U=\Phi(U):={\gamma w-E(U)\over b_1}.
\]
Consider the closed unit ball
\[
  \calB=\{U\in\calA: U(0)=0,\ \|U\|_1\le1\}.
\]
If $U\in\calB$, then
\[
  \|E(U)\|_1\le\sum_{m\ge3}|b_m|\|U\|_1^m\le\eta_0,
\]
so
\[
  \|\Phi(U)\|_1\le{\gamma+\eta_0\over b_1}<1.
\]
For $U,V\in\calB$, \eqref{eq:E-lipschitz-simple} gives
\[
  \|\Phi(U)-\Phi(V)\|_1\le{\eta_1\over b_1}\|U-V\|_1.
\]
Thus $\Phi$ is a contraction from $\calB$ to itself.  Let $U$ be its unique fixed point.  Then $H(U(w))=\gamma w$ as a power-series identity in $\calA$, and
\[
  \|U\|_1=\sum_{n\ge1}|A_n|\gamma^n\le {\gamma+\eta_0\over b_1}<1.
\]

It remains to record the analytic room needed for the finite-dimensional transfer and to identify the fixed point with a holomorphic inverse branch.  Put $q=\|U\|_1<1$, and choose $q<q_*<1$.  For $u,v\in q_*\overline\D$,
\[
  |H(u)-H(v)|\ge b_1|u-v|-\sum_{m\ge3}|b_m||u^m-v^m|
  \ge \left(b_1-\sum_{m\ge3}m|b_m|q_*^{m-1}\right)|u-v|
  \ge (b_1-\eta_1)|u-v|.
\]
Hence $H$ is injective on $q_*\D$ and $H'$ has no zero there.  Since $U(\overline\D)\subset q\overline\D\subset q_*\D$, the compact set $\gamma\overline\D=H(U(\overline\D))$ lies in the open set $H(q_*\D)$, on which the inverse branch is holomorphic.  In particular, it is holomorphic on a neighborhood of $\gamma\overline\D$; after shrinking this neighborhood to a slightly larger disk if necessary, it has the form required for the finite-dimensional transfer theorem.
\end{proof}



\subsection{The coefficient tail through a Sobolev norm}\label{sec:sobolev-tail}

This subsection controls the tail of the original correlation series $H$, not the tail of the inverse series.  The advantage is that the coefficients $b_m$ are signed and have substantial cancellation; the Sobolev norm below sees this cancellation.

Let
\[
  \Dop=t{d\over dt}
\]
be the Euler operator, so that $\Dop t^m=mt^m$.  For the odd series $H(t)=\sum_{m\ \mathrm{odd}}b_mt^m$, define
\begin{equation}\label{eq:B-s}
  B_s^2=\sum_{\substack{m\ge1\\m\ \mathrm{odd}}}m^{2s}b_m^2
  ={1\over2\pi}\int_0^{2\pi}\left|\Dop^sH(e^{i\theta})\right|^2\,d\theta.
\end{equation}
The equality is Parseval on the unit circle.

\begin{lemma}[Sobolev tail]\label{lem:sobolev-tail}
Let $N$ be odd.  Then
\[
  \sum_{m>N}|b_m|\le B_3\left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2},
\]
and
\[
  \sum_{m>N}m|b_m|\le B_3\left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-4}\right)^{1/2}.
\]
\end{lemma}

\begin{proof}
Write $|b_m|=m^{-3}\cdot m^3|b_m|$ and $m|b_m|=m^{-2}\cdot m^3|b_m|$, then apply Cauchy-Schwarz and use $\sum_{m>N}m^6b_m^2\le B_3^2$.
\end{proof}

The power-sum factors are tiny.  With $N=251$,
\begin{equation}\label{eq:tail-factors}
  \left(\sum_{\substack{m>251\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}\le3.13677\cdot10^{-7},
  \qquad
  \left(\sum_{\substack{m>251\\m\ \mathrm{odd}}}m^{-4}\right)^{1/2}\le1.020511\cdot10^{-4}.
\end{equation}
Each odd power sum is enclosed by a finite head plus a decreasing-integral remainder.  Thus even a crude bound on $B_3$ suffices.



\subsection{Bounding the Sobolev norm}\label{sec:sobolev-norm}

By \eqref{eq:B-s}, it is enough to bound $\Dop^3H(e^{i\theta})$ on the circle.  We realize $\Dop^3H$ as a trace of a two-dimensional differential kernel and apply an averaged inequality.


\subsubsection{A combined kernel}

For real $|r|<1$, let $\Kr_r$ be the centered bivariate Gaussian density of correlation $r$,
\begin{equation}\label{eq:Kr-kernel}
  \Kr_r(u,v)={1\over2\pi\sqrt{1-r^2}}
  \exp\left(-{u^2-2ruv+v^2\over2(1-r^2)}\right).
\end{equation}
We use the same formula by analytic continuation for the complex values $r=\rho(e^{i\theta})$ that occur below; on this compact curve $1-r^2$ is bounded away from zero, and the square-root branch is fixed continuously from $r=0$.  Set $h(x)=\He_3(x)$ and let $\vartheta=\eta/\sqrt V$ be as in Definition~\ref{def:collapsed-data}.  For fixed real $x,y$, define the threshold-covariance kernel
\begin{equation}\label{eq:threshold-cov-kernel}
  \mathcal C_r(x,y)
  ={\pi\over2}\,\E\bigl[\sgn(W+\vartheta h(x))\sgn(W'+\vartheta h(y))\bigr],
\end{equation}
where $(W,W')$ is a centered standard Gaussian pair of correlation $r$.  Equivalently, for $|r|<1$,
\begin{equation}\label{eq:C-Hermite-expansion}
  \mathcal C_r(x,y)
  ={\pi\over2}\sum_{a\ge0}r^a q_a(\vartheta h(x))q_a(\vartheta h(y)),
\end{equation}
with $q_a$ as in Definition~\ref{def:qk}.  This formula gives the analytic continuation in $r$ used in the differentiated kernels.

The two first derivative identities are
\begin{equation}\label{eq:C-first-derivatives}
  \partial_r\mathcal C_r(x,y)=2\pi\Kr_r(\vartheta h(x),\vartheta h(y)),
  \qquad
  \partial_x\partial_y\mathcal C_r(x,y)
  =2\pi\vartheta^2h'(x)h'(y)\Kr_r(\vartheta h(x),\vartheta h(y)).
\end{equation}
Indeed, the first identity is Price's theorem in the $W,W'$ variables, or follows by differentiating \eqref{eq:C-Hermite-expansion} and using the Mehler expansion of $\Kr_r$.  For the second, one uses $q_a'(u)=2\varphi(u)\He_a(-u)$ and then the same Mehler expansion.  Thus after one correlation derivative every kernel is a polynomial differential operator applied to $\Kr_r$; no discontinuous sign kernel remains.

We next define the boundary trace in the $x,y$ variables.  Let $\mu$ be the product standard Gaussian measure on $\R^2$.  If a kernel $\Psi$ satisfies $\Psi,\partial_x\partial_y\Psi\in L^2(\mu)$, write its Hermite coefficients as
\[
  \widehat\Psi_{i,j}=\iint_{\R^2}\Psi(x,y)\He_i(x)\He_j(y)\,d\mu(x,y).
\]
For $|\lambda|\le1$ set
\begin{equation}\label{eq:Tlambda-definition}
  T_\lambda[\Psi]
  =\widehat\Psi_{0,0}+\sum_{n\ge1}\lambda^n\widehat\Psi_{n,n}.
\end{equation}
For $|\lambda|<1$, this is exactly the correlated Gaussian expectation $\E[\Psi(X,Y)]$ with $\operatorname{corr}(X,Y)=\lambda$.  For $|\lambda|=1$, \eqref{eq:Tlambda-definition} is the Sobolev boundary trace of that expectation.

The series in \eqref{eq:Tlambda-definition} converges absolutely on $|\lambda|=1$.  Moreover
\begin{equation}\label{eq:Tlambda-bound}
  |T_\lambda[\Psi]|
  \le {\pi\over\sqrt6}
  \left(\|\Psi\|_{L^2(\mu)}^2+4\|\partial_x\partial_y\Psi\|_{L^2(\mu)}^2\right)^{1/2}.
\end{equation}
To see this, note that
\[
  |\widehat\Psi_{0,0}|\le\|\Psi\|_{L^2(\mu)}
\]
and, since the coefficient of $\He_{n-1}(x)\He_{n-1}(y)$ in $\partial_x\partial_y\Psi$ is $n\widehat\Psi_{n,n}$,
\[
  \sum_{n\ge1}|\widehat\Psi_{n,n}|
  \le\left(\sum_{n\ge1}{1\over n^2}\right)^{1/2}
      \left(\sum_{n\ge1}n^2|\widehat\Psi_{n,n}|^2\right)^{1/2}
  \le {\pi\over\sqrt6}\|\partial_x\partial_y\Psi\|_{L^2(\mu)}.
\]
The displayed estimate follows from the elementary inequality
\[
  A+{\pi\over\sqrt6}B
  \le {\pi\over\sqrt6}\sqrt{A^2+4B^2}\qquad(A,B\ge0),
\]
using $\pi^2/6>4/3$.

With $\lambda=-t$ and $\Dop_t=t\partial_t$, define recursively
\begin{equation}\label{eq:Phi-recursion}
  \Phi_0(t;x,y)=\mathcal C_{\rho(t)}(x,y),
  \qquad
  \Phi_{k+1}=\Dop_t\Phi_k+\lambda\,\partial_x\partial_y\Phi_k\quad(k\ge0),
\end{equation}
where $\rho$ is the polynomial in \eqref{eq:rho-collapsed}.  Here $\Dop_t$ differentiates all explicit $t$-dependence of $\Phi_k$, including the dependence through $\rho(t)$ and through scalar prefactors created at earlier steps.  The combined kernel $\Phi_3$ is obtained by carrying out this recursion before any norm is taken.  By \eqref{eq:C-first-derivatives}, $\Phi_3$ is a finite sum of smooth $\Kr_r$-derivative kernels.

\begin{lemma}[Trace representation]\label{lem:trace-rep}
For $|t|=1$,
\[
  \Dop^3H(t)=T_{-t}\bigl[\Phi_3(t;\cdot,\cdot)\bigr],
\]
and $T_{-t}$ satisfies the bound \eqref{eq:Tlambda-bound}.
\end{lemma}

\begin{proof}
First assume $|t|<1$, and put $\lambda(t)=-t$.  The collapsed representation of Proposition~\ref{prop:collapsed-coefficients} is equivalently
\begin{equation}\label{eq:H-as-trace-C}
  H(t)=T_{\lambda(t)}\bigl[\mathcal C_{\rho(t)}\bigr].
\end{equation}
Indeed, for $|\lambda|<1$, the trace is the correlated expectation in the $X,Y$ variables, and \eqref{eq:threshold-cov-kernel} is precisely the conditional $W,W'$ expectation multiplied by the normalizing factor $\pi/2$.

We use the following differentiation identity.  If $\Psi(t)$ is a smooth family of kernels with enough decay, then
\begin{equation}\label{eq:trace-differentiation}
  \Dop_t\,T_{\lambda(t)}[\Psi(t)]
  =T_{\lambda(t)}\bigl[\Dop_t\Psi(t)+\lambda(t)\partial_x\partial_y\Psi(t)\bigr].
\end{equation}
For $|\lambda|<1$ this is Price's theorem in the outer Gaussian variables.  Equivalently, it follows directly from the Hermite definition of $T_\lambda$: differentiating
\[
  T_{\lambda(t)}[\Psi(t)]
  =\sum_{n\ge0}\lambda(t)^n\widehat\Psi_{n,n}(t)
\]
gives the term $\sum_n\lambda^n\Dop_t\widehat\Psi_{n,n}$ plus
\[
  \sum_{n\ge1} n\lambda^n\widehat\Psi_{n,n}
  =\lambda\sum_{m\ge0}(m+1)\lambda^m\widehat\Psi_{m+1,m+1},
\]
and the latter is $\lambda T_\lambda[\partial_x\partial_y\Psi]$ because
\[
  \partial_x\partial_y\Psi
  =\sum_{i,j\ge1}\sqrt{ij}\,\widehat\Psi_{i,j}\He_{i-1}(x)\He_{j-1}(y)
  \quad\text{in the Hermite sense.}
\]

Starting from \eqref{eq:H-as-trace-C} and applying \eqref{eq:trace-differentiation} three times gives
\[
  \Dop^3H(t)=T_{\lambda(t)}[\Phi_3(t;\cdot,\cdot)]
  \qquad(|t|<1),
\]
with $\Phi_k$ exactly as in \eqref{eq:Phi-recursion}.  The identities \eqref{eq:C-first-derivatives} show that every term in $\Phi_3$ is a smooth kernel of the form used in Subsection~\ref{sec:formulas}; in particular $\Phi_3$ and $\partial_x\partial_y\Phi_3$ lie in $L^2(\mu)$ uniformly for radial limits $t=re^{i\theta}$, $0<r\le1$.

Letting $r\uparrow1$ in the identity for $re^{i\theta}$ gives the asserted boundary identity for $|t|=1$, with $\Dop^3H(e^{i\theta})$ understood as the radial boundary value.  The right-hand side has this limit because $\Phi_3$ is an explicit finite sum of the smooth kernels listed in Subsection~\ref{sec:formulas}, and because $T_\lambda$ is continuous for the Sobolev trace norm appearing in \eqref{eq:Tlambda-bound}.  Finally, the bound for $T_{-t}$ is \eqref{eq:Tlambda-bound}.
\end{proof}

The recursion \eqref{eq:Phi-recursion} expands $\Phi_3$ as a finite sum over a nine-term index set; the explicit prefactors and kernels are recorded in Subsection~\ref{sec:formulas}.

\subsubsection{An averaged Minkowski bound}

From Lemma~\ref{lem:trace-rep} and \eqref{eq:B-s},
\begin{equation}\label{eq:B3-avg}
  B_3^2={1\over2\pi}\int_0^{2\pi}|\Dop^3H(e^{i\theta})|^2\,d\theta
  \le {\pi^2\over6}\,\overline S,
\end{equation}
where
\[
  \overline S={1\over2\pi}\int_0^{2\pi}S(\theta)\,d\theta,
  \qquad
  S(\theta)=\|\Phi_3\|_{L^2(\mu)}^2+4\|\partial_x\partial_y\Phi_3\|_{L^2(\mu)}^2,
\]
and $\Phi_3$ is taken at $t=e^{i\theta}$.

\begin{lemma}[Averaged Minkowski]\label{lem:averaged-minkowski}
Write $\Phi_3=\sum_{p,a}c_{p,a}(t)G_{p,a}$ for the expansion produced by \eqref{eq:Phi-recursion}, with scalar prefactors $c_{p,a}$ and kernels $G_{p,a}$ as in Subsection~\ref{sec:formulas}.  For each pair set
\[
  Q^{(0)}_{p,a}={1\over2\pi}\int_0^{2\pi}|c_{p,a}(e^{i\theta})|^2\|G_{p,a}\|_{L^2(\mu)}^2\,d\theta,
\]
and
\[
  Q^{(1)}_{p,a}={1\over2\pi}\int_0^{2\pi}|c_{p,a}(e^{i\theta})|^2\|\partial_x\partial_yG_{p,a}\|_{L^2(\mu)}^2\,d\theta.
\]
Then
\begin{equation}\label{eq:S-minkowski}
  \overline S\le
  \left(\sum_{p,a}\sqrt{Q^{(0)}_{p,a}}\right)^2
  +4\left(\sum_{p,a}\sqrt{Q^{(1)}_{p,a}}\right)^2.
\end{equation}
\end{lemma}

\begin{proof}
By the triangle inequality in $L^2(\mu)$,
\[
  \|\Phi_3\|_{L^2(\mu)}\le\sum_{p,a}|c_{p,a}|\|G_{p,a}\|_{L^2(\mu)}
\]
pointwise in $\theta$, and likewise for $\partial_x\partial_y\Phi_3$.  Taking the $L^2(d\theta/2\pi)$ norm of each sum and applying the triangle inequality there gives the two terms in \eqref{eq:S-minkowski}.
\end{proof}

Each $G_{p,a}$ is, on the real axis, a polynomial times a super-Gaussian, so the $L^2(\mu)$ norms are two-dimensional Gaussian integrals.  We enclose these integrals and then enclose the circle averages $Q^{(\cdot)}_{p,a}$ by a composite Gauss-Legendre rule with a certified remainder, as described in Subsection~\ref{sec:formulas}.

\begin{lemma}[Certified Sobolev bound]\label{lem:B3-certified}
The interval computation gives
\[
  \overline S\le1803.317.
\]
Consequently,
\[
  B_3\le{\pi\over\sqrt6}\sqrt{1803.317}\le54.4641.
\]
\end{lemma}

The per-pair contributions, certified through the quadrature, are listed in Table~\ref{tab:Q}.  The bound $54.4641$ is intentionally generous; it is already far more than enough because of the small tail factors in \eqref{eq:tail-factors}.

\begin{table}[t]\centering
\small
\begin{tabular}{c r r}
\toprule
$(p,a)$ & $\sqrt{Q^{(0)}_{p,a}}$ & $\sqrt{Q^{(1)}_{p,a}}$ \\
\midrule
$(0,1)$ & $0.04286765$ & $0.10127946$ \\
$(0,2)$ & $0.30383835$ & $1.10543141$ \\
$(0,3)$ & $0.36847714$ & $7.40413211$ \\
$(1,0)$ & $2.67546361$ & $0.10772752$ \\
$(1,1)$ & $0.19214422$ & $0.85400602$ \\
$(1,2)$ & $0.51708607$ & $6.83760791$ \\
$(2,0)$ & $2.30597621$ & $0.29542681$ \\
$(2,1)$ & $0.41663640$ & $3.10773691$ \\
$(3,0)$ & $2.36356861$ & $0.91665956$ \\
\bottomrule
\end{tabular}
\caption{Certified upper bounds for the per-pair quantities of Lemma~\ref{lem:averaged-minkowski}; substituting into \eqref{eq:S-minkowski} gives $\overline S\le1803.317$.}
\label{tab:Q}
\end{table}



\subsection{Assembling the certificate}\label{sec:assembly}

This subsection combines the certified coefficient head, the Sobolev tail, and the Wiener-algebra criterion.  The cutoff is $N=251$.

\begin{lemma}[Certified coefficient head]\label{lem:certified-head}
Using the coefficient formula of Proposition~\ref{prop:collapsed-coefficients} and the interval enclosures described in Subsection~\ref{sec:formulas}, the first coefficients are certified with
\[
  b_1\ge0.881573822049,
  \qquad
  b_3\approx3.4538733\cdot10^{-9},
  \qquad
  b_5\approx-9.0435536\cdot10^{-11}.
\]
Here ``$\approx$'' means that the displayed decimal lies in the corresponding outward-rounded interval enclosure.
Moreover the partial sums through degree $251$ satisfy
\begin{equation}\label{eq:certified-head-sums}
  \sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|\le1.1328860\cdot10^{-5},
  \qquad
  \sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}m|b_m|\le1.5737642\cdot10^{-4}.
\end{equation}
\end{lemma}

The near-vanishing of $b_3$ and $b_5$ is the design goal.  If
\[
  H(t)=b_1t+b_3t^3+b_5t^5+\cdots,
  \qquad
  H^{-1}(\zeta)=A_1\zeta+A_3\zeta^3+A_5\zeta^5+\cdots,
\]
then formal series reversion gives
\begin{equation}\label{eq:low-inverse}
  A_1={1\over b_1},
  \qquad
  A_3=-{b_3\over b_1^4},
  \qquad
  A_5={3b_3^2-b_1b_5\over b_1^7}.
\end{equation}
Thus making $b_3$ and $b_5$ small makes the first two nonlinear inverse coefficients small.

\begin{proposition}[Limiting admissibility]\label{prop:limiting-admissibility}
For $\gamma=0.881545409$, the limiting third/fifth model satisfies
\[
  \sum_{n\ge1}|A_n|\gamma^n<1,
  \qquad H^{-1}(\zeta)=\sum_{n\ge1}A_n\zeta^n.
\]
The inverse branch is holomorphic on a neighborhood of $\gamma\overline\D$ and maps $\gamma\D$ into $\D$.
\end{proposition}

\begin{proof}
By Lemmas~\ref{lem:sobolev-tail} and~\ref{lem:B3-certified}, together with \eqref{eq:tail-factors},
\[
  \sum_{m>251}|b_m|
  \le 54.4641\cdot3.13677\cdot10^{-7},
\]
and
\[
  \sum_{m>251}m|b_m|
  \le 54.4641\cdot1.020511\cdot10^{-4}.
\]
Combining these inequalities with \eqref{eq:certified-head-sums},
\[
  \eta_0=\sum_{m\ge3}|b_m|
  \le1.1328860\cdot10^{-5}+54.4641\cdot3.13677\cdot10^{-7}
  \le2.84130\cdot10^{-5},
\]
and
\[
  \eta_1=\sum_{m\ge3}m|b_m|
  \le1.5737642\cdot10^{-4}+54.4641\cdot1.020511\cdot10^{-4}
  \le5.71550\cdot10^{-3}.
\]
With $b_1\ge0.881573822049$, we have $\eta_1<b_1$ and
\[
  \gamma+\eta_0\le0.881573821996<0.881573822049\le b_1.
\]
Theorem~\ref{thm:simple-wiener} applies and proves the claim.
\end{proof}

\subsection{Formal proof of Theorem~\ref{thm:main}}\label{subsec:formal-proof-main}

\begin{proof}[Proof of Theorem~\ref{thm:main}]
By Proposition~\ref{prop:limiting-admissibility}, the limiting model satisfies a strict inverse-majorant certificate at $\gamma=0.881545409$, with inverse branch holomorphic on a neighborhood of $\gamma\overline\D$ and with values in $\D$ on a slightly larger closed disk around $\gamma\overline\D$.  Corollary~\ref{cor:finite-scheme} transfers this certificate to all sufficiently high finite-dimensional third/fifth Gaussianized-chaos schemes \eqref{eq:finite-f-35}--\eqref{eq:finite-g-35}.  Applying the Krivine criterion, Lemma~\ref{lem:local-inverse-expansion} or equivalently Theorem~\ref{thm:krivine-criterion}, to such a finite scheme gives
\[
  \KG\le {\pi\over2\gamma}\le1.7818666069360661.
\]
Since
\[
  {\pi\over 2\log(1+\sqrt2)}-{\pi\over2\gamma}
  =3.473712553\cdot10^{-4}\ldots,
\]
the hyperplane-improvement form follows.
\end{proof}



\subsection{Computational formulas}\label{sec:formulas}

This subsection lists the explicit objects used in the interval certificate.  All real inputs are decimal intervals and all derived quantities are outward-rounded Arb balls.

\paragraph{Parameters.}
The parameters are $\eta,s_3,s_5$ from \eqref{eq:params}.  We set
\[
  V=1+s_3^2+s_5^2,
  \qquad
  \vartheta={\eta\over\sqrt V},
  \qquad
  \rho(t)={t-s_3^2t^3+s_5^2t^5\over V}.
\]

\paragraph{Coefficient integrals.}
The collapsed coefficients are
\[
  \mathsf A_{a,b}=\int_\R \He_b(x)q_a(\vartheta\He_3(x))\varphi(x)\,dx,
\]
where $q_a$ is given by Lemma~\ref{lem:qk}.  The integrand is entire.  For $a\ge1$ it contains the extra factor $e^{-(\vartheta\He_3(x))^2/2}$ and is super-Gaussian on the real axis; for $a=0$ it has the ordinary Gaussian tail from $\varphi(x)$.  It is enclosed by Arb's adaptive integrator on a finite interval $[-L,L]$, plus a closed Gaussian-tail bound outside the interval using $|q_a|\le1$.  The coefficient $b_m$ is then the interval sum \eqref{eq:bm-collapsed}, with $[t^{m-b}]\rho(t)^a$ computed by a finite convolution of $(1,-s_3^2,s_5^2)/V$.  Absolute values in $\eta_0$ and $\eta_1$ are taken on enclosures bounded away from zero.

\paragraph{Combined kernel.}
The recursion \eqref{eq:Phi-recursion} produces
\[
  \Phi_3=\sum_{(p,a)}c_{p,a}(t)G_{p,a}
\]
over the nine pairs in Table~\ref{tab:Q}.  The scalar prefactors $c_{p,a}(t)$ are polynomials in $t$, generated from the formal seed $c_{0,0}=1$ for the threshold-covariance kernel $\mathcal C_{\rho(t)}$ by applying three times the substitutions
\[
  c_{p,a}\longmapsto \Dop_tc_{p,a}\quad\text{at the same }(p,a),
\]
\[
  c_{p,a}\longmapsto (\Dop_t\rho)c_{p,a}\quad\text{at }(p+1,a),
  \qquad
  c_{p,a}\longmapsto (-t)c_{p,a}\quad\text{at }(p,a+1).
\]
The first time a substitution moves from the formal seed to either $(p+1,a)$ or $(p,a+1)$, the identities \eqref{eq:C-first-derivatives} supply the displayed $2\pi$ factors.  The kernels are, with $\varphi_r=\Kr_r$ from \eqref{eq:Kr-kernel} evaluated at $u=\vartheta h(x)$, $v=\vartheta h(y)$, and $r=\rho(t)$,
\[
  G_{p,0}=2\pi\,\partial_r^{p-1}\varphi_r\quad(p\ge1),
\]
and
\[
  G_{p,a}=\partial_x^{a-1}\partial_y^{a-1}
  \left(2\pi\vartheta^2h'(x)h'(y)\partial_r^p\varphi_r\right)
  \quad(a\ge1).
\]
Each derivative $\partial_r^p\partial_x^i\partial_y^j\varphi_r$ equals a polynomial in $(r,u,v,1-r^2)$ times $\varphi_r$, with integer coefficients computed by a fixed operator recurrence.

\paragraph{Gaussian norms.}
Writing $u=\vartheta h(x)$, the squared modulus of a kernel against $\mu$ is
\[
  \|G_{p,a}\|_{L^2(\mu)}^2=
  \iint_{\R^2}|G_{p,a}(x,y)|^2{e^{-(x^2+y^2)/2}\over2\pi}\,dx\,dy.
\]
This is a positive integral of a polynomial times $e^{-x^2/2-y^2/2}$ and the bounded factor
\[
  \exp\left(-A\vartheta^2(h(x)^2+h(y)^2)+2B\vartheta^2h(x)h(y)\right),
\]
where
\[
  A=\Re(1/d),\qquad B=\Re(r/d),\qquad d=1-r^2.
\]
Using the identity $x^3=\sqrt6\,h(x)+3x$, every mode reduces to a combination of one-dimensional base moments
\[
  I_{\varepsilon,q}(A)=\E\bigl[X^\varepsilon h(X)^q e^{-A\vartheta^2h(X)^2}\bigr],
  \qquad \varepsilon\in\{0,1,2\},
\]
each enclosed by Arb's integrator; the cross term is expanded in a convergent series with a Chernoff tail.

\paragraph{Circle quadrature and its remainder.}
The averages $Q^{(\cdot)}_{p,a}$ are computed by a composite four-point Gauss-Legendre rule on $[0,2\pi]$ with $M$ panels of the certified point values $|c_{p,a}|^2\|G_{p,a}\|^2$.  For an integrand $g(\theta)$, the rule's error is at most
\[
  C_4(2\pi)^8M^{-9}\sum_jD_{8,j},
  \qquad
  C_4={(4!)^4\over9(8!)^3},
\]
where each panel bound $D_{8,j}\ge\sup_{I_j}|g^{(8)}|$ is obtained without cancellation from
\[
  |g^{(8)}|\le\sum_{j=0}^{8}\binom8j\sqrt{V_jV_{8-j}},
  \qquad
  V_j(\theta)=\|\partial_\theta^j(c_{p,a}G_{p,a})\|_{L^2(\mu)}^2.
\]
The estimate
\[
  V_j\le |d|^{-1}\left(\sum_\nu |p_{j,\nu}(\theta)|\sqrt{L_\nu L_{\nu'}}\right)^2
\]
uses $2|B|\,|UV|\le |B|(U^2+V^2)$ to absorb the mixed term in the exponent, giving the residual decay
\[
  -A(U^2+V^2)+2BUV\le -(A-|B|)(U^2+V^2).
\]
The required positivity margin
\[
  A-|B|=\Re(1/d)-|\Re(r/d)|\ge {1\over2}
\]
on the unit circle is verified on all panels.  Here $L_\nu$ are precomputed positive one-dimensional integrals and $|p_{j,\nu}|$ are bounded by evaluating the $\theta$-derivative coefficients on each panel as intervals.  At $M=2048$ the total remainder is at most $9.1\cdot10^{-4}$ per pair, negligible compared with the final value of $\overline S$.



\subsection{Implementation notes}\label{sec:impl}

The following comments are not needed for the logical proof, but they explain why the certificate is organized in the form used above.

\begin{enumerate}[label=\textbf{I\arabic*.},leftmargin=*]
\item \textbf{Why real-axis integration.}  The integrand of a Gaussian norm decays like $e^{-c x^6}$ on the real axis but can grow like $e^{c|z|^6}$ off the real axis, because $\He_3(z)^2\sim z^6/6$ has negative real part in some complex sectors.  Interval boxes in $(x,y)$, or a complex contour, see this far-field growth and produce much worse bounds.  The certificate therefore evaluates every integral at real points; Arb's adaptive integrator is effective because the local error model only probes small neighborhoods of the real subintervals.

\item \textbf{Why the Sobolev tail.}  Bounding $\sum|b_m|$ through $B_3=\|\Dop^3H\|_{L^2(\T)}$ keeps the cancellation in the signed coefficients $b_m$.  A direct Hermite-mass bound, or a complex Cauchy estimate of $H^{-1}$ near $t=1$, overshoots by many orders of magnitude.

\item \textbf{Why the combined kernel.}  Forming $\Phi_3$ by the recursion \eqref{eq:Phi-recursion} before taking norms is essential.  Expanding $\Dop^3H$ as a sum of separately bounded terms discards a nine-fold cancellation and gives a much looser estimate.

\item \textbf{Why the cancellation-free eighth-derivative bound.}  The exact eighth $\theta$-derivative of the quadrature integrand is a signed combination of inner products whose terms can be enormous near $\theta=0$ and $\theta=\pi$ before cancellation.  The Minkowski bound in Subsection~\ref{sec:formulas} avoids this signed sum entirely: every $V_a$ is a positive quantity, at the cost of a looser derivative bound that is absorbed by the $M^{-9}$ factor in the quadrature remainder.

\item \textbf{Precision.}  The base moments require higher precision for large powers and for circle nodes near $\theta=0,\pi$.  The reported headline inequalities are stable under further refinement of precision and panel count.
\end{enumerate}


==> old/certification_new.tex <==
\section{Certification}
\label{sec:certification}

Write the correlation function of the cubic--quintic limiting scheme as
\begin{equation}
  H(t)=b_1t+\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}} b_m t^m,
  \label{eq:certification-H-series}
\end{equation}
and let
\begin{equation}
  \Delta_H:=\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}}|b_m|
  \label{eq:nonlinear-coefficient-mass}
\end{equation}
be the total mass of its nonlinear coefficients.  Let
\[
  G(z)=H^{-1}(z)=\sum_{n\ge1}a_nz^n
\]
denote the local holomorphic inverse of $H$ at the origin, and define its
majorant by
\begin{equation}
  \mathcal M(r):=\sum_{n\ge1}|a_n|r^n.
  \label{eq:inverse-majorant-certification}
\end{equation}
The local inverse exists because $H'(0)=b_1>0$, by the holomorphic inverse
function theorem.

For the linear map $t\mapsto b_1t$, the condition $\mathcal M(\gamma)<1$ is
simply $\gamma<b_1$.  The next proposition shows that the nonlinear part costs
at most $\Delta_H$ of this margin.

\begin{proposition}[Inverse certificate from near-linearity]
\label{prop:inverse-certificate-near-linearity}
Assume $b_1>0$ and $\Delta_H<\infty$.  If
\begin{equation}
  \gamma+\Delta_H<b_1,
  \label{eq:near-linearity-condition}
\end{equation}
then there exists $R>\gamma$ such that the local inverse $G$ extends
holomorphically to $R\mathbb D$, maps $R\mathbb D$ into $\mathbb D$, and
satisfies
\begin{equation}
  \mathcal M(\gamma)
  \le \frac{\gamma+\Delta_H}{b_1}
  <1.
  \label{eq:near-linearity-conclusion}
\end{equation}
\end{proposition}

\begin{proof}
Set
\[
  E(t):=\sum_{m\ge3}b_mt^m,
  \qquad
  E_{\mathrm{maj}}(u):=\sum_{m\ge3}|b_m|u^m.
\]
There is a unique formal power series
\[
  V(z)=\sum_{n\ge1}v_nz^n
\]
satisfying
\begin{equation}
  b_1V(z)=z+E_{\mathrm{maj}}(V(z)).
  \label{eq:majorizing-inverse-equation}
\end{equation}
Indeed, comparison of the coefficient of $z$ gives $v_1=b_1^{-1}$.  For
$n\ge2$, the coefficient of $z^n$ in $E_{\mathrm{maj}}(V)$ depends only on
$v_1,\ldots,v_{n-1}$, so \eqref{eq:majorizing-inverse-equation} determines
$v_n$ recursively.  The same recursion shows that $v_n\ge0$ for every $n$.

Comparing coefficients in
\[
  b_1G(z)=z-E(G(z))
\]
and in \eqref{eq:majorizing-inverse-equation}, induction on $n$ gives
\begin{equation}
  |a_n|\le v_n
  \qquad(n\ge1).
  \label{eq:inverse-coefficient-domination}
\end{equation}
Indeed, at degree $n$, every nonlinear composition involves only previously
determined coefficients, and replacing each $b_m$ by $|b_m|$ removes all
possible cancellation.

Choose $R>\gamma$ so close to $\gamma$ that
\[
  q:=\frac{R+\Delta_H}{b_1}<1.
\]
Starting from $V_0(z)=0$, define
\begin{equation}
  V_{k+1}(z):=\frac{z+E_{\mathrm{maj}}(V_k(z))}{b_1}.
  \label{eq:majorizing-inverse-iteration}
\end{equation}
The series $V_k$ have nonnegative coefficients and increase coefficientwise,
meaning that each Taylor coefficient is nondecreasing in $k$.
Moreover, if $V_k(R)\le q$, then $V_k(R)<1$ and
\[
  V_{k+1}(R)
  \le \frac{R+E_{\mathrm{maj}}(1)}{b_1}
  =q.
\]
Thus $V_k(R)\le q$ for every $k$.  Their coefficientwise limit satisfies
\eqref{eq:majorizing-inverse-equation}, and hence equals $V$ by uniqueness.
The monotone convergence theorem now gives
\[
  V(R)=\sum_{n\ge1}v_nR^n\le q<1.
\]
Together with \eqref{eq:inverse-coefficient-domination}, this implies
\[
  \sum_{n\ge1}|a_n|R^n\le V(R)<1.
\]
Consequently, the Taylor series of $G$ converges on $R\mathbb D$ and takes
values in $\mathbb D$.  Since the identity $H(G(z))=z$ holds near the origin,
it holds throughout $R\mathbb D$ by the identity theorem.  Finally,
\[
  \mathcal M(\gamma)
  \le V(\gamma)
  =\frac{\gamma+E_{\mathrm{maj}}(V(\gamma))}{b_1}
  \le\frac{\gamma+\Delta_H}{b_1},
\]
because $0\le V(\gamma)\le V(R)<1$.
\end{proof}

It remains to certify $\Delta_H$.  We compute the coefficients through a
finite degree $N$ and bound the remaining tail indirectly.  The point is that
the Euler operator
\[
  D:=t\frac{d}{dt}
\]
multiplies the coefficient of $t^m$ by $m$, so $D^3$ strongly amplifies
high-degree coefficients.  The $L^2(\mathbb T)$ norm below is the
root-mean-square size of the resulting function around the unit circle
$\mathbb T:=\{z\in\mathbb C:|z|=1\}$.

\begin{lemma}[Third-order coefficient-tail bound]
\label{lem:third-order-tail}
Suppose that $D^3H$ has radial boundary values in $L^2(\mathbb T)$, with
\[
  \|D^3H\|_{L^2(\mathbb T)}^2
  :=\frac{1}{2\pi}\int_0^{2\pi}
  |D^3H(e^{i\theta})|^2\,d\theta.
\]
Then, for every odd $N$,
\begin{equation}
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
  \le
  \|D^3H\|_{L^2(\mathbb T)}
  \left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}
  \le
  \frac{\|D^3H\|_{L^2(\mathbb T)}}{\sqrt{10N^5}}.
  \label{eq:third-order-tail}
\end{equation}
\end{lemma}

\begin{proof}
Since $D^3(t^m)=m^3t^m$, Parseval's identity gives
\begin{equation}
  \|D^3H\|_{L^2(\mathbb T)}^2
  =\sum_{\substack{m\ge1\\m\ \mathrm{odd}}}m^6|b_m|^2.
  \label{eq:parseval-third-order}
\end{equation}
The Cauchy--Schwarz inequality therefore gives
\[
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
  =\sum_{\substack{m>N\\m\ \mathrm{odd}}}
  m^{-3}\bigl(m^3|b_m|\bigr)
  \le
  \left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}
  \|D^3H\|_{L^2(\mathbb T)}.
\]
Finally, since $x\mapsto x^{-6}$ is decreasing and consecutive odd integers
are separated by two, the monotone integral estimate gives
\[
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}
  \le\frac12\int_N^\infty x^{-6}\,dx
  =\frac{1}{10N^5}.
\]
\end{proof}

\begin{proposition}[Certified numerical input]
\label{prop:certified-numerical-input}
For the cubic--quintic correlation function, interval arithmetic certifies
\begin{equation}
  b_1\ge0.881573822049,
  \qquad
  \sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|
  \le1.1328860\cdot10^{-5},
  \qquad
  \|D^3H\|_{L^2(\mathbb T)}<35.774<36.
  \label{eq:certified-numerical-input}
\end{equation}
\end{proposition}

\begin{proof}
See Appendix~\ref{app:certification-details}.
\end{proof}

Lemma~\ref{lem:third-order-tail} and
Proposition~\ref{prop:certified-numerical-input} give
\begin{equation}
  \Delta_H
  \le
  1.1328860\cdot10^{-5}
  +\frac{36}{\sqrt{10\cdot251^5}}
  <2.2734462\cdot10^{-5}.
  \label{eq:certified-nonlinear-mass}
\end{equation}

\begin{theorem}[Cubic--quintic upper bound]
\label{thm:cubic-quintic-upper-bound-certified}
For
\[
  \gamma=0.881545409,
\]
the cubic--quintic limiting scheme satisfies $\mathcal M(\gamma)<1$.
Consequently,
\begin{equation}
  K_G\le\frac{\pi}{2\gamma}
  \le1.7818666069360661.
  \label{eq:certified-KG-bound}
\end{equation}
\end{theorem}

\begin{proof}
By \eqref{eq:certified-nonlinear-mass},
\[
  \gamma+\Delta_H
  <0.881545409+2.2734462\cdot10^{-5}
  =0.881568143462
  <0.881573822049
  \le b_1.
\]
Proposition~\ref{prop:inverse-certificate-near-linearity} therefore gives
$\mathcal M(\gamma)<1$, together with the analytic room required by the
finite-dimensional transfer theorem.  That theorem passes the strict
certificate to all sufficiently large ordinary finite-dimensional
approximations.  The classical Krivine preprocessing theorem then gives
\eqref{eq:certified-KG-bound}.
\end{proof}


==> old/coefficient_formulas_old.tex <==
\section{Coefficient Formula for the Limiting Model}
\label{sec:coefficients}

This section implements the coefficient step in the proof architecture.  The point is to reduce the limiting threshold model, with the correlation powers defined in Definition~\ref{def:limiting-model}, to explicit two-dimensional Gaussian integrals.

\subsection{Degree-direction data}\label{subsec:degree-data}

\begin{definition}[Degree-direction normalization]\label{def:degree-normalization}
For a finite degree set $D$ and weights $(s_d)_{d\in D}$, define
\[
  S=\biggl(\sum_{d\in D}s_d^2\biggr)^{1/2},
  \qquad
  \alpha_d={s_d\over S}\quad(d\in D).
\]
Thus $\sum_{d\in D}\alpha_d^2=1$, and
\[
  \sum_{d\in D}s_dr_d=S\sum_{d\in D}\alpha_dr_d.
\]
\end{definition}

\begin{definition}[One-dimensional threshold coefficients]\label{def:qk}
Let $R\sim N(0,1)$.  For $u\in\R$ and $k\in\Nzero$, define
\[
  q_k(u)=\E_R[\sgn(u+R)\He_k(R)].
\]
These are the Hermite coefficients of the one-dimensional threshold $R\mapsto \sgn(u+R)$.
\end{definition}

\begin{lemma}[Closed form for $q_k$]\label{lem:qk}
For all $u\in\R$,
\begin{align}
  q_0(u)&=\erf\left({u\over\sqrt2}\right),\label{eq:q0}\\
  q_k(u)&=2\varphi(u){\He_{k-1}(-u)\over\sqrt{k}},\qquad k\ge1,\label{eq:qk}
\end{align}
where $\varphi(u)=(2\pi)^{-1/2}e^{-u^2/2}$.
\end{lemma}

\begin{proof}
For $k=0$,
\[
  q_0(u)=\Prob[R>-u]-\Prob[R<-u]=\erf\left({u\over\sqrt2}\right).
\]
For $k\ge1$, orthogonality to constants gives
\[
  q_k(u)=2\int_{-u}^{\infty}\He_k(r)\varphi(r)\,dr.
\]
The orthonormal Hermite polynomials satisfy
\[
  {d\over dr}\left(\varphi(r)\He_{k-1}(r)\right)
  =-\sqrt{k}\,\varphi(r)\He_k(r),
\]
so integration from $-u$ to $\infty$ gives \eqref{eq:qk}.
\end{proof}

\begin{definition}[Two-dimensional coefficient integrals]\label{def:Cabk}
For $a,b,k\in\Nzero$, define
\begin{equation}\label{eq:C-abk}
  C_{a,b,k}
  =\E_{Z,X}\left[\He_a(Z)\He_b(X)
    q_k\left({Z+\eta \He_3(X)\over S}\right)\right],
\end{equation}
where $Z,X$ are independent standard Gaussians.  Equivalently,
\[
  C_{a,b,k}=\int_{\R^2}\He_a(z)\He_b(x)
  q_k\left({z+\eta \He_3(x)\over S}\right)\varphi(z)\varphi(x)\,dz\,dx.
\]
\end{definition}

The quantities $C_{a,b,k}$ are the only continuous integrals appearing in the coefficient formula.  Everything else is finite bookkeeping by degree.

\subsection{Hermite coefficients of the limiting thresholds}\label{subsec:threshold-hermite-coefficients}

For a multi-index $\beta=(\beta_d)_{d\in D}\in\Nzero^D$, write
\[
  |\beta|=\sum_{d\in D}\beta_d,
  \qquad
  \beta!=\prod_{d\in D}\beta_d!,
  \qquad
  \alpha^\beta=\prod_{d\in D}\alpha_d^{\beta_d}.
\]

\begin{proposition}[Hermite coefficients of the limiting thresholds]\label{prop:hermite-coefficients}
Let $f,g$ be the limiting threshold functions in Definition~\ref{def:limiting-model}.  Write their Hermite expansions in the tensor basis as
\[
  f=\sum_{a,b,\beta} A_{a,b,\beta}\,\He_a(Z)\He_b(X)\prod_{d\in D}\He_{\beta_d}(R_d),
\]
\[
  g=\sum_{a,b,\beta} B_{a,b,\beta}\,\He_a(Z)\He_b(X)\prod_{d\in D}\He_{\beta_d}(R_d).
\]
Then, for $k=|\beta|$,
\begin{equation}\label{eq:f-coeff}
  A_{a,b,\beta}=C_{a,b,k}\sqrt{k!\over \beta!}\,\alpha^\beta,
\end{equation}
while
\begin{equation}\label{eq:g-coeff}
  B_{a,b,\beta}=(-1)^b\prod_{d\in D}\sigma_d^{\beta_d}\,A_{a,b,\beta}.
\end{equation}
\end{proposition}

\begin{proof}
Set
\[
  T(Z,X)=Z+\eta \He_3(X),
  \qquad
  R_\alpha=\sum_{d\in D}\alpha_dR_d.
\]
Then
\[
  f=\sgn(T+SR_\alpha).
\]
Conditioning on $Z,X$, the coefficient of $\He_k(R_\alpha)$ in the $R_\alpha$ direction is
\[
  q_k\left({T(Z,X)\over S}\right).
\]
Taking the additional inner product against $\He_a(Z)\He_b(X)$ gives $C_{a,b,k}$.

The multivariate Hermite addition formula gives
\begin{equation}\label{eq:hermite-addition}
  \He_k\left(\sum_{d\in D}\alpha_dR_d\right)
  =\sum_{\substack{\beta\in\Nzero^D\\ |\beta|=k}}
  \sqrt{k!\over \beta!}\,\alpha^\beta
  \prod_{d\in D}\He_{\beta_d}(R_d).
\end{equation}
Combining the previous paragraph with \eqref{eq:hermite-addition} proves \eqref{eq:f-coeff}.

Finally,
\[
  g(z,x,(r_d))=f(z,-x,(\sigma_dr_d)_{d\in D}).
\]
Since $\He_b(-x)=(-1)^b\He_b(x)$ and $\He_{\beta_d}(\sigma_dr_d)=\sigma_d^{\beta_d}\He_{\beta_d}(r_d)$, the coefficient relation \eqref{eq:g-coeff} follows.
\end{proof}

\subsection{The degree coefficient formula}\label{subsec:degree-formula}

\begin{theorem}[Coefficient formula]\label{thm:coefficient-formula}
Let
\[
  H(t)=\sum_{m\ge1}b_m t^m
\]
be the limiting normalized correlation \eqref{eq:lim-H}.  Then
\begin{equation}\label{eq:general-bm}
  b_m={\pi\over2}
  \sum_{\substack{a,b\in\Nzero,\ \beta\in\Nzero^D\\ a+b+\sum_{d\in D}d\beta_d=m}}
  (-1)^b\prod_{d\in D}\sigma_d^{\beta_d}
  {k!\over \beta!}
  \prod_{d\in D}\alpha_d^{2\beta_d}
  C_{a,b,k}^2,
  \qquad k=|\beta|.
\end{equation}
Only odd $m$ occur.
\end{theorem}

\begin{proof}
Under the correlation model in Definition~\ref{def:limiting-model}, the Hermite covariance identity \eqref{eq:hermite-cov} contributes
\[
  t^a t^b\prod_{d\in D}(t^d)^{\beta_d}
  =t^{a+b+\sum_d d\beta_d}
\]
to the tensor basis element indexed by $(a,b,\beta)$.  Multiplying the $f$- and $g$-coefficients from Proposition~\ref{prop:hermite-coefficients} and summing over all indices of degree $m$ gives \eqref{eq:general-bm}.

The functions $f$ and $g$ are odd under simultaneous negation of all coordinates.  Hence their Hermite coefficients vanish unless $a+b+|\beta|$ is odd.  Since all degrees $d\in D$ are odd, $a+b+\sum_d d\beta_d$ has the same parity as $a+b+|\beta|$.  Thus only odd degrees appear.
\end{proof}

\subsection{The third/fifth specialization}\label{subsec:third-fifth-coefficients}

\begin{definition}[Third/fifth coefficient data]\label{def:third-fifth-coeff-data}
For the scheme $D=\{3,5\}$, write
\[
  \alpha={s_3\over S},\qquad \beta={s_5\over S},
  \qquad S=(s_3^2+s_5^2)^{1/2}.
\]
With the numerical parameters \eqref{eq:params},
\[
  S=0.345068689589145\ldots,
  \quad
  \alpha=0.988241617650167\ldots,
  \quad
  \beta=0.152900311131734\ldots .
\]
\end{definition}

For $D=\{3,5\}$, Theorem~\ref{thm:coefficient-formula} becomes
\begin{equation}\label{eq:35-bm}
  b_m={\pi\over2}
  \sum_{\substack{a,b,\beta_3,\beta_5\in\Nzero\\ a+b+3\beta_3+5\beta_5=m}}
  (-1)^{b+\beta_3}
  {k!\over \beta_3!\beta_5!}
  \alpha^{2\beta_3}\beta^{2\beta_5}
  C_{a,b,k}^2,
  \qquad k=\beta_3+\beta_5.
\end{equation}
This is the general weighted-degree formula.  The certification below uses the equivalent collapsed formula in Proposition~\ref{prop:collapsed-coefficients}.


\subsection{A collapsed formula for the third/fifth certificate}\label{subsec:collapsed-formula}

The interval certificate uses the following specialized form of the third/fifth coefficient formula.  It is equivalent to \eqref{eq:35-bm}, but it combines the three Gaussian coordinates $Z,R_3,R_5$ into one Gaussian direction before expanding.  This reduces the coefficient computation to one-dimensional threshold integrals and is the form used in Sections~\ref{sec:assembly} and~\ref{sec:formulas}.

\begin{definition}[Collapsed third/fifth data]\label{def:collapsed-data}
For the parameters \eqref{eq:params}, set
\[
  V=1+s_3^2+s_5^2,
  \qquad
  \vartheta={\eta\over\sqrt V},
\]
and define
\[
  F(w,x)=\sgn\bigl(w+\vartheta\He_3(x)\bigr).
\]
For $a,b\ge0$, define
\begin{equation}\label{eq:mathsfAab}
  \mathsf A_{a,b}=\E_{W,X}\bigl[\He_a(W)\He_b(X)F(W,X)\bigr],
\end{equation}
where $W,X$ are independent standard Gaussians.  Finally set
\begin{equation}\label{eq:rho-collapsed}
  \rho(t)={t-s_3^2t^3+s_5^2t^5\over V}.
\end{equation}
\end{definition}

\begin{proposition}[Collapsed coefficient formula]\label{prop:collapsed-coefficients}
For the third/fifth limiting model,
\begin{equation}\label{eq:H-collapsed}
  H(t)={\pi\over2}\sum_{a,b\ge0}\mathsf A_{a,b}^2\rho(t)^a(-t)^b.
\end{equation}
Consequently, for every $m\ge1$,
\begin{equation}\label{eq:bm-collapsed}
  b_m={\pi\over2}\sum_{a,b\ge0}(-1)^b\mathsf A_{a,b}^2\,[t^{m-b}]\rho(t)^a.
\end{equation}
Only terms with $a+b$ odd contribute.
\end{proposition}

\begin{proof}
Set
\[
  W={Z+s_3R_3+s_5R_5\over\sqrt V},
  \qquad
  \widetilde W={Z'-s_3R_3'+s_5R_5'\over\sqrt V}.
\]
Then $W$ and $\widetilde W$ are standard Gaussians and
\[
  \mathrm{corr}(W,\widetilde W)={t-s_3^2t^3+s_5^2t^5\over V}=\rho(t).
\]
Moreover
\[
  f=F(W,X),
  \qquad
  g'=F(\widetilde W,-X'),
\]
because $\He_3(-X')=-\He_3(X')$.  Expand
\[
  F(W,X)=\sum_{a,b\ge0}\mathsf A_{a,b}\He_a(W)\He_b(X).
\]
The Hermite covariance identity gives
\[
  \E[\He_a(W)\He_a(\widetilde W)]=\rho(t)^a,
  \qquad
  \E[\He_b(X)\He_b(-X')]=(-1)^b t^b.
\]
Multiplying the matching Hermite coefficients and summing proves \eqref{eq:H-collapsed}.  Reading off coefficients gives \eqref{eq:bm-collapsed}.  The parity statement follows from $F(-w,-x)=-F(w,x)$, which forces $\mathsf A_{a,b}=0$ unless $a+b$ is odd.
\end{proof}

\begin{remark}[One-dimensional form of \texorpdfstring{$\mathsf A_{a,b}$}{Aab}]
The coefficient $\mathsf A_{a,b}$ can be written using the same threshold coefficients $q_a$ from Definition~\ref{def:qk}:
\[
  \mathsf A_{a,b}=\E_X\bigl[\He_b(X)q_a(\vartheta\He_3(X))\bigr].
\]
This is the formula used in the interval computation of the coefficient head.
\end{remark}


==> old/simplifications_old.tex <==
\section{Preliminaries}

We first state Vitali's theorem, which lets us convert pointwise convergence to uniform convergence. See~\cite{schiff1993normal} for a reference. 

\begin{fact}[Vitali's convergence theorem]
Let \(h_1,h_2,\ldots\) be holomorphic functions on a connected open set
\(\Omega\). Suppose that:
\begin{enumerate}
    \item the sequence \((h_N)_{N\geq 1}\) is locally bounded on \(\Omega\); and
    \item \(h_N(z)\) converges for every \(z\) in some subset of \(\Omega\)
    having an accumulation point in \(\Omega\).
\end{enumerate}
Then \((h_N)_{N\geq 1}\) converges locally uniformly on \(\Omega\) to a
holomorphic function.
\end{fact}


\section{Limiting Krivine Schemes}

In this section, we extend classical Krivine schemes by allowing them to have arbitrary correlations among variables (up to some criteria). We will show that we can state asymptotic statements about regular Krivine schemes using this extended class of schemes, that we call \textit{limiting Krivine schemes}. This gives us analytic machinery for searching and analyzing limits of high dimensional schemes that were previously inaccessible via standard techniques. It is first instructive for us to start with a motivating example. 

\paragraph{Motivating example.}
Consider the two-dimensional classical Krivine rounding scheme
\[
f(X_1,X_2)=\operatorname{sgn}(X_1+\lambda X_2),
\qquad
g(Y_1,Y_2)=\operatorname{sgn}(y_1+\lambda y_2),
\]
where \(X_1,X_2,Y_1,Y_2\) are standard Gaussians, \(X_1\) is independent of \(X_2\), \(Y_1\) is independent of \(Y_2\), and
\[
\operatorname{corr}(X_1,Y_1)
=
\operatorname{corr}(X_2,Y_2)
=
t.
\]
In a classical Krivine scheme, every pair of corresponding coordinates has correlation \(t\). Suppose instead that we would like the first pair to have correlation \(t\), but the second pair to have correlation \(t^3\). To obtain this from a classical high-dimensional scheme, define
\[
U_N=\frac{1}{\sqrt N}\sum_{j=1}^N \mathrm{He}_3(X_{2,j}),
\qquad
V_N=\frac{1}{\sqrt N}\sum_{j=1}^N \mathrm{He}_3(Y_{2,j}),
\]
where the pairs \((X_{2,j},Y_{2,j})\) are independent standard Gaussian pairs with correlation \(t\). The Hermite identity gives
\[
\mathbb{E}[U_NV_N]
=
\mathbb{E}[\mathrm{He}_3(X_{2,1})\mathrm{He}_3(Y_{2,1})]
=
t^3.
\]
Moreover, by the central limit theorem, \((U_N,V_N)\) converges in distribution to a standard Gaussian pair \((U,V)\) with correlation \(t^3\). Thus, the classical rounding schemes
\[
F_N=\operatorname{sgn}(X_1+\lambda U_N),
\qquad
G_N=\operatorname{sgn}(Y_1+\lambda V_N)
\]
converge to the fixed-dimensional Gaussian rounding scheme
\[
f(X_1,U)=\operatorname{sgn}(X_1+\lambda U),
\qquad
g(Y_1,V)=\operatorname{sgn}(Y_1+\lambda V),
\]
in which the two coordinate pairs have correlations \(t\) and \(t^3\), respectively.

To use this construction, we need to carefully handle the following analytic hurdles:
\begin{enumerate}
    \item Pointwise convergence of the correlation functions must be strengthened to locally uniform convergence;
    \item An inverse-majorant $\gamma$-admissibility proved for the limiting scheme must remain valid for all sufficiently large finite-dimensional approximations.
\end{enumerate}

We now generalize this construction and prove both properties. First, we define the notion of allowable correlation maps.  
\begin{definition}[Allowable correlation map]
\label{def:allowable-correlation-map}
A function \(\rho:(-1,1)\to\mathbb{R}\) is an \emph{allowable correlation map}
if it admits an expansion
\[
\rho(t)
=
\sum_{\substack{d\geq 1\\ d\ \mathrm{odd}}} c_d t^d,
\qquad
\sum_{\substack{d\geq 1\\ d\ \mathrm{odd}}}|c_d|
\leq 1.
\]
\end{definition}

We can now state the definition of limiting Krivine schemes. 

\begin{definition}[Limiting Krivine Schemes]
A $k$-dimensional \emph{limiting Krivine scheme} is a tuple $\mathcal{S} = (f, g, \rho)$, where  \(f,g:\mathbb{R}^k\to\{-1,1\}\) are odd measurable functions and \(\rho = (\rho_1,\ldots,\rho_k)\) is a tuple of allowable correlation maps.  

The arcsine-normalized correlation function of this scheme is given by 
\[
H_{f, g, \rho}(t)
=
\frac{\pi}{2}\mathbb{E}[f(X)g(Y)].
\]
where \(X,Y\in\mathbb{R}^k\) are jointly Gaussian such that
\[
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij},
\qquad
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t).
\]
\end{definition}

\begin{remark}
    This is a generalization of the usual high dimensional Krivine schemes with $\rho_i(t) = t$ for all $i$. 

    At this stage, \(H_{f, g, \rho}\) is defined only on \((-1,1)\); in particular, we do not assume that it extends holomorphically to the strip associated with classical Krivine schemes.
\end{remark}

The motivation for this definition is that every limiting Krivine scheme can be approximated arbitrarily well by ordinary finite-dimensional Krivine schemes, as we will show below. This allows us to use the usual projection scheme to round the vectors, and get the inverse-majorant machinery for free. We make this precise in the following theorem.  

\begin{theorem}[Finite-dimensional approximation of limiting schemes]
Let \(\mathcal S=(f,g,\rho_1,\ldots,\rho_k)\) be a limiting Krivine scheme. Then there exists a sequence of ordinary finite-dimensional Krivine schemes
\(
\mathcal S_1,\mathcal S_2,\ldots,
\)
of increasing dimension, whose correlation functions $H_{\mathcal S_1}, H_{\mathcal S_2}, \ldots$ converge to the correlation function $H_{\mathcal S}$ of \(\mathcal S\), uniformly on every compact subset of \((-1,1)\).
\end{theorem}

We dedicate the rest of the section to proving this theorem. First, we prove an equivalence condition on allowability of a function. 

\begin{lemma}[Allowable function criteria]
A map \(\rho\) is allowable if and only if there are odd functions
\(p,q: \R^3 \to \R\), such that
\(\|p\|_2=\|q\|_2=1\) and
\[
\rho(t)=\mathbb{E}[p(U)q(V)],
\]
where \(U,V\in\mathbb{R}^m\) are standard Gaussian vectors with
\(\mathbb{E}[U_iV_j]=t\delta_{ij}\).
\end{lemma}

\begin{proof}
Suppose first that \(p\) and \(q\) are odd and have \(L_2\)-norm one. Write
their Hermite expansions by degree as
\[
p=\sum_{\substack{d\geq 1\\ d\text{ odd}}}p_d,
\qquad
q=\sum_{\substack{d\geq 1\\ d\text{ odd}}}q_d.
\]
Here \(p_d\) and \(q_d\) are the degree-\(d\) Hermite components.

Different Hermite degrees are orthogonal, while degree \(d\) contributes a
factor \(t^d\). Hence
\[
\mathbb{E}[p(U)q(V)]
=
\sum_{\substack{d\geq 1\\ d\text{ odd}}}
\langle p_d,q_d\rangle t^d.
\]
Set \(c_d=\langle p_d,q_d\rangle\). Then
\[
\sum_d|c_d|
\leq
\sum_d\|p_d\|_2\|q_d\|_2
\leq
\left(\sum_d\|p_d\|_2^2\right)^{1/2}
\left(\sum_d\|q_d\|_2^2\right)^{1/2}
=
1.
\]
Thus the resulting correlation map is allowable.

Conversely, suppose that
\[
\rho(t)=\sum_{d\text{ odd}}c_dt^d,
\qquad
s:=\sum_{d\text{ odd}}|c_d|\leq 1.
\]
For \(x=(x_1,x_2,x_3)\in\mathbb{R}^3\), define
\[
p(x)
=
\sum_{d\text{ odd}}
\sqrt{|c_d|}\operatorname{He}_d(x_1)
+
\sqrt{1-s}\,x_2
\]
and
\[
q(x)
=
\sum_{d\text{ odd}}
\operatorname{sgn}(c_d)\sqrt{|c_d|}
\operatorname{He}_d(x_1)
+
\sqrt{1-s}\,x_3.
\]
Both functions are odd. Orthogonality gives \(\|p\|_2=\|q\|_2=1\).

Let \(U,V\in\mathbb{R}^3\) be standard Gaussian vectors with
\(\mathbb{E}[U_iV_j]=t\delta_{ij}\). The terms involving \(U_2\) and \(V_3\)
have zero cross-correlation. Therefore
\[
\mathbb{E}[p(U)q(V)]
=
\sum_{d\text{ odd}}c_dt^d
=
\rho(t).
\]
\end{proof}

We are now ready to prove our theorem, which follows as a direct corollary of the stronger statement we prove below. 

\begin{theorem}[Finite-dimensional approximation of limiting schemes]
Let \((f,g,\rho_1,\ldots,\rho_k)\) be a limiting Krivine scheme, and suppose
that the discontinuity sets of \(f\) and \(g\) have Gaussian measure zero.
Then its correlation function extends holomorphically to the unit disk and is
the locally uniform limit there of the correlation functions of ordinary
finite-dimensional Krivine schemes.
\end{theorem}

\begin{proof}
By the above lemma, for each \(i\in\{1,\ldots,k\}\), there exist odd measurable functions 
\(
p_i,q_i:\mathbb{R}^3\to\mathbb{R}
\)
with $\|p\|_2 = \|q\|_2 = 1$ such that, whenever \(U,V\in\mathbb{R}^3\) are joint standard Gaussian vectors with
\(
\mathbb{E}[U_aV_b]=t\delta_{ab},
\)
we have
\[
\mathbb{E}[p_i(U)q_i(V)]
=
\rho_i(t).
\]
We combine these functions into vector-valued maps. Write
\(u\in\mathbb{R}^{3k}\) in \(k\) blocks as
\[
u=\bigl(u^{(1)},\ldots,u^{(k)}\bigr),
\qquad
u^{(i)}\in\mathbb{R}^3,
\]
and define
\[
P(u)
=
\bigl(
p_1(u^{(1)}),\ldots,p_k(u^{(k)})
\bigr),
\]
\[
Q(u)
=
\bigl(
q_1(u^{(1)}),\ldots,q_k(u^{(k)})
\bigr).
\]
For each positive integer \(N\), define functions on
\(\bigl(\mathbb{R}^{3k}\bigr)^N\) by
\[
F_N(u_1,\ldots,u_N)
=
f\left(
\frac{1}{\sqrt{N}}\sum_{r=1}^N P(u_r)
\right)
\]
and
\[
G_N(v_1,\ldots,v_N)
=
g\left(
\frac{1}{\sqrt{N}}\sum_{r=1}^N Q(v_r)
\right).
\]
Since \(P\), \(Q\), \(f\), and \(g\) are odd, the functions \(F_N\) and
\(G_N\) are odd. They therefore define an ordinary finite-dimensional
Krivine scheme.

Let \(H_N\) denote the correlation function of this scheme. Fix
\(t\in(-1,1)\), and let
\[
(U_1,V_1),\ldots,(U_N,V_N)
\]
be independent pairs of standard Gaussian vectors in \(\mathbb{R}^{3k}\)
satisfying
\[
\mathbb{E}[(U_r)_a(V_r)_b]
=
t\delta_{ab}.
\]
Define
\[
A_N
=
\frac{1}{\sqrt{N}}\sum_{r=1}^N P(U_r),
\qquad
B_N
=
\frac{1}{\sqrt{N}}\sum_{r=1}^N Q(V_r).
\]
By the definition of the correlation function,
\[
H_N(t)
=
\frac{\pi}{2}\,
\mathbb{E}\bigl[f(A_N)g(B_N)\bigr].
\]

\begin{claim}
As \(N \rightarrow \infty\), we have \[
(A_N,B_N)
\xrightarrow{d}
(X,Y),
\]
where \((X,Y)\) is jointly Gaussian and satisfies
\[
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij},
\qquad
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t).
\]
\end{claim}

\begin{claimproof}
The random vectors
\[
\bigl(P(U_r),Q(V_r)\bigr)\in\mathbb{R}^{2k}
\]
are independent, identically distributed, and centered. Because the
\(k\) Gaussian blocks are independent, their covariance matrix is
\[
\begin{pmatrix}
I_k & D(t)\\
D(t) & I_k
\end{pmatrix},
\qquad
D(t)
=
\operatorname{diag}\bigl(
\rho_1(t),\ldots,\rho_k(t)
\bigr).
\]
By the multivariate central limit theorem, we have
\(
(A_N,B_N)
\xrightarrow[N\to\infty]{d}
(X,Y),
\)
where \((X,Y)\) is jointly Gaussian satisfying
\(
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij}\) and 
\(
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t),
\)
as desired. 
\end{claimproof}

Returning to the proof of the theorem, since the function
\(
(x,y)\longmapsto f(x)g(y)
\)
 is bounded and has discontinuity set with measure 0, it follows that
\[
\mathbb{E}\bigl[f(X_N)g(Y_N)\bigr]
\longrightarrow
\mathbb{E}\bigl[f(X(t))g(Y(t))\bigr].
\]
Consequently,
\[
H_N(t)\longrightarrow H(t)
\]
for every \(t\in(-1,1)\), where
\[
H(t)
=
\frac{\pi}{2}\,
\mathbb{E}\bigl[f(X(t))g(Y(t))\bigr]
\]
is the correlation function of the limiting scheme.

It remains to convert this pointwise convergence to locally uniform
convergence on the unit disk. For each \(N\), the Hermite expansions of
\(F_N\) and \(G_N\) give a holomorphic extension of \(H_N\) to
\[
\mathbb{D}
=
\{z\in\mathbb{C}:|z|<1\}.
\]
More explicitly, if
\[
F_N=\sum_{\alpha}\widehat{F_N}(\alpha)\operatorname{He}_{\alpha},
\qquad
G_N=\sum_{\alpha}\widehat{G_N}(\alpha)\operatorname{He}_{\alpha},
\]
then
\[
H_N(z)
=
\frac{\pi}{2}
\sum_{\alpha}
\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)z^{|\alpha|}.
\]
For \(z\) in the unit disk, the Cauchy--Schwarz inequality gives
\[
\begin{aligned}
|H_N(z)|
&\leq
\frac{\pi}{2}
\sum_{\alpha}
\bigl|
\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)
\bigr|
|z|^{|\alpha|} \\
&\leq
\frac{\pi}{2}
\left(
\sum_{\alpha}
|\widehat{F_N}(\alpha)|^2
\right)^{1/2}
\left(
\sum_{\alpha}
|\widehat{G_N}(\alpha)|^2
\right)^{1/2} \\
&\leq
\frac{\pi}{2}
\|F_N\|_2\|G_N\|_2
=
\frac{\pi}{2}.
\end{aligned}
\]
Here the second inequality uses \(|z|<1\), and the third follows from
the orthonormality of the Hermite polynomials.
% For \(z\in\mathbb{D}\), the Cauchy--Schwarz inequality and Parseval's identity
% give
% \[
% \begin{aligned}
% |H_N(z)|
% &\leq
% \frac{\pi}{2}
% \sum_{\alpha}
% \bigl|\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)\bigr|
% |z|^{|\alpha|} \\
% &\leq
% \frac{\pi}{2}
% \left(
% \sum_{\alpha}
% |\widehat{F_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2}
% \left(
% \sum_{\alpha}
% |\widehat{G_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2} \\
% &\leq
% \frac{\pi}{2}\|F_N\|_2\|G_N\|_2
% =
% \frac{\pi}{2}.
% \end{aligned}
% \]
Thus, the family \((H_N)_{N\geq 1}\) is locally bounded on \(\mathbb{D}\).
Since it converges pointwise on the interval \((-1,1)\), which has an
accumulation point in \(\mathbb{D}\). Vitali's theorem implies that
\((H_N)\) converges locally uniformly on \(\mathbb{D}\) to a holomorphic
function. On \((-1,1)\), this function agrees with \(H\). It is therefore
the holomorphic extension of the correlation function of the limiting
scheme.
\end{proof}

\begin{corollary}[Upper bound from a limiting Krivine scheme]
Let
\(
\mathcal{S}=(f,g,\rho_1,\ldots,\rho_k)
\)
be a limiting Krivine scheme. Let \(H\) be its correlation
function. Suppose that \(H'(0)\neq 0\), so that \(H\) has a local holomorphic inverse
at the origin. Write
\[
H^{-1}(z)
=
\sum_{j=0}^{\infty}a_{2j+1}z^{2j+1},
\]
and define its majorant by
\[
M(r)
=
\sum_{j=0}^{\infty}|a_{2j+1}|r^{2j+1}.
\]
If there exists \(\gamma>0\), within the radius of convergence of
\(H^{-1}\), such that
\(
M(\gamma)=1,
\)
then
\(
K_G
\leq
\frac{\pi}{2\gamma}.
\)
\end{corollary}
% \begin{theorem}[Finite-dimensional approximation of limiting schemes]
% Let
% \[
% \mathcal{S}=(f,g,\rho_1,\ldots,\rho_k)
% \]
% be a limiting Krivine scheme, and suppose that the discontinuity sets of
% \(f\) and \(g\) have Gaussian measure zero. Then the correlation function of
% \(\mathcal{S}\) extends holomorphically to the unit disk and is the locally
% uniform limit there of the correlation functions of ordinary
% finite-dimensional Krivine schemes.
% \end{theorem}

% \begin{proof}
% For each \(i\in\{1,\ldots,k\}\), there exist odd functions
% \(
% p_i,q_i: \R^3 \to \R 
% \)
% such that
% \(
% \|p_i\|_2=\|q_i\|_2=1
% \)
% and
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)]
% \]
% for every \(t\in(-1,1)\), where \(U,V\in\mathbb{R}^{3}\) are standard
% Gaussian vectors satisfying
% \[
% \mathbb{E}[U_aV_b]=t\delta_{ab}.
% \]

% For each positive integer \(N\), identify
% \[
% \mathbb{R}^{3N}
% =
% \prod_{i=1}^k \bigl(\mathbb{R}^{3}\bigr)^N.
% \]
% Thus, a point \(u\in\mathbb{R}^{3N}\) can be written as
% \[
% u=(u_{i,r})_{\substack{1\leq i\leq k\\1\leq r\leq N}},
% \qquad
% u_{i,r}\in\mathbb{R}^{3}.
% \]
% Define
% \[
% F_N(u)
% =
% f\left(
% \frac{1}{\sqrt{N}}\sum_{r=1}^N p_1(u_{1,r}),
% \ldots,
% \frac{1}{\sqrt{N}}\sum_{r=1}^N p_k(u_{k,r})
% \right).
% \]
% Similarly, for
% \[
% v=(v_{i,r})_{\substack{1\leq i\leq k\\1\leq r\leq N}}
% \in\mathbb{R}^{3N},
% \]
% define
% \[
% G_N(v)
% =
% g\left(
% \frac{1}{\sqrt{N}}\sum_{r=1}^N q_1(v_{1,r}),
% \ldots,
% \frac{1}{\sqrt{N}}\sum_{r=1}^N q_k(v_{k,r})
% \right).
% \]
% Because \(p_i,q_i,f\), and \(g\) are odd, both \(F_N\) and \(G_N\) are odd.
% Hence \((F_N,G_N)\) is an ordinary finite-dimensional Krivine scheme.

% Let \(H_N\) denote its correlation function. Fix \(t\in(-1,1)\), and let
% \(U^{(N)},V^{(N)}\in\mathbb{R}^{3N}\) be standard Gaussian vectors satisfying
% \[
% \mathbb{E}\bigl[U^{(N)}_aV^{(N)}_b\bigr]
% =
% t\delta_{ab}.
% \]
% Write these vectors in blocks as
% \[
% U^{(N)}=(U_{i,r})_{i,r},
% \qquad
% V^{(N)}=(V_{i,r})_{i,r},
% \]
% where the pairs \((U_{i,r},V_{i,r})\) are independent over \(i\) and \(r\),
% and each pair is a standard Gaussian pair in \(\mathbb{R}^3\) satisfying
% \[
% \mathbb{E}\bigl[(U_{i,r})_a(V_{i,r})_b\bigr]
% =
% t\delta_{ab}.
% \]

% Define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{r=1}^N p_i(U_{i,r}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{r=1}^N q_i(V_{i,r}),
% \]
% and set
% \[
% X_N=(X_{1,N},\ldots,X_{k,N}),
% \qquad
% Y_N=(Y_{1,N},\ldots,Y_{k,N}).
% \]
% Then
% \[
% H_N(t)
% =
% \frac{\pi}{2}\,
% \mathbb{E}\bigl[f(X_N)g(Y_N)\bigr].
% \]

% For each \(r\), consider the \(2k\)-dimensional random vector
% \[
% Z_r
% =
% \bigl(
% p_1(U_{1,r}),\ldots,p_k(U_{k,r}),
% q_1(V_{1,r}),\ldots,q_k(V_{k,r})
% \bigr).
% \]
% The vectors \(Z_1,Z_2,\ldots\) are independent and identically distributed,
% and
% \[
% (X_N,Y_N)
% =
% \frac{1}{\sqrt{N}}\sum_{r=1}^N Z_r.
% \]
% Since the functions \(p_i\) and \(q_i\) are odd, all coordinates of \(Z_r\)
% have mean zero. Moreover,
% \[
% \mathbb{E}[X_{i,N}X_{j,N}]
% =
% \mathbb{E}[Y_{i,N}Y_{j,N}]
% =
% \delta_{ij}
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{j,N}]
% =
% \delta_{ij}\rho_i(t).
% \]
% Indeed, coordinates with different values of \(i\) are independent, while
% for \(i=j\),
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]

% The multivariate central limit theorem therefore gives
% \[
% (X_N,Y_N)
% \xrightarrow[N\to\infty]{d}
% (X(t),Y(t)),
% \]
% where \((X(t),Y(t))\) is jointly Gaussian and satisfies
% \[
% \mathbb{E}[X_i(t)X_j(t)]
% =
% \mathbb{E}[Y_i(t)Y_j(t)]
% =
% \delta_{ij},
% \qquad
% \mathbb{E}[X_i(t)Y_j(t)]
% =
% \delta_{ij}\rho_i(t).
% \]
% This is precisely the Gaussian pair appearing in the definition of the
% limiting scheme.

% The function
% \[
% (x,y)\longmapsto f(x)g(y)
% \]
% is bounded, and its discontinuity set is contained in
% \[
% \bigl(\operatorname{Disc}(f)\times\mathbb{R}^k\bigr)
% \cup
% \bigl(\mathbb{R}^k\times\operatorname{Disc}(g)\bigr).
% \]
% Because \(X(t)\) and \(Y(t)\) are standard Gaussian vectors, the assumed
% Gaussian-nullity of the discontinuity sets implies that this union has
% probability zero under the law of \((X(t),Y(t))\). It follows that
% \[
% \mathbb{E}\bigl[f(X_N)g(Y_N)\bigr]
% \longrightarrow
% \mathbb{E}\bigl[f(X(t))g(Y(t))\bigr].
% \]
% Consequently,
% \[
% H_N(t)\longrightarrow H(t)
% \]
% for every \(t\in(-1,1)\), where
% \[
% H(t)
% =
% \frac{\pi}{2}\,
% \mathbb{E}\bigl[f(X(t))g(Y(t))\bigr]
% \]
% is the correlation function of the limiting scheme.

% It remains to upgrade this pointwise convergence to locally uniform
% convergence on the unit disk. For each \(N\), the Hermite expansions of
% \(F_N\) and \(G_N\) give a holomorphic extension of \(H_N\) to
% \[
% \mathbb{D}
% =
% \{z\in\mathbb{C}:|z|<1\}.
% \]
% More explicitly, if
% \[
% F_N=\sum_{\alpha}\widehat{F_N}(\alpha)\operatorname{He}_{\alpha},
% \qquad
% G_N=\sum_{\alpha}\widehat{G_N}(\alpha)\operatorname{He}_{\alpha},
% \]
% then
% \[
% H_N(z)
% =
% \frac{\pi}{2}
% \sum_{\alpha}
% \widehat{F_N}(\alpha)\widehat{G_N}(\alpha)z^{|\alpha|}.
% \]
% For \(z\in\mathbb{D}\), the Cauchy--Schwarz inequality and Parseval's identity
% give
% \[
% \begin{aligned}
% |H_N(z)|
% &\leq
% \frac{\pi}{2}
% \sum_{\alpha}
% \bigl|\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)\bigr|
% |z|^{|\alpha|} \\
% &\leq
% \frac{\pi}{2}
% \left(
% \sum_{\alpha}
% |\widehat{F_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2}
% \left(
% \sum_{\alpha}
% |\widehat{G_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2} \\
% &\leq
% \frac{\pi}{2}\|F_N\|_2\|G_N\|_2
% =
% \frac{\pi}{2}.
% \end{aligned}
% \]
% Thus, the family \((H_N)_{N\geq 1}\) is locally bounded on \(\mathbb{D}\).
% Since it converges pointwise on the interval \((-1,1)\), which has an
% accumulation point in \(\mathbb{D}\), Vitali's theorem implies that
% \((H_N)\) converges locally uniformly on \(\mathbb{D}\) to a holomorphic
% function. On \((-1,1)\), this function agrees with \(H\). It is therefore
% the holomorphic extension of the correlation function of the limiting
% scheme.
% \end{proof}


% \begin{lemma}
% Let \(\rho_1,\ldots,\rho_k\) be allowable correlation functions. 
% For every \(t\in(-1,1)\), there is a sequence \(\left\{\left(X^{(N)},Y^{(N)}\right)\right\}_{N \ge 1}\) of pairs of finite-dimensional random vectors in \(\mathbb{R}^k\), constructed from coordinatewise
% \(t\)-correlated Gaussians, such that
% \[
% \left(X^{(N)},Y^{(N)}\right)
% \longrightarrow
% (X,Y), \qquad N \rightarrow \infty 
% \]
% where \(X,Y \in \R^k\) are standard Gaussian vectors satisfying
% \[
% \mathbb{E}[X_iY_j]
% =
% \delta_{ij}\rho_i(t).
% \]
% \end{lemma}

% \begin{proof}
% For each \(i\), choose odd variance-one functions \(p_i,q_i\) such that
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)].
% \]
% For \(N\geq 1\), define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}),
% \]
% where the pairs \((U_{i,j},V_{i,j})\) are independent over \(i\) and \(j\),
% and each pair has coordinatewise correlation \(t\).

% For every \(i\),
% \[
% \mathbb{E}[X_{i,N}^2]
% =
% \mathbb{E}[Y_{i,N}^2]
% =
% 1
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]
% Coordinates with different values of \(i\) are independent. The multivariate
% central limit theorem therefore gives the claimed convergence.
% \end{proof}

% For example, taking \(p=q=\operatorname{He}_3\) gives the correlation \(t^3\),
% while taking \(p=q=\operatorname{He}_5\) gives \(t^5\). The theorem allows
% arbitrary allowable correlations in place of these individual powers.


% \begin{theorem}
% Suppose that the discontinuity sets of \(f\) and \(g\) have Gaussian measure
% zero. Then the correlation function of a limiting Krivine scheme is the locally
% uniform limit on the unit disk of correlation functions of ordinary
% finite-dimensional Krivine schemes.
% \end{theorem}

% \begin{proof}
% For each \(i\), choose odd variance-one functions \(p_i,q_i\) such that
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)].
% \]
% For \(N\geq 1\), define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}),
% \]
% where the pairs \((U_{i,j},V_{i,j})\) are independent over \(i\) and \(j\),
% and each pair has coordinatewise correlation \(t\).

% For every \(i\),
% \[
% \mathbb{E}[X_{i,N}^2]
% =
% \mathbb{E}[Y_{i,N}^2]
% =
% 1
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]
% Coordinates with different values of \(i\) are independent. By the multivariate central limit theorem, this implies that 


% Define finite-dimensional rounding functions by
% \[
% f_N
% =
% f(X_{1,N},\ldots,X_{k,N}),
% \qquad
% g_N
% =
% g(Y_{1,N},\ldots,Y_{k,N}).
% \]
% Since the functions \(p_i,q_i,f,g\) are odd, the functions \(f_N\) and \(g_N\)
% are odd. They therefore define ordinary finite-dimensional Krivine schemes.

% Let
% \[
% H_N(t)
% =
% \frac{\pi}{2}\mathbb{E}[f_Ng_N]
% \]
% be their correlation functions. For every fixed \(t\in(-1,1)\), the previous
% theorem gives
% \[
% \bigl(X^{(N)},Y^{(N)}\bigr)
% \Longrightarrow
% (X,Y).
% \]
% The discontinuity assumption then implies
% \[
% H_N(t)\longrightarrow H(t).
% \]

% For each \(N\), the Hermite expansion of \(f_N\) and \(g_N\) shows that \(H_N\)
% is holomorphic on the unit disk and satisfies
% \[
% |H_N(z)|
% \leq
% \frac{\pi}{2}.
% \]
% The family \((H_N)\) is therefore locally bounded. Since it converges pointwise
% on the real interval \((-1,1)\), Vitali's theorem gives locally uniform
% convergence on the unit disk.
% \end{proof}




% \section{Limiting Krivine Schemes}

% The construction in this paper starts from a simple observation. A normalized
% average of degree-\(d\) Hermite polynomials converges to a Gaussian coordinate,
% while its correlation with the corresponding coordinate on the other side is
% \(t^d\). The degrees \(3\) and \(5\) used in our construction therefore produce
% the correlations \(t^3\) and \(t^5\).

% In this section, we first determine which correlation functions can be produced
% in this way. We then use them to define limiting Krivine schemes and show that
% these limiting schemes arise from ordinary finite-dimensional Krivine schemes.

% \subsection{Correlation functions}

% Let \((\operatorname{He}_d)_{d\geq 0}\) denote the orthonormal probabilist
% Hermite polynomials. If \(U,V\) are standard Gaussians with correlation \(t\),
% then
% \[
% \mathbb{E}
% \left[
% \operatorname{He}_d(U)\operatorname{He}_e(V)
% \right]
% =
% \mathbf{1}_{\{d=e\}}t^d.
% \]

% Thus a degree-\(d\) Hermite function produces the correlation \(t^d\). More
% generally, suppose that \(p\) and \(q\) are odd functions of a standard Gaussian
% vector. Writing their Hermite expansions by degree suggests that their
% correlation must have the form
% \[
% \sum_{\substack{d\geq 1\\ d\text{ odd}}} c_dt^d.
% \]
% Cauchy--Schwarz will force \(\sum_d |c_d|\leq 1\). This motivates the following
% definition.

% \begin{definition}
% A function \(\rho:(-1,1)\to\mathbb{R}\) is an allowable correlation function
% if
% \[
% \rho(t)
% =
% \sum_{\substack{d\geq 1\\ d\text{ odd}}}c_dt^d
% \qquad\text{and}\qquad
% \sum_{\substack{d\geq 1\\ d\text{ odd}}}|c_d|
% \leq 1.
% \]
% \end{definition}

% The coefficient condition implies that \(|\rho(t)|\leq |t|\) for
% \(t\in(-1,1)\). In particular, \(\rho(t)\in[-1,1]\). The functions \(t\),
% \(t^3\), and \(t^5\) are the simplest examples.

% The next theorem shows that this is exactly the class produced by odd Gaussian
% functions.

% \begin{theorem}
% A function \(\rho\) is allowable if and only if there are odd functions
% \(p,q\in L_2(\gamma_m)\), for some \(m\), such that
% \(\|p\|_2=\|q\|_2=1\) and
% \[
% \rho(t)=\mathbb{E}[p(U)q(V)],
% \]
% where \(U,V\in\mathbb{R}^m\) are standard Gaussian vectors with
% \(\mathbb{E}[U_iV_j]=t\delta_{ij}\).
% \end{theorem}

% \begin{proof}
% Suppose first that \(p\) and \(q\) are odd and have \(L_2\)-norm one. Write
% their Hermite expansions by degree as
% \[
% p=\sum_{\substack{d\geq 1\\ d\text{ odd}}}p_d,
% \qquad
% q=\sum_{\substack{d\geq 1\\ d\text{ odd}}}q_d.
% \]
% Here \(p_d\) and \(q_d\) are the degree-\(d\) Hermite components.

% Different Hermite degrees are orthogonal, while degree \(d\) contributes a
% factor \(t^d\). Hence
% \[
% \mathbb{E}[p(U)q(V)]
% =
% \sum_{\substack{d\geq 1\\ d\text{ odd}}}
% \langle p_d,q_d\rangle t^d.
% \]
% Set \(c_d=\langle p_d,q_d\rangle\). Then
% \[
% \sum_d|c_d|
% \leq
% \sum_d\|p_d\|_2\|q_d\|_2
% \leq
% \left(\sum_d\|p_d\|_2^2\right)^{1/2}
% \left(\sum_d\|q_d\|_2^2\right)^{1/2}
% =
% 1.
% \]
% Thus the resulting correlation function is allowable.

% Conversely, suppose that
% \[
% \rho(t)=\sum_{d\text{ odd}}c_dt^d,
% \qquad
% s:=\sum_{d\text{ odd}}|c_d|\leq 1.
% \]
% For \(x=(x_1,x_2,x_3)\in\mathbb{R}^3\), define
% \[
% p(x)
% =
% \sum_{d\text{ odd}}
% \sqrt{|c_d|}\operatorname{He}_d(x_1)
% +
% \sqrt{1-s}\,x_2
% \]
% and
% \[
% q(x)
% =
% \sum_{d\text{ odd}}
% \operatorname{sgn}(c_d)\sqrt{|c_d|}
% \operatorname{He}_d(x_1)
% +
% \sqrt{1-s}\,x_3.
% \]
% Both functions are odd. Orthogonality gives \(\|p\|_2=\|q\|_2=1\).

% Let \(U,V\in\mathbb{R}^3\) be standard Gaussian vectors with
% \(\mathbb{E}[U_iV_j]=t\delta_{ij}\). The terms involving \(U_2\) and \(V_3\)
% have zero cross-correlation. Therefore
% \[
% \mathbb{E}[p(U)q(V)]
% =
% \sum_{d\text{ odd}}c_dt^d
% =
% \rho(t).
% \]
% \end{proof}

% If the same function is used on both sides, then the coefficients are
% nonnegative. Indeed, if \(\rho(t)=\mathbb{E}[p(U)p(V)]\), then
% \[
% \rho(t)=\sum_{d\text{ odd}}\|p_d\|_2^2t^d.
% \]
% Thus \(c_d\geq 0\) and \(\sum_dc_d=1\). Allowing different functions on the two
% sides gives the signed coefficients in the theorem.


% \subsection{Central limit realization}

% We now explain why allowable correlation functions occur as limits of ordinary
% finite-dimensional Gaussian constructions. The idea is the same as in the
% degree-\(3\) and degree-\(5\) averages used in this paper: take many independent
% copies of the functions \(p\) and \(q\), and normalize their sums.

% \begin{theorem}
% Let \(\rho_1,\ldots,\rho_k\) be allowable correlation functions. For every
% \(t\in(-1,1)\), there are finite-dimensional random vectors
% \(X^{(N)},Y^{(N)}\in\mathbb{R}^k\), constructed from coordinatewise
% \(t\)-correlated Gaussian inputs, such that
% \[
% \bigl(X^{(N)},Y^{(N)}\bigr)
% \Longrightarrow
% (X,Y),
% \]
% where \(X,Y\) are standard Gaussian vectors satisfying
% \[
% \mathbb{E}[X_iY_j]
% =
% \delta_{ij}\rho_i(t).
% \]
% \end{theorem}

% \begin{proof}
% For each \(i\), choose odd variance-one functions \(p_i,q_i\) such that
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)].
% \]
% For \(N\geq 1\), define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}),
% \]
% where the pairs \((U_{i,j},V_{i,j})\) are independent over \(i\) and \(j\),
% and each pair has coordinatewise correlation \(t\).

% For every \(i\),
% \[
% \mathbb{E}[X_{i,N}^2]
% =
% \mathbb{E}[Y_{i,N}^2]
% =
% 1
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]
% Coordinates with different values of \(i\) are independent. The multivariate
% central limit theorem therefore gives the claimed convergence.
% \end{proof}

% For example, taking \(p=q=\operatorname{He}_3\) gives the correlation \(t^3\),
% while taking \(p=q=\operatorname{He}_5\) gives \(t^5\). The theorem allows
% arbitrary allowable correlations in place of these individual powers.

% \subsection{Limiting schemes}

% We can now package several allowable correlations into a Krivine scheme. The
% only change from the usual definition is that the \(i\)-th pair of Gaussian
% coordinates has correlation \(\rho_i(t)\), rather than \(t\).

% \begin{definition}
% A limiting Krivine scheme consists of odd measurable functions
% \(f,g:\mathbb{R}^k\to\{-1,1\}\) and allowable correlation functions
% \(\rho_1,\ldots,\rho_k\).

% For \(t\in(-1,1)\), let \(X,Y\in\mathbb{R}^k\) be jointly Gaussian with
% \[
% \mathbb{E}[X_iX_j]
% =
% \mathbb{E}[Y_iY_j]
% =
% \delta_{ij},
% \qquad
% \mathbb{E}[X_iY_j]
% =
% \delta_{ij}\rho_i(t).
% \]
% The correlation function of the scheme is
% \[
% H(t)
% =
% \frac{\pi}{2}\mathbb{E}[f(X)g(Y)].
% \]
% \end{definition}

% The usual Krivine scheme is the special case
% \(\rho_1(t)=\cdots=\rho_k(t)=t\). The limiting scheme used in this paper has
% correlations
% \[
% (t,t,t^3,t^5).
% \]

% The point of the definition is that these limiting objects do not enlarge the
% theory artificially. They are limits of ordinary finite-dimensional Krivine
% schemes.

% \begin{theorem}
% Suppose that the discontinuity sets of \(f\) and \(g\) have Gaussian measure
% zero. Then the correlation function of a limiting Krivine scheme is the locally
% uniform limit on the unit disk of correlation functions of ordinary
% finite-dimensional Krivine schemes.
% \end{theorem}

% \begin{proof}
% For each \(\rho_i\), choose functions \(p_i,q_i\) as above and form the
% normalized sums
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}).
% \]
% Define finite-dimensional rounding functions by
% \[
% f_N
% =
% f(X_{1,N},\ldots,X_{k,N}),
% \qquad
% g_N
% =
% g(Y_{1,N},\ldots,Y_{k,N}).
% \]
% Since the functions \(p_i,q_i,f,g\) are odd, the functions \(f_N\) and \(g_N\)
% are odd. They therefore define ordinary finite-dimensional Krivine schemes.

% Let
% \[
% H_N(t)
% =
% \frac{\pi}{2}\mathbb{E}[f_Ng_N]
% \]
% be their correlation functions. For every fixed \(t\in(-1,1)\), the previous
% theorem gives
% \[
% \bigl(X^{(N)},Y^{(N)}\bigr)
% \Longrightarrow
% (X,Y).
% \]
% The discontinuity assumption then implies
% \[
% H_N(t)\longrightarrow H(t).
% \]

% For each \(N\), the Hermite expansion of \(f_N\) and \(g_N\) shows that \(H_N\)
% is holomorphic on the unit disk and satisfies
% \[
% |H_N(z)|
% \leq
% \frac{\pi}{2}.
% \]
% The family \((H_N)\) is therefore locally bounded. Since it converges pointwise
% on the real interval \((-1,1)\), Vitali's theorem gives locally uniform
% convergence on the unit disk.
% \end{proof}

% The boundary assumption is automatic for the threshold functions used in this
% paper. It can also be removed for general odd measurable functions by a
% standard approximation argument.

==> paper/ai_paper_abstract.tex <==
\abstract{

AI agents are increasingly used in mathematics research, but it is often unclear how to use them effectively.
Towards this, we present an extensive case study of how AI was used to improve bounds on the Grothendieck constant $K_G$, which captures the hardness between combinatorial problems and their continuous relaxations.
Specifically, while the precise value of $K_G$ is not known, we recently tightened the best known bounds to
\[
    \frac{6\pi}{11}
    \;\le\;
    K_G
    \;\le\;
    \frac{\pi}{2\log(1+\sqrt2)} - 10^{-4}.
\]
Crucially, these improvements were achieved using an AI research system that could arrive at insights deemed novel by domain experts.
We give a detailed discussion of our experience using AI for mathematics research, particularly touching upon its strengths and weaknesses, as well as our experience with creating ideal conditions for AI to arrive at breakthrough insights.
The mathematical results are presented and proved in a companion paper~\cite{saha2026new}.
}


% which quantifies the hardness threshold between hard combinatorial problems and their efficient continuous relaxations.


% Points for the final sentence:
% * Documentation of our system
% * Strengths and weaknesses
% * Limitations of current AI
% * Ideal conditions for AI to do discovery
% * "Our harness is just some harness ... but we do wanna talk more generally about harnesses"

% We give an extensive documentation of our system, its strengths and weaknesses, as well as our experinece 



% We give extensive documentation of our system, as well as a discussion on what makes ideal conditions for the AI to discover.




% {
% \color{red}
% Mathematics research is a long-horizon task. It comprises of evolving goals, a growing body of knowledge, and delayed feedback. 
% As AI agents become increasingly common in research, it is important to understand conditions under which agents can successfully collaborate with humans on open ended problems. 
% We report an extended case study of human--AI collaboration on such a task: a six-week, 240-session run of an AI research system that we engineered and steered asynchronously, aimed at the Grothendieck constant ($\KG$). The Grothendieck constant is a central constant in optimization, combinatorial algorithms, and analysis. Despite this,  its value has been a mystery since 1953.
% The collaboration produced novel theoretical machinery that discovered new upper and lower bounds,
% \[
%     \frac{6\pi}{11}
%     \;\le\;
%     \KG
%     \;\le\;
%     \frac{\pi}{2\log(1+\sqrt2)} - 10^{-4},
% \]
% This paper ...
% }


% Mathematics research is a long-horizon task: goals evolve, most attempts fail, and the record of what has been learned outgrows any single model context.
% We report an extended case study of human--AI collaboration on such a task: a six-week, roughly 240-session run of an AI research system that we engineered and steered asynchronously, aimed at the Grothendieck constant $\KG$, a central constant in optimization whose value has been open since 1953.
% The collaboration produced new upper and lower bounds,
% \[
%     \frac{6\pi}{11}
%     \;\le\;
%     \KG
%     \;\le\;
%     \frac{\pi}{2\log(1+\sqrt2)} - 10^{-4},
% \]
% determining the previously unknown tenths digit of $\KG$, together with the new frameworks behind them: asymptotic families of rounding schemes on the upper side, and obstructions valid for all such schemes on the lower side.
% The lower bound was discovered and first proved by the AI system; complete proofs appear in a companion paper.
% This paper explains the mathematics at a high level, documents the methodology, reconstructs the discovery, and analyzes the run's capability profile: strong technical execution, but limited research judgement and fragile maintenance of the research state.
% }

\newpage

\tableofcontents

\newpage


==> paper/ai_paper_grothendieck.tex <==
\section{The Grothendieck Constant}
\label{sec:grothendieck}

We first describe the mathematical problem at a high level. The exposition here is deliberately informal; precise definitions and full proofs appear in the companion paper~\cite{saha2026new}.

\paragraph{A hard optimization problem and its relaxation.}
Consider the following discrete optimization problem: given a matrix $A=(a_{ij})\in\R^{m\times n}$, find sign vectors maximizing the bilinear form
\[
    \OPT(A)
    \;:=\;
    \max_{x\in\{\pm1\}^m,\; y\in\{\pm1\}^n}
    \;\sum_{i,j} a_{ij}\, x_i y_j.
\]
Intuitively, we are looking for the best pair of $\pm1$ labelings of the rows and columns of $A$; this quantity is closely related to the \emph{cut norm} of the matrix, a basic primitive in combinatorial optimization, and the problem is NP-hard in general.
A standard way to make it tractable is to relax each sign to a unit vector and each product to an inner product:
\[
    \SDP(A)
    \;:=\;
    \max_{u_i, v_j \in S^{d-1}}
    \;\sum_{i,j} a_{ij}\, \ip{u_i}{v_j},
\]
where the maximum now runs over unit vectors in any dimension $d$.
This relaxation is a semidefinite program (SDP) and can be solved in polynomial time.
Since every sign is a one-dimensional unit vector, $\OPT(A)\le\SDP(A)$: the relaxation can only overshoot.
The basic question is by how much.

Grothendieck's inequality~\cite{Gro53,LP68} answers this question: the overshoot is bounded by a universal constant.
That is, there exists $K<\infty$, independent of $A$, $m$, $n$, and the dimension $d$, such that
\[
    \OPT(A)
    \;\le\;
    \SDP(A)
    \;\le\;
    K\cdot\OPT(A)
    \qquad
    \text{for every matrix } A.
\]
The \emph{Grothendieck constant} $\KG$ is the smallest such $K$.
In modern language, $\KG$ is exactly the worst-case integrality gap of the canonical SDP relaxation of the bilinear optimization problem above.
\cref{fig:groth-pipeline} illustrates the two optimization problems and the rounding step that connects them.

\begin{figure}[t]
\centering
% Source: paper_artifacts/plots/sdp_workflow_figure.py (parent repo)
\includegraphics[width=0.9\textwidth]{figures/sdp_workflow}
\caption{\textbf{From a hard combinatorial problem to a rounded solution.}
\emph{(a)} An instance of the bilinear optimization problem, drawn as a weighted graph: every node carries an unknown sign, every edge a weight $a_{ij}$ (an orange $+2$ edge rewards giving its endpoints equal signs; a dark $-2$ edge rewards opposite signs), and the goal is to choose the signs maximizing the total reward.
\emph{(b)} The SDP relaxation replaces signs by unit vectors; its feasible set is a slice of a convex cone, and the relaxed problem is solvable in polynomial time.
\emph{(c)} The optimal vectors $u_i^\star, v_j^\star$ spread out over a unit sphere in ways that signs cannot.
\emph{(d)} A rounding scheme converts the vectors back into signs (orange $=+1$, dark $=-1$); in this instance the rounded signs satisfy every $-2$ edge.
The Grothendieck constant $\KG$ is the worst-case ratio between the relaxed and the combinatorial optimum.}
\label{fig:groth-pipeline}
\end{figure}

Grothendieck's inequality is a foundational result well beyond this algorithmic reading: it originated in functional analysis, where it is central to the geometry of Banach spaces and harmonic analysis~\cite{pisier2011grothendieckstheorempastpresent,KN11}, it underlies constant-factor approximation algorithms for cut norms~\cite{AN06}, and it governs the maximal advantage of quantum over classical correlations in Bell-type experiments~\cite{Tsi85,CHTW04}.
Despite this breadth of connections, and more than seventy years of study, the exact value of $\KG$ remains unknown.

\paragraph{Rounding schemes as partitions.}
Every upper bound on $\KG$ is, at heart, an algorithm: a \emph{rounding scheme} that converts the unit vectors of an SDP solution back into signs while provably retaining a $1/K$ fraction of the objective.
The schemes relevant to this paper have a simple geometric description.
A \emph{Krivine scheme} is a pair of partitions of $\R^k$ into a $+1$ region and a $-1$ region, encoded by odd sign functions $f,g:\R^k\to\{\pm1\}$ (see \cref{fig:partitions}).
To round, the algorithm maps each SDP vector to a random Gaussian point in $\R^k$, arranged so that the points of $u_i$ and $v_j$ are correlated according to the inner product $\ip{u_i}{v_j}$, and then labels each vector by the region its point lands in: $x_i = f(X_i)$ and $y_j = g(Y_j)$.
The simplest instance takes both partitions to be the same half-space, $f(z)=g(z)=\sgn(z_2)$.
This is called the random hyperplane rounding: label each vector by the side of a random hyperplane it falls on.

\begin{figure}[t]
\centering
% Source: figures/make_partition_schemes.py
\includegraphics[width=0.85\textwidth]{figures/partition_schemes}
\caption{\textbf{Krivine schemes are partitions of space.}
A scheme labels the points of $\R^k$ with $\pm1$ (orange is $+1$, dark is $-1$; shown here for $k=2$), and each SDP vector is rounded to the label of a correlated random Gaussian point.
\emph{Left:} the half-space partition underlying hyperplane rounding and Krivine's classical bound.
\emph{Right:} a partition with a cubic boundary, of the kind used by the cubic--quintic scheme of the companion paper; the dashed line marks the half-space boundary for comparison.
The extra freedom in the shape of the boundary, combined with the enriched correlation structure of limiting schemes, is what suppresses the nonlinearity of the correlation function $H$.}
\label{fig:partitions}
\end{figure}

\paragraph{The normalized correlation function.}
The quality of a Krivine scheme is governed by a single analytic object.
Let $X,Y$ be standard Gaussian points in $\R^k$ whose coordinates are pairwise correlated: $\E[X_iY_i]=t$ for each $i$.
The \emph{normalized correlation function} of the scheme is
\[
    H(t)
    \;:=\;
    \frac{\pi}{2}\,\E\bigl[f(X)\,g(Y)\bigr],
\]
which measures how correlated the two output labels are when the underlying inputs have correlation $t$.
This function is the central object in the analysis of Krivine schemes: the entire performance of a scheme can be read off from it, and, speaking informally, the closer $H$ is to a straight line with a large slope, the better the scheme rounds.

For the half-space partition, a classical identity of Grothendieck gives $H(t)=\arcsin t$, and Krivine's analysis of this arcsine nonlinearity yields his celebrated bound~\cite{Kri77}
\[
    \KG
    \;\le\;
    \frac{\pi}{2\log(1+\sqrt2)}
    \;=\;
    1.7822\ldots
\]
Krivine conjectured that this value is optimal.
The conjecture stood for over three decades, until Braverman, Makarychev, Makarychev, and Naor disproved it in 2011 by mixing hyperplane rounding with a carefully chosen two-dimensional scheme; their argument establishes the strict inequality $\KG<\pi/(2\log(1+\sqrt2))$ but does not quantify the gap~\cite{braverman2011grothendieckconstantstrictlysmaller}.
Naor and Regev later proved a striking converse: such mixed Krivine schemes are asymptotically \emph{optimal}, meaning that as the dimension of the scheme grows, they achieve approximation ratios arbitrarily close to the true value of $\KG$~\cite{naor2014krivine}.
The search for $\KG$ can therefore, in principle, be carried out entirely within this one family of partitions.
Building on this, recent works of Heilman~\cite{heilman2026upperboundgrothendiecksconstant} and of a subset of the authors~\cite{LiSahaXueChaudhuriKlivansKothariMeka2026} independently obtained the first explicit numerical improvements over Krivine's bound, on the order of $10^{-5}$.

\paragraph{Limiting Krivine schemes.}
The companion paper enlarges the space of previously known schemes.
A \emph{limiting Krivine scheme} is obtained as a limit of classical Krivine schemes of growing dimension; it is again described by a pair of partitions, and it inherits the rounding guarantees of the schemes converging to it.
This enlarged search space is where both of the main results live.

\paragraph{Lower bounds are hard instances.}
Lower bounds on $\KG$ have historically come from the complementary direction: exhibiting an explicit matrix $A$ for which $\SDP(A)$ provably exceeds $\OPT(A)$ by a large factor.
Grothendieck's own work implies $\KG\ge\pi/2$, and a high-dimensional Gaussian construction found independently by Davie and Reeds gives $\KG\ge1.6769\ldots$~\cite{Davie1984LowerBoundKG,Reeds1991LowerBoundKG}.
That bound stood for more than four decades, until two recent works improved it by $10^{-26}$ and $10^{-12}$, respectively~\cite{heilman2026lowerboundgrothendiecksconstant,jones2026grothendieckconstantstrictlylarger}.
The state of the art entering this work was thus
\[
    1.6769\ldots \;\le\; \KG \;\le\; 1.7822\ldots,
\]
an interval wide enough that even the tenths digit of $\KG$ was unknown.

\section{The Results of the Companion Paper}
\label{sec:companion-results}

The companion paper~\cite{saha2026new} proves two results, one for lower bound and one for upper bound.
We state them here in abridged form; the rest of this paper needs only the statements and the shape of the arguments.

\begin{theorem}[Upper bound, abridged]
\label{thm:ub-abridged}
% Alias so that references in ai_section_revised.tex resolve in this paper:
\label{thm:cubic-quintic-upper-bound}
There is an explicit limiting Krivine scheme, the \emph{cubic--quintic scheme}, which can be used to show
\[
    \KG
    \;\le\;
    \frac{\pi}{2\log(1+\sqrt2)} - 3.47\times10^{-4}.
\]
\end{theorem}

The scheme's partitions have cubic boundaries of the kind shown in \cref{fig:partitions} (right).
All previous constructions, including the two recent $10^{-5}$-scale improvements, were fixed low-dimensional schemes; this is the first improvement obtained by letting the dimension grow, and it answers affirmatively a question of Braverman et al.~\cite{braverman2011grothendieckconstantstrictlysmaller} on whether higher dimension helps.

\begin{theorem}[Lower bound, abridged]
\label{thm:lb-abridged}
The correlation function $H(t)=b_1t+b_3t^3+\cdots$ of every Krivine scheme satisfies the constraint
\begin{equation}
% Label matches the main paper's, so that references in ai_section_revised.tex
% resolve in this paper:
\label{eq:affine-coefficient-inequality}
    b_3 \;\ge\; 2b_1-\frac{11}{6}.
\end{equation}
Combined with the optimality theorem of Naor and Regev~\cite{naor2014krivine}, this implies
\[
    \KG \;\ge\; \frac{6\pi}{11} \;=\; 1.7135\ldots
\]
\end{theorem}

The interesting feature of \cref{thm:lb-abridged} is the reversal of strategy.
Instead of constructing a hard instance, the proof establishes a ceiling on the performance of \emph{every} scheme. 
This is the first lower bound on $\KG$ that does not proceed by constructing a gap instance.
The proof reduces the constraint on high-dimensional partitions to a small set of one-dimensional Gaussian inequalities.

Together, the two theorems give
\[
    \frac{6\pi}{11}
    \;\le\;
    \KG
    \;\le\;
    \frac{\pi}{2\log(1+\sqrt2)} - 3.47\times10^{-4},
\]
determining the tenths digit of $\KG$ to be $7$.
The remainder of this paper concerns how these results were found: the AI research system and its methodology, the run itself, and what the record shows about current AI systems as mathematical collaborators.


==> paper/ai_paper_introduction.tex <==
\section{Introduction}
\label{sec:intro}

The mathematical capabilities of AI systems have grown at a remarkable pace.
Within a few years, they have progressed from solving grade-school word problems to matching the best human performers on competition and advanced mathematics benchmarks~\cite{hubert2026alphaproof, imo-gold, glazer2024frontiermath}.
Mathematics research, however, is a \emph{long-horizon} task.
Its goals are often not clearly defined and evolve over time. 
Success is judged not only by whether a statement is proved, but also by whether the right statement was chosen in the first place. 
It requires building a body of knowledge whose significance may be apparent only later; that is, in research, rewards are sparse, and often delayed.
% It comprises of goals that are not clearly defined, a growing body of knowledge, and sparse, often delayed reward signals. 
% Success is judged not only by whether a statement gets proved, but by whether the right statement was chosen in the first place. 
It is still an open question how to use AI effectively at this horizon.

Existing systems occupy well-specified corners of this space.
Evaluator-guided searches such as FunSearch and AlphaEvolve explore spaces of programs or constructions, but require a fixed objective and an automatic scoring function~\cite{funsearch,novikov2025alphaevolvecodingagentscientific}.
Formal-proof systems such as AlphaProof obtain a similarly clear correctness signal from a proof assistant, but require a fixed formal statement~\cite{hubert2026alphaproof}.
Interactive use of frontier models provides broad technical assistance, but leaves agenda-setting, memory, and verification with the human expert~\cite{bubeck2025science}.

In this work, we provide a detailed case study of our experience using AI operating at the level of a research \emph{program}: deciding what to attempt next, retaining what failed and why, and converting an accumulation of failures into new mathematics.
We engineered an AI research system asynchronously steered by human operators.
We directed it at a concrete open problem: the Grothendieck constant $\KG$, which quantifies the hardness threshold between hard combinatorial optimization problems and their efficient continuous relaxations, and whose value has been open since 1953.

The collaboration tightened the best known bounds on both sides,
\[
    1.7135\ldots
    \;=\;
    \frac{6\pi}{11}
    \;\le\;
    \KG
    \;\le\;
    \frac{\pi}{2\log(1+\sqrt2)} - 3.47\times10^{-4}
    \;=\;
    1.7818\ldots,
\]
The upper bound comes from a new asymptotic framework for rounding algorithms, and the lower bound from the first argument that bounds $\KG$ from below without constructing a hard instance.
Central steps of this mathematics originated with the AI system and were judged novel by domain experts; all results stated as theorems have been independently verified by the authors, and complete proofs appear in the companion paper~\cite{saha2026new}.
Our contributions are as follows.
\begin{enumerate}[label=(\arabic*), leftmargin=*]
    \item \textbf{Novel approaches for a longstanding open problem.}
    We give an expository account of the Grothendieck constant and of the results in \cref{sec:grothendieck} and \cref{sec:companion-results}.
    The upper bound introduces \emph{limiting Krivine schemes}, which enlarge the space of rounding algorithms studied since Krivine's work.
    The lower bound converts obstructions on all rounding schemes into lower bounds on $\KG$; it is the first lower bound on the constant that does not proceed by constructing a hard instance.

    \item \textbf{A methodology for long-horizon AI research.}
    We document the system in \cref{sec:ai-methodology}: its division of labor between a reasoning model and a coding agent, its file-based memory, its calibrated internal verification protocol, and its channel for asynchronous human steering.
    The run and its outcomes are quantified in \cref{sec:ai-results}.

    \item \textbf{A case study with an analysis of capabilities.}
    We reconstruct how the lower bound was found in \cref{sec:ai-case-study} and analyze the full record in \cref{sec:ai-discussion}.
    The record shows a consistent asymmetry: the system was strong at technical execution, but substantially less reliable at research judgement and at maintaining an accurate research state.
    % This suggests where human oversight has the greatest leverage, and \cref{sec:ai-future} proposes concrete directions for closing the gap.
\end{enumerate}


==> paper/ai_section.tex <==
% ============================================================================
% AI SECTION -- draft to be merged into the main paper as a single section.
% No abstract and no title: the \section below is the section itself.
% Style: anton_style.md. Items needing author confirmation are marked %% TODO.
% ============================================================================


\hypersetup{
  colorlinks=true,
  linkcolor=blue!55!black,
  urlcolor=blue!55!black,
  citecolor=blue!55!black
}

\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}
\setlist[itemize]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}
\setlist[enumerate]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}

\part{AI Methodology and Analysis}
\label{sec:ai}


The results in this paper were obtained in collaboration with an autonomous
AI research system. The cubic--quintic
construction and its certificate (Theorem~\ref{thm:cubic-quintic-upper-bound})
predate the current system and were found through conversation with GPT-5.5-Pro. The lower bound $\KG\ge6\pi/11$ was
discovered and first proved by the system; we have since verified the
argument ourselves, and the proof in this paper is our revision of the
system's write-up. The system also produced further improvements on both
sides of the problem, which we report in Section~\ref{sec:ai-results} but do
not state as theorems, because their certificates have not yet been human-verified. This section documents the methodology
(Section~\ref{sec:ai-methodology}), quantifies the run and its outcomes
(Section~\ref{sec:ai-results}), reconstructs how the lower bound was found
(Section~\ref{sec:ai-case-study}), and discusses what the record shows about
the strengths and weaknesses of current AI systems as mathematical
collaborators (Sections~\ref{sec:ai-discussion} and~\ref{sec:ai-future}).

\section{Methodology}
\label{sec:ai-methodology}

\paragraph{AI models and compute.}
The run used two frontier language models: a reasoning model (OpenAI
GPT-5.5-Pro at maximal reasoning effort, replaced mid-run by GPT-5.6-Sol)
and a coding agent (Anthropic Claude Code, running Claude Opus and later
Claude Fable~5). Floating-point searches
ran on a single four-GPU node, and every Arb-certified computation was redone in interval arithmetic on CPU.

% \paragraph{The AI research system.}
% The AI research system is designed as a harness. The 
% harness couples the two models in distinct roles: (1) The \textit{reasoning model}
% serves as the brain that selects directions, develops arguments, specifies
% experiments, and audits the resulting claims; (2) The \textit{coding agent} serves as
% the executor that maintains the project repository, implements and runs
% experiments, retrieves literature, and drives the reasoning model through
% a scripted interface. The models run in bounded sessions, and no model
% context survives from one session to the next; continuity is carried by
% files, principally a problem statement, a single summary file that serves
% as working memory and into which finished work is merged, and append-only
% transcripts and experiment logs. The harness was adjusted repeatedly over
% the run in response to observed failures; we describe its final form, to
% the extent needed to interpret the record.

\paragraph{The AI research system.}
The AI research system is organized as a harness coupling two agents in distinct roles: (1) the \textit{reasoning agent} serves as the brain that selects directions, develops arguments, specifies experiments, and audits the resulting claims, and (2) the \textit{coding agent} serves as the executor that maintains the project repository, implements and runs experiments, retrieves literature, and drives the reasoning model through a scripted interface.

The agents run in bounded sessions, and no agent context survives from one session to the next. Continuity is instead carried by files, principally a problem statement, a single summary file that serves as working memory and into which finished work is merged, and append-only transcripts and experiment logs. The harness was adjusted repeatedly over the run in response to observed failures; we describe its final form, to the extent needed to interpret the record.

\paragraph{Run configuration.}
Work is organized into \emph{sessions} of a few hours, of which two to
five run concurrently on mutually distinct directions. A session passes
through fixed phases: orientation from the problem statement and summary
files, selection of a focus, a research loop in which the reasoning model
requests computations, literature, or further reasoning time, and a
closing audit that produces a calibrated summary in which every claim is
tagged as proven, numerically supported, conjectural, or heuristic. We
reserve the word theorem, here and in the rest of the paper, for
statements that we have additionally checked ourselves.

The run was initialized with our prior work on the constant: the
cubic--quintic scheme, the coefficient formulas and certification
machinery, several months of accumulated notes, and a problem statement
listing candidate directions for both bounds. The search space the run
explored is a generalization of the cubic--quintic scheme, and the
possibility of converting obstructions into lower bounds was raised, as a
suggestion, in the problem statement. The system therefore operated
downstream of the mathematical framework it was given, a point quantified
in Section~\ref{sec:ai-case-study}.

\paragraph{Human collaboration.}
Human operators (the authors) steered the run asynchronously
through text files read at the start of, and during, every session.
Steering consisted of priorities, targets, audits of the run's own claims,
and occasional mathematical pointers; about forty directives were
issued over the run. 
% The operator contributed no proof steps through this
channel.

\section{Results}
\label{sec:ai-results}

The run spanned June~16 to July~24, 2026. It comprised
roughly 240 research sessions. The reasoning model was called 2{,}091
times, consuming about 152 million tokens at an estimated \$5{,}400 in
API cost; the coding agent ran on a flat-rate subscription (Claude Max).
Table~\ref{tab:run} collects these figures, and
Table~\ref{tab:timeline} gives the timeline of the bounds.

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}ll@{}}
\toprule
Duration & June 16 -- July 24, 2026 (main phase through July 4)\\
Research sessions & $\approx240$\\
Reasoning model & GPT-5.5-Pro, later GPT-5.6-Sol; maximal effort\\
Usage and cost & 2{,}091 calls; $\approx152$M tokens; $\approx\$5{,}400$\\
Coding agent & Claude Code (Opus, later Fable 5); subscription\\
Human steering  $\approx40$ dated directives\\
\bottomrule
\end{tabular}
\caption{\textbf{The run at a glance.} Aggregates computed from the harness
telemetry. Dollar figures are list-price estimates; coding-agent usage was
only partially metered.
}
\label{tab:run}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lp{0.76\textwidth}@{}}
\toprule
Sessions & Event\\
\midrule
1 & run begins from the interval $1.6769566742\le\KG\le1.7818666070$
(the upper end is the cubic--quintic bound of this paper)\\
18 & upper-bound search plateaus; the operators direct a pivot to the
lower bound\\
44 & numerical upper bound $1.7802243$ recorded (later withdrawn)\\
55--57 & affine reframe; $\KG\ge6\pi/11$ derived\\
58--64 & $6\pi/11$ proof machine-audited; first \LaTeX{} write-up\\
92, 117 & lower bounds $27\pi/49\approx1.7311$ and
$51\pi/92\approx1.7415$ machine-verified\\
follow-up & the session-44 value found unsupported by internal audit and
withdrawn\\
follow-up & upper bound $1.781801841033$ machine-certified\\
follow-up & upper bound $1.7813319810625639$ machine-certified;
adversarial review passed\\
\bottomrule
\end{tabular}
\caption{\textbf{Timeline of the bounds produced during the run.}
Machine-verified means accepted by the verification protocol of
Section~\ref{sec:ai-methodology}. The last three events fall in the short
follow-up phases, whose sessions we do not cite individually. Of the
run's results, only $\KG\ge6\pi/11$ has additionally been verified by the
authors; it is the result stated as a theorem in this paper.}
\label{tab:timeline}
\end{table}

The run's principal outcome, and the one this paper states as a theorem,
is the lower bound $\KG\ge6\pi/11$, whose discovery
Section~\ref{sec:ai-case-study} reconstructs. Beyond it, the run produced
machine-certified upper bounds of $1.781801841033$ and then
$1.7813319810625639$, improving on the cubic--quintic value, together with
the two stronger lower bounds listed in Table~\ref{tab:timeline}. We
report these as machine-verified claims rather than theorems: each passed
the full internal protocol, but we have not yet verified their
certificates ourselves.
%% TODO: reconcile with the main paper's discussion of concurrent work
%% (e.g. Heilman's computer-assisted improvement of Krivine's bound,
%% arXiv:2606.00247).

\section{Case study: from a failed upper-bound search to a lower bound}
\label{sec:ai-lower-bound-case-study}

The lower bound is the run's main discovery. We reconstruct it here in
outline, highlighting the human interventions that shaped it, and the ingenuity of the AI system once it had the right framing.

The lower bound began with a plateauing search for a better upper bound. The system explored several variants of the limiting Krivine schemes developed in Section~\ref{sec:LimitingKrivine}. Although the constructions differed, they repeatedly encountered
the same tradeoff: suppressing the unwanted nonlinear terms in the inverse majorant series also weakened
the leading term. The run recorded this pattern, but continued to search
for further constructions rather than treating the repeated failures as
evidence of a general obstruction.

The important human contribution was in identifying there was likely an analytic obstruction, and in recognizing that proving the generality of this obstruction for all mixed and limiting schemes is mathematically valuable as the optimality theorem of Naor and Regev~\cite{naor2014krivine} would imply a lower bound for $K_G$. Thus, the operators asked the system to stop searching for new limiting Krivine schemes, and instead synthesize the its failures so far, search for patterns, and attempt to generalize and prove these for all schemes.

Once this objective was fixed, and with a bit more high-level human guidance, the system developed the central argument
and produced a complete proof (see all of Part~\ref{part:LowerBound}). It expressed the obstruction as an
affine inequality between the two leading coefficients of a scheme's
correlation function (see Equation~\ref{eq:affine-coefficient-inequality}). Because this inequality is preserved under averaging
and limits, it extends to mixed and limiting schemes. The system then
cleverly reduced the high-dimensional terms it needed to bound to one-dimensional estimates and produced
the required computer-assisted certificate, yielding
\[
    \KG \geq \frac{6\pi}{11}.
\]
The authors subsequently revised the exposition and independently verified
the proof.

This episode illustrates the different roles of the human operators and the AI system throughout the run. The system was effective at technical execution: drawing from its wealth of mathematical knowledge and its competence in problem-solving to propose lemmas and construct proofs. The human input was primarily of research judgement and mathematical taste: judging when a research direction has been somewhat exhausted, understanding that mathematical understanding and discoveries frequently come from synthesizing failures, 
and recoginizing that a new lower-bound mechanism is much more interesting than a small numerical improvement to a
known upper-bound method. Appendix~\ref{app:ai-case-study} gives the
detailed chronology.


\section{Discussion}
\label{sec:ai-discussion}

The record supports a consistent capability profile: strong technical
execution, with persistent failures in the judgement that directs it. We
summarize the strengths, then the weaknesses, exemplified by Section~\ref{sec:ai-case-study} 

make concrete, describe
the human operator's involvement, and close by relating the run to recent
AI results in mathematics.

\subsection{Strengths}

Three strengths carried the run. The first is technical range with effective
recall: given a one-word pointer to Naor's work, the system identified the
relevant theorem, verified its normalization against the paper, and computed
the slack available for a lossy transfer; given a plateau, it produced six
structurally distinct escape mechanisms in two days. The second is local
invention: the affine family, the fiber reduction, the closure lemma, and
the certificate architecture were machine products, several arriving within
hours once the question was well posed. The third is speed and reliability
of execution: from the reframe to a machine-audited, interval-certified
proof took about a day, and most individual technical errors were caught by
the system's own verification passes. In one representative episode
(sessions p44 and p49), a claimed bound of $\KG\ge1.7754518$
was refuted within five hours by an adversarial session that computed its
true margin to be approximately $-8\times10^{-8}$, and the record was
corrected to the defensible value.

\subsection{Weaknesses}

Each intervention of Section~\ref{sec:ai-case-study} was needed because a
specific capability was absent. The paragraphs below name these
capabilities and add further instances from the record.

\paragraph{Poor judgement of what is interesting.}
The system did not reliably rank work by mathematical interest. The second
and third interventions are the clearest cases: the run treated refinements
of the two-dimensional ceiling as progress when only the general bound
mattered, and, once the family of rungs existed, it valued improvements
within the family over establishing the first certified rung. The same
tendency appeared at smaller scales throughout, from sessions spent on
$10^{-5}$-sized improvements to mechanisms the run already understood, down
to reported values tuned to the edges of their enclosures. The implication
for collaboration is that the objective of the research cannot yet be
delegated. The operator's judgements of interest were few, but each
redirected weeks of machine effort, and between them the system optimized,
competently, whatever was in front of it. On a problem of this size the
space of possible intermediate constructions is unbounded, and a ranking by
expected interest is what makes the search tractable; supplying that
ranking was the human's principal ongoing contribution.

\paragraph{Lack of high-level research skills.}
The system managed individual arguments well and the research process
poorly: it did not decide when to persist, when to switch, or what a
sequence of failures implied. The first intervention is the sharpest case,
since the dualization of failures into a lower bound was suggested in the
problem statement the system re-read at every session, the six failures
were in its memory, and the step was taken only when ordered. The record
contains three further episodes of the same shape, of fourteen, roughly two
dozen, and about a dozen sessions respectively (the two-dimensional
extension, near-sharp variants of the lower bound, and the July
certification effort), in each of which the run circled a target without
progress until the operator ended the loop. The implication is that
autonomous running time does not by itself convert into progress. Once the
accessible directions were exhausted, additional sessions multiplied
execution, not judgement, and the run's rate of real progress was set by
the frequency of strategic correction; additional compute would not have
changed it. Oversight of such systems is accordingly most valuable at the
level of strategy, which is precisely the level at which the system did not
correct itself.

\paragraph{Unreliable memory.}
The harness's file-based memory preserved statements more reliably than
their qualifications. The withdrawn upper bound of Table~\ref{tab:timeline}
is the clearest case. In session 44 the run recorded a numerical upper
bound of $1.7802243$, with caveats attached; over the nineteen days the
value stood in working memory, re-summarization detached the caveats from
the headline number, and a note defending the value was written three days
before the internal audit that refuted it, finding the score inflated by a
finite truncation window and the underlying correlation profile
infeasible. A related failure occurred inside verification, where a
dedicated replay of the $51\pi/92$ certificate (session p95) passed it
because the replay inherited the framing of the argument it was checking;
the invalidating error was found the same day by a session that rebuilt the
argument from scratch (session p102). We attribute both failures to scale.
The run produced hundreds of sessions and tens of millions of tokens of
intermediate mathematics, and each new session could be shown only a small
distillate of it. What to retain, at what resolution, and with which
qualifications attached was itself decided by the models, through repeated
summarization, and repeated summarization is exactly where caveats detach
and inherited framings go unquestioned. Unlike the previous two weaknesses,
this one looks amenable to engineering: memory for such systems plausibly
needs more structure than prose summaries provide, for instance a graph of
claims carrying provenance and qualifications, so that important
information remains retrievable without being repeatedly re-serialized
through a model's context window.

\paragraph{Origins of the weaknesses.}
We believe these gaps have a common origin in how current systems are
produced. Models are trained and evaluated on problems selected for being
small enough to pose, sandbox, and score, and nothing in that regime
exercises the allocation of weeks of effort across an open-ended search.
The corpus they learn mathematics from is, moreover, made of finished
mathematics: the literature records definitions, theorems, and polished
proofs, while the process that produced them, the dead ends, the decisions
to abandon or reframe, the judgement of what was worth attempting, is
largely absent from the written record. A system trained this way can be
expected to acquire technique and the form of finished mathematics while
remaining weak at exactly the process skills described above, and that is
what we observe.

\subsection{Human operator involvement}

A useful summary of the collaboration is obtained by counting who caught
which errors. Errors in individual claims, such as wrong constants, broken
certificates, and invalid steps, were caught almost entirely by the system
itself. Failure patterns spanning many sessions, such as the three circling
episodes and the detachment of caveats from claims, were caught by the
operator in every recorded instance and by the system in none. The system
reliably falsifies a claim once the claim is specified; deciding which
claims to distrust remained a human function throughout. Consistent with
this, the operator's leverage came less from mathematical suggestions, most
of which the system correctly tested and discarded, than from calibration:
setting targets, ending loops, and auditing the run's own reporting. We also
note a regularity with design consequences: every overclaiming incident in
the record sits at a target with nearly zero margin, whereas the results
that survived verification all carry slack. This suggests that systems of
this kind are most productive when aimed at robust targets, with sharp
constants attempted only from a secured base.

\subsection{Relation to recent work}

Recent successes of AI in mathematics, including on open problems, are of
a different kind from the work reported here. Evaluator-guided search has
produced record
constructions~\cite{funsearch,novikov2025alphaevolvecodingagentscientific, charton2024patternboostconstructionsmathematicslittle},
and formal provers have shown proficiency at solving olympiad-level
problems \cite{novikov2025alphaevolvecodingagentscientific}.
%% TODO: the formal-provers citation should probably point to AlphaProof
%% (Hubert et al., Nature 651:607--613, 2026) rather than AlphaEvolve.
In recent and concurrent work, frontier models have gone further: an
internal reasoning model at OpenAI has disproved the Erd\H{o}s
unit-distance conjecture \cite{openai2026planarpointsets}, a counterexample to the Jacobian conjecture using Claude Fable 5
\cite{jacobian}, and OpenAI has announced solutions to ten open problems in mathematics and theoretical computer
science \cite{openai2026ten}. Most of these results involved resolving a
single well-posed statement by construction. Moreover, none explicitly
required significant long-horizon reasoning. Finally, all of the recent
results with frontier models were found fully autonomously, without
sustained human intervention.

Our work is an extensive case study of how humans and AI can collaborate
on mathematical research. The problem is more open-ended, requiring a
research program where over the course of weeks intermediate results
accumulate and directions are opened and abandoned. Moreover, humans were
consistently steering the system and providing feedback. We hope that our
experiences outlined in this section will be useful to future AI and mathematics researchers alike.

\section{Future directions}
\label{sec:ai-future}

\paragraph{Mathematics.}
The immediate items are the machine-verified claims of
Table~\ref{tab:timeline}: human verification of the two certified upper
bounds and of the lower bounds $27\pi/49$ and $51\pi/92$ would upgrade each
to a theorem. Beyond them, the run's internal analysis identifies the
tangent case $\lambda=\tfrac12$ of the affine family, equivalent to a sharp
degree-three chaos inequality, as the natural boundary of the method and
worth $\KG\ge9\pi/16$ if resolved.
% {\color{red}AX: If you're brave, conjecture that \(K_G = \sqrt{\pi}\)}

\paragraph{Toward AI systems for long-horizon research.}
If the diagnosis of Section~\ref{sec:ai-discussion} is right, the
requirements for progress follow from it. First, mathematical
interestingness needs to become an object of study in its own right: the
judgement that selects which questions, intermediate constructions, and
targets are worth pursuing was the most consequential input the human
supplied, and there is at present no training signal or benchmark that
rewards it. Second, the process of research mathematics needs data. What
humans actually do between problem statement and finished paper,
how they allocate effort, learn from repeated failure, and decide to
reframe, is barely recorded anywhere; records of long runs such as ours,
which preserve every step including the unsuccessful ones, are one way to
begin creating such data, and we release ours in that spirit. Third,
evaluation must move to horizons where these capabilities matter, treating
a weeks-long research program rather than a single problem as the unit of
assessment, with memory and calibration measured alongside correctness.
These conclusions carry the usual caution that they derive from one run on
one problem; replications on other open problems, successful or not, would
be the most useful follow-up work.

\paragraph{Human--AI collaboration.}
The run also suggests where collaboration of this kind is heading. Within
it, the contributions that required a human were not technical: the system
supplied the arguments, the computations, the certificates, and the first
write-up, while the human supplied the problem, the taste, and the
strategic corrections. If the technical abilities of these systems continue
to improve, this division will sharpen, and the human's role in
such collaborations will concentrate into choosing what to work on, judging
which objects and targets matter, and deciding what to trust: directing
research that one does not personally execute. A similar shift is already
under way in software engineering. We expect working modes of this kind to
become common in mathematics, and the run documented here, with its
weaknesses as much as its results, is an early picture of what they will
require of the human operator.

\paragraph{Statement on AI use.}
Large language models were used extensively in the research reported in
this paper, in the roles described in this section: GPT-5.5-Pro and
GPT-5.6-Sol (OpenAI) as the reasoning model, and Claude Opus and Claude
Fable~5 (Anthropic) as the coding agent. AI assistance was also used in
preparing parts of this manuscript. All results stated as theorems have been
verified by the authors independently of these systems, and the account of
the run given in this section reflects the authors' own reading of the
record. The authors take full responsibility for the contents of this
paper.



==> paper/ai_section_revised.tex <==

\hypersetup{
  colorlinks=true,
  linkcolor=blue!55!black,
  urlcolor=blue!55!black,
  citecolor=blue!55!black
}

\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}
\setlist[itemize]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}
\setlist[enumerate]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}

\section{AI Methodology and Analysis}
% \label{sec:ai}
\label{sec:ai-methodology}

The lower bound results in this paper were obtained in collaboration with an AI research system. The cubic--quintic
construction and its certificate (Theorem~\ref{thm:cubic-quintic-upper-bound})
predate the current system and were found through conversation with GPT-5.5-Pro. The lower bound $\KG\ge6\pi/11$ was
discovered and first proved by the system; we have since verified the
argument ourselves, and the proof in the companion paper~\cite{saha2026new} is our revision of the
system's write-up. The system also produced further improvements on both
sides of the problem, which we report in Section~\ref{sec:ai-results} but do
not state as theorems, because their certificates have not yet been human-verified. This section documents the methodology
(Section~\ref{sec:ai-methodology}), quantifies the run and its outcomes
(Section~\ref{sec:ai-results}), reconstructs how the lower bound was found
(Section~\ref{sec:ai-case-study}), and discusses what the record shows about
the strengths and weaknesses of current AI systems as mathematical
collaborators (Section~\ref{sec:ai-discussion}).

% \section{Methodology}

\paragraph{AI models and compute.}
The run used two frontier language models: a reasoning model (OpenAI
GPT-5.5-Pro at maximal reasoning effort, replaced mid-run by GPT-5.6-Sol)
and a coding agent (Anthropic Claude Code, running Claude Opus and later
Claude Fable~5). Floating-point searches
ran on a single four-GPU node, and every Arb-certified computation was redone in interval arithmetic on CPU.

% \paragraph{The AI research system.}
% The AI research system is designed as a harness. The 
% harness couples the two models in distinct roles: (1) The \textit{reasoning model}
% serves as the brain that selects directions, develops arguments, specifies
% experiments, and audits the resulting claims; (2) The \textit{coding agent} serves as
% the executor that maintains the project repository, implements and runs
% experiments, retrieves literature, and drives the reasoning model through
% a scripted interface. The models run in bounded sessions, and no model
% context survives from one session to the next; continuity is carried by
% files, principally a problem statement, a single summary file that serves
% as working memory and into which finished work is merged, and append-only
% transcripts and experiment logs. The harness was adjusted repeatedly over
% the run in response to observed failures; we describe its final form, to
% the extent needed to interpret the record.

\paragraph{The AI research system.}
The AI research system is organized as a harness coupling two agents in distinct roles: (1) the \textit{reasoning agent} serves as the brain that selects directions, develops arguments, specifies experiments, and audits the resulting claims, and (2) the \textit{coding agent} serves as the executor that maintains the project repository, implements and runs experiments, retrieves literature, and drives the reasoning model through a scripted interface.

The agents run in bounded sessions, and no agent context survives from one session to the next. Continuity is instead carried by files, principally a problem statement, a single summary file that serves as working memory and into which finished work is merged, and append-only transcripts and experiment logs. The harness was adjusted repeatedly over the run in response to observed failures; we describe its final form, to the extent needed to interpret the record.

\paragraph{Run configuration.}
Work is organized into \emph{sessions} of a few hours, of which two to
five run concurrently on mutually distinct directions. A session passes
through fixed phases: orientation from the problem statement and summary
files, selection of a focus, a research loop in which the reasoning model
requests computations, literature, or further reasoning time, and a
closing audit that produces a calibrated summary in which every claim is
tagged as proven, numerically supported, conjectural, or heuristic. We
reserve the word theorem, here and in the rest of the paper, for
statements that we have additionally checked ourselves.

The run was initialized with our prior work on the constant: the
cubic--quintic scheme, the coefficient formulas and certification
machinery, several months of accumulated notes, and a problem statement
listing candidate directions for both bounds. The search space the run
explored is a generalization of the cubic--quintic scheme, and the
possibility of converting obstructions into lower bounds was raised, as a
suggestion, in the problem statement. The system therefore operated
downstream of the mathematical framework it was given, a point quantified
in Section~\ref{sec:ai-case-study}.

\paragraph{Human collaboration.}
Human operators (the authors) steered the run asynchronously
through text files read at the start of, and during, every session.
Steering consisted of priorities, targets, audits of the run's own claims,
and occasional mathematical pointers; about forty directives were
issued over the run. 
% The operator contributed no proof steps through this channel.

\section{Results}
\label{sec:ai-results}

The run spanned June~16 to July~24, 2026. It comprised
roughly 240 research sessions. The reasoning model was called 2{,}091
times, consuming about 152 million tokens at an estimated \$5{,}400 in
API cost; the coding agent ran on a flat-rate subscription (Claude Max).
Table~\ref{tab:run} collects these figures, and
Table~\ref{tab:timeline} gives the timeline of the bounds.

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}ll@{}}
\toprule
Duration & June 16 -- July 24, 2026 (main phase through July 4)\\
Research sessions & $\approx240$\\
Reasoning model & GPT-5.5-Pro, later GPT-5.6-Sol; maximal effort\\
Usage and cost & 2{,}091 calls; $\approx152$M tokens; $\approx\$5{,}400$\\
Coding agent & Claude Code (Opus, later Fable 5); subscription\\
Human steering  $\approx40$ dated directives\\
\bottomrule
\end{tabular}
\caption{\textbf{The run at a glance.} Aggregates computed from the harness
telemetry. Dollar figures are list-price estimates; coding-agent usage was
only partially metered.
}
\label{tab:run}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lp{0.76\textwidth}@{}}
\toprule
Sessions & Event\\
\midrule
1 & run begins from the interval $1.6769566742\le\KG\le1.7818666070$
(the upper end is the cubic--quintic bound of this paper)\\
18 & upper-bound search plateaus; the operators direct a pivot to the
lower bound\\
44 & numerical upper bound $1.7802243$ recorded (later withdrawn)\\
55--57 & affine reframe; $\KG\ge6\pi/11$ derived\\
58--64 & $6\pi/11$ proof system-tested; first \LaTeX{} write-up\\
92, 117 & lower bounds $27\pi/49\approx1.7311$ and
$51\pi/92\approx1.7415$ machine-verified\\
follow-up & the session-44 value found unsupported by internal audit and
withdrawn\\
follow-up & upper bound $1.781801841033$ system-tested\\
follow-up & upper bound $1.7813319810625639$ system-tested;
adversarial review passed\\
\bottomrule
\end{tabular}
\caption{\textbf{Timeline of the bounds produced during the run.}
Machine-verified means accepted by the verification protocol of
Section~\ref{sec:ai-methodology}. The last three events fall in the short
follow-up phases, whose sessions we do not cite individually. Of the
run's results, only $\KG\ge6\pi/11$ has additionally been verified by the
authors; it is the result stated as a theorem in this paper.}
\label{tab:timeline}
\end{table}

The run's principal outcome, and the one this paper states as a theorem,
is the lower bound $\KG\ge6\pi/11$, whose discovery
Section~\ref{sec:ai-case-study} reconstructs. Beyond it, the run produced
system-tested upper bounds of $1.781801841033$ and then
$1.7813319810625639$, improving on the cubic--quintic value, together with
the two stronger lower bounds listed in Table~\ref{tab:timeline}. We
report these as machine-verified claims rather than theorems: each passed
the full internal protocol, but we have not yet verified their
certificates ourselves.
%% TODO: reconcile with the main paper's discussion of concurrent work
%% (e.g. Heilman's computer-assisted improvement of Krivine's bound,
%% arXiv:2606.00247).

\section{Case study: from a failed upper-bound search to a lower bound}
\label{sec:ai-case-study}

The lower bound is the run's main discovery. We reconstruct it here in
outline, highlighting the human interventions that shaped it and the
mathematical contributions of the AI system once it had the right framing.

The lower bound began with a plateauing search for a better upper bound.
The system explored several variants of the limiting Krivine schemes.
Although the constructions differed, they repeatedly encountered the same
tradeoff: suppressing the unwanted nonlinear terms in the inverse majorant
series also weakened the leading term. The run recorded this pattern, but
continued to search for further constructions rather than treating the
repeated failures as evidence of a general obstruction.


The key human intervention was to recognize that the repeated failures likely reflected a general analytic obstruction, and that proving such an obstruction for mixed and limiting schemes would itself be mathematically valuable: by the optimality theorem of Naor and Regev~\cite{naor2014krivine}, it would imply a lower bound on $K_G$. The operators therefore redirected the system away from searching for new limiting Krivine schemes and asked it instead to synthesize the accumulated failures, identify their common structure, and attempt to prove a universal obstruction.

After further program-level directives, the system found the central
mathematical reframe and developed a complete proof
(see \cite[Part~1]{saha2026new}). It expressed the obstruction as an affine
inequality between the two leading coefficients of a scheme's correlation
function. Because this
inequality is preserved under averaging and limits, it extends to mixed and
limiting schemes. The system then reduced the required high-dimensional
estimates to one-dimensional inequalities and produced the computer-assisted
certificate, yielding
\[
    \KG \geq \frac{6\pi}{11}.
\]
The authors subsequently revised the exposition and independently verified
the proof.

This illustrates the different roles of the human operators and the AI system throughout the run. The system was effective at technical execution: drawing from its wealth of mathematical knowledge and its competence in problem-solving to propose lemmas and construct proofs. The human input was primarily of research judgement and mathematical taste: judging when a research direction has been somewhat exhausted, understanding that mathematical understanding and discoveries frequently come from synthesizing failures, 
and recognizing that a new lower-bound mechanism is much more interesting than a small numerical improvement to a
known upper-bound method.
Appendix~\ref{app:ai-case-study} gives the
detailed chronology.


\section{Discussion}
\label{sec:ai-discussion}
Motivated by mathematical problem-solving frameworks such as~\cite{carlson2005problemsolving, schoenfeld1983episodes}, we present the following decomposition of long-horizon mathematical
research in the harness (see Figure~\ref{fig:research-cycle}). At any point in time, a research program has an \emph{active represented state}. This is a compact representation of the complete history of the run for the purpose of choosing the next step, including current objectives, established and conjectural claims, evidence, failed approaches, open proof obligations, and unresolved choices. From this state, the
researcher uses \emph{research judgement} to select a high-level action. Such
an action might be to prove an auxiliary lemma, test a new construction,
compare several failures, search for a counterexample, reformulate the target,
or audit an earlier claim. \emph{Technical execution} takes the high-level action, and then plans and executes the steps needed to produce results. Finally, those results must be distilled and incorporated into
an updated active represented state, in a way that is efficient and preserves all important information. The cycle then repeats.

\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
      box/.style={
        draw,
        rounded corners=2pt,
        align=center,
        minimum height=1.1cm,
        text width=0.245\textwidth,
        inner sep=6pt
      },
      flow/.style={-{Latex[length=2.2mm]}, thick},
      process/.style={font=\small\bfseries, align=center}
    ]
    \node[box] (state) {
      \textbf{Research state}\\[-1mm]
      \footnotesize objectives, claims, evidence, and failures
    };
    \node[box, below left=2.0cm and 0.9cm of state] (action) {
      \textbf{High-level action}\\[-1mm]
      \footnotesize the direction or mode of inquiry to pursue next
    };
    \node[box, below right=2.0cm and 0.9cm of state] (results) {
      \textbf{Results}\\[-1mm]
      \footnotesize proofs, computations, counterexamples, or informative failures
    };

    \draw[flow] (state) -- node[process, midway, left=14pt] {
      Research\\judgement
    } (action);
    \draw[flow] (action) -- node[process, midway, below=5pt] {
      Technical execution
    } (results);
    \draw[flow] (results) -- node[process, midway, right=14pt] {
      Research-state\\representation
    } (state);
  \end{tikzpicture}
  \caption{A simplified research cycle modelling the process of long-horizon
  mathematical research. The decomposition is intended as a systems-level
  description.}
  \label{fig:research-cycle}
\end{figure}

The components of this research cycle have familiar precedents. Newell and Simon model problem
solving as the application of operators to states in a problem
space~\cite{newell1972human}; P\'olya separates understanding and planning
from execution and looking back~\cite{polya1957solve}; Schoenfeld emphasizes
\emph{control}, the executive decisions that select and monitor mathematical
strategies~\cite{schoenfeld1983episodes,schoenfeld1985mathematical}; and
Sch\"on describes professional inquiry as a reflective conversation in which
action changes the situation and may require it to be reframed
~\cite{schon1983reflective}. Figure~\ref{fig:research-cycle} is a minimal synthesis of these ideas, adapted to the architecture of the harness.

\subsection{Performance across research functionalities}

The system consistently exhibited an asymmetry in its capabilities between its local and global functionalities. It was exceptionally strong at
technical execution, and substantially less reliable at research judgement and research-state representation, the two functionalities that operate over the research program as a whole.

\paragraph{(1) Technical execution: strong.}
Once a sufficiently well-specified high-level action was fixed, the system was
usually effective at thinking creatively and devising the mathematics and computations necessary to advancing the action. It drew upon its vast range of
mathematical knowledge and problem-solving skills to develop lemmas and proofs, and it also effectively ran and interpreted experiments. A prominent example of this was how the system found and developed the current lower bound, as detailed in the case study. After the upper-bound failures were reframed as evidence for a
universal obstruction, the system developed the central proof of the lower
bound with comparatively little further intervention. This required a lengthy argument with many intermediate results, involving creative application of areas such as Gaussian harmonic analysis, geometric and functional inequalities, variational arguments, and finite-dimensional optimization. 


\paragraph{(2) Research judgement: limited autonomy.}
Long-horizon research requires repeated decisions about what the program
should do next~\cite{tao2007good,thurston1994proof}. These decisions combine mathematical valuation --- the
expected significance, generality, explanatory value, and downstream use of
a result --- with estimates of difficulty, probability of success, information
gained from failure, verification cost, and opportunity cost.
% Mathematical value is itself multidimensional, rather than reducible to the numerical strength of a bound~\cite{tao2007good,thurston1994proof}.

The system did not reliably make these decisions at the program level. The initial
upper-bound search in the case study is a clear example: several distinct approaches had
failed for the same structural reason, yet the run opened another variation
rather than asking whether the common obstruction was universal, and could be proven as a theorem. Other failings of the system included not recognizing the value of a theoretical result over numerical evidence, and prioritizing a sharper restricted result that is not inherently interesting over a general result. The relevant limitation was not an inability to perform the required
reasoning. Once prompted to step back, synthesize, or reframe, the system
often did so effectively. It was the failure to recognize, from the evolving
state of the project, when such a change in reasoning mode was called for.
This resembles the distinction made by Mason and Spence~\cite{mason1999beyond} between possessing a strategy and
\emph{knowing to} activate it in the appropriate situation. 
% In the terminology of AI, it is also a form of metareasoning: selecting which computations or lines of inquiry are worth performing under limited resources~\cite{russell1991metareasoning}.




\paragraph{(3) Research-state representation: fragile.}


This functionality became more difficult as the run grew. The project produced
far more intermediate mathematics than could be placed in a model's context
at once, so the harness maintained an archive of transcripts and experiments
together with a much smaller curated summary, rewritten at every merge, that
each new session read as its working memory. The withdrawn upper bound in session 44 (see Table~\ref{tab:timeline}) is a
clear case of failure. A fast numerical evaluator built in session~4 carried
an explicit caveat that its score was safe only for exploration; the caveat
did not survive later representations of the research state, and by
session~44 the uncertified score had set the record.
A feasibility criterion that would have invalidated the record was lost even earlier: the run proved it in session~8, but it disappeared in a later handoff and was eventually reproved from scratch by the audit that withdrew the record 25 days later.
In both failures, the archive retained the original facts; it was the compressed state governing decisions that
failed.


% This function became more difficult as the run grew. The project produced
% far more intermediate mathematics than could be placed in a model's context
% at once, so the harness maintained an archive of transcripts and experiments
% together with a much smaller curated summary that each new session read as
% its working memory. The withdrawn upper bound is a clear case of failure. A
% fast numerical evaluator built in session~4 carried an explicit caveat that
% its score was safe only for exploration; the caveat did not survive later
% representations of the research state, and by session~44 the uncertified
% score had set the record. A feasibility criterion that would have
% invalidated the record fared worse: it was proven by the run in session~8 and lost in a handoff, and was subsequently reproven from scratch by the
% audit that withdrew the record twenty-five days later.

% Two features make this function difficult. First, deciding what to keep
% requires the same research judgement whose limits we have just described:
% which details matter depends on decisions not yet taken. Second, the active
% state was rewritten roughly two hundred times over the run, and iterated
% rewriting acts as a transmission chain: headline values survive retelling
% more reliably than their evidential status, scope, and caveats, a bias
% documented in both human and language-model
% retelling~\cite{bartlett1932remembering,acerbi2023transmission,mohamed2025broken}.
% The archive retained the original caveats throughout; it was the compressed
% state governing decisions that failed. More context alone is unlikely to
% solve the problem, as language models do not use all positions in long contexts
% equally reliably~\cite{liu2024lost,hsieh2024ruler}.
% and an unstructured
% archive does not by itself determine which information should govern the
% next decision. We return to this in Section~\ref{sec:ai-future}.






% The archive retained the
% original caveats, 
% but repeated compression preserved the headline value more
% reliably than its evidential status and assumptions. The active state thus
% came to represent a conditional numerical observation as an established
% result. This is better described as a failure of research-state management
% than as ordinary forgetting: the system needed to preserve not only claims,
% but also their provenance, dependencies, scope, counterevidence, and current
% status. More context alone is unlikely to solve the problem. Language models
% do not use all positions in long contexts equally reliably
% ~\cite{liu2024lost}, and an unstructured archive does not by itself determine
% which information should govern the next decision.

% The classical AI literature on truth maintenance is directly relevant here.
% Truth-maintenance systems record why a belief is held and revise dependent
% beliefs when a justification fails~\cite{doyle1979truth,dekleer1986atms}; the
% data-provenance literature similarly represents where a result came from and
% how it was derived~\cite{buneman2001why}. A research state for this setting
% would ideally combine these ideas with retrieval: claims would be stored as
% structured objects carrying their status, assumptions, evidence,
% dependencies, counterevidence, and revision history, while the active context
% would contain only the portion relevant to the current action.

\subsection{Origins of the capability profile}
\label{sec:ai-origins}

We hypothesize the following explanation for the AI system's performance in each of these functionalities. There is a plausible asymmetry in both the training data and feedback received by the base model, where it has a lot more experience with local, technical execution over global, long-horizon reasoning and planning. Mathematical papers, textbooks, and solved problems provide many
examples of technical execution where definitions are used and results are proven. Moreover, AI models can be trained effectively on problems where the final answer or proof can be scored automatically~\cite{shao2024deepseekmath,hubert2026alphaproof}, which roughly corresponds to the skills required for strong technical execution we see in the run.


The training data and feedback available for research judgement is much rarer. Finished
mathematical papers rarely record the full process of discovery, including the abandoned approaches, the experiments performed, and decisions to pivot directions. Instead, they represent a polished final state, written for expositional clarity, rigor, and brevity. Lakatos's contrast between deductive exposition and the process of proofs,
criticism, and revision makes this explicit~\cite{lakatos1976proofs}; Thurston likewise argues that mathematical progress
and understanding are not captured by formal proofs alone~\cite{thurston1994proof}. Moreover, it is computationally much more difficult to run long-horizon mathematical research projects in the same training environments as the more elementary mathematical problems AI models are trained on. The reward design for this would also be more difficult, as reward signals are very sparse and success can be open-ended.

The weakness in research-state representation fits the same asymmetry.
Curation is a global functionality: deciding what the program will later need to
know is a prediction about its future, of the same kind as the judgements
above. The record that would teach the model this prediction (what was kept, what was dropped,
and which omission later mattered) is what finished exposition
omits. The hypothesis also predicts the direction of the failure we
observed. The active state was rewritten roughly two hundred times over the
run, and each rewrite draws on a training genre, the finished mathematical paper, that
states results and omits caveats, scope, and doubt. Therefore, iterated rewriting regresses toward that genre, and headline values survive retelling
more reliably than their evidential status, a bias documented in both human
and language-model
retelling~\cite{bartlett1932remembering,acerbi2023transmission,mohamed2025broken}.
The corpus records mathematics as product rather than process, and both
global functionalities need the process view.

% On the other hand, it is possible that a different representation of the state can significantly improve the performance here.

\subsection{Human collaboration}

The decomposition is also instructive in classifying the human contribution in the run, which entered in three areas. First, the operators supplied the initial
research state, including the cubic--quintic framework and its certification
machinery, and a problem statement with candidate directions for both
bounds (Section~\ref{sec:ai-methodology}). Second, through about forty directives, they supplied
program-level research judgement: selecting and redirecting the
high-level action (the lower bound pivot of Section~\ref{sec:ai-case-study} is the
crucial instance) and fixing priorities such as generality over
numerical sharpness. Third, they
intervened in research-state representation, continuously changing the structure of the research-state representation, and changing the guidelines for what information to store and how. The technical execution was left almost entirely
to the system.

This contribution is itself mathematically significant. Recognizing when to switch to another approach, or when a common obstruction might be able to be generalized to a useful theorem are instances of the higher-level, largely intuitive
judgement that mathematicians acquire with
experience~\cite{tao2007good,thurston1994proof}.
The same holds for research-state representation: deciding which information may matter to future directions requires foresight and experience with mathematical research.


\subsection{Relation to recent work}

Recent successes of AI in mathematics, including on open problems, vary
in method and in the role of the human. Evaluator-guided search has
produced record constructions on problems whose candidate solutions can
be scored
automatically~\cite{funsearch,novikov2025alphaevolvecodingagentscientific,charton2024patternboostconstructionsmathematicslittle},
and formal provers have reached medal-level performance on olympiad
problems~\cite{hubert2026alphaproof}. Frontier reasoning models have
resolved open questions with varying degrees of human involvement: an
internal OpenAI model disproved the Erd\H{o}s unit-distance
conjecture~\cite{openai2026planarpointsets}, a mathematician working with
Claude Fable~5 found a counterexample to the Jacobian
conjecture~\cite{jacobian}, and OpenAI has announced solutions to ten
open problems~\cite{openai2026ten}.


To the best of our knowledge, this work is the first in-depth case study of a long-horizon human--AI collaboration on a mathematical research program:
% The work reported here is, to the best of our knowledge, the first
% sustained human--AI collaboration on a mathematical research program:
over several weeks, we accumulated intermediate results, explored and shelved various directions, and steered at the program level (Section~\ref{sec:ai-methodology}).
We expect this collaborative mode, rather than
full autonomy,
to be the likeliest source of strongest results and thus the prevailing near-term form of AI-assisted mathematics:
% to be both the prevailing near-term form of AI-assisted mathematics and the likeliest source of its strongest results:
% reasoning models are already entering mathematicians' working practice~\cite{bubeck2025science}, while the weaknesses documented in this section leave current systems some distance from carrying a research program alone.
reasoning models are already entering mathematicians' working practice~\cite{bubeck2025science}, but the weaknesses we document show the current limitations of full autonomy.
This report is thus a useful case study of a successful human--AI collaboration in mathematics.

% We hope the experience recorded here proves useful to mathematicians and AI researchers pursuing such collaborations research.

\subsection{Future directions}
Our analysis suggests two complementary directions. For AI research, improving research judgement and research-state representation may require training and evaluation on records of mathematics as a process, including failed approaches, strategic decisions, and evolving assessments of evidence. For mathematical practice, while these limitations persist, human expertise is likely to remain most valuable in these global functionalities: deciding when to persist or reframe a direction, and maintaining an accurate representation of accumulated progress.





% \section{Future directions}
% \label{sec:ai-future}

% We see two directions: for AI research, addressing the weaknesses
% documented in Section~\ref{sec:ai-discussion}; for mathematical practice,
% accounting for them while they persist.




% \paragraph{For AI research.}
% On the hypothesis of Section~\ref{sec:ai-origins}, what the two global
% functions (research judgement and research-state representation) lack is training data that records research as a process.
% Collaborative research programs between humans and AI produce such data as a byproduct, as every human intervention is a labelled instance of when the human's research judgement differed from the AI system, given the state. We hope our work and experience serves as a starting point, for 
% Comparable records across problems, systems, and research
% groups would test whether the capability profile we observed is general.


% \paragraph{For mathematical practice.}
% With the current capabilities of AI, mathematicians working with AI systems should plan to use their expertise to perform
% the global functions themselves. In particular, mathematicians should be aware of these AI systems' tendency to persist on an approach rather than reframing the goal, and to inaccurately summarize previous progress in long-context situations.


% We see two complementary directions: for AI research, addressing the
% weaknesses documented in Section~\ref{sec:ai-discussion}; for mathematical
% practice, accounting for them while they persist.

% \paragraph{For AI research.}
% The two unreliable global functions are concrete targets. For research
% judgement, an evaluation could present a partially developed research
% program, with its accumulated claims and failures, and score the choice of
% the next high-level action rather than the final answer. For research-state
% representation, the target is a representation under which a claim's
% evidential status, assumptions, and caveats survive repeated compression as
% reliably as its headline value.

% Both directions need the same raw material: records of research as it
% happened, retaining the failed approaches, the decisions taken, and the
% reasons for them. Collaborative runs produce such records as a byproduct.
% Each of the about forty directives in ours is an instance of research
% judgement, captured at the decision point together with the project state
% that prompted it, and the amount of steering a run requires is itself a
% measure of the reliability of these functions. Beyond the record released
% with this work, comparable records across problems, systems, and research
% groups would test whether the capability profile we observed is general,
% and would begin to supply the process data that, on the hypothesis of
% Section~\ref{sec:ai-origins}, these functions currently lack.

% \paragraph{For mathematical practice.}
% In the near term, mathematicians working with such systems should plan to
% supply the global functions themselves, and our record indicates where.
% Judgement is needed at the moments the system does not reliably flag: when
% repeated failures call for synthesis into a common obstruction, and when a
% general mechanism is worth more than a sharper number. The system's summary
% of its own progress needs periodic auditing against the primary record,
% since caveats and evidential status erode under repeated summarization, as
% with the withdrawn upper bound.

% Independent verification remains the final safeguard, and in our run it was
% the bottleneck: the system produced results faster than we have been able
% to verify them, which is why the improved bounds of
% Section~\ref{sec:ai-results} are reported as machine-verified claims rather
% than as theorems. A natural remedy is formal verification. Had the system
% delivered its results as formal proofs in a proof assistant, human checking
% would reduce to auditing the formal statements, and the distinction this
% paper maintains between machine-verified claims and theorems would largely
% collapse.


==> paper/conclusion.tex <==
\section{Conclusion}

==> paper/discussion_future_directions.tex <==
\section{Discussion and Future Directions}
\label{sec:discussion}

This section explains the parameter choices, nearby extensions, and finite-dimensional effectiveness questions.

\subsection{Why degrees three and five}

The low-order inverse relations \eqref{eq:low-inverse} explain the parameter search.  The hyperplane scheme has $H(t)=\arcsin t$, so its inverse $\sin\zeta$ has alternating nonlinear coefficients.  To increase the admissible radius, the first objective is to suppress the cubic inverse obstruction.  An anti-aligned third-chaos average changes $b_3$ in the correct direction.  Once $b_3$ is controlled, the next obstruction is quintic, and an aligned fifth-chaos average gives the next degree of freedom.

The small two-dimensional perturbation $\eta \He_3(X)$ in the base threshold is also important.  A threshold depending only on the linear combination $Z+\sum_ds_dR_d$ would reduce to a hyperplane after rotation.  The $X$-dependent cubic term changes the coefficient integrals $\mathsf A_{a,b}$ and gives the higher coefficients the needed shape.

\subsection{A degree \texorpdfstring{$7/9$}{7/9} extension}

The coefficient formula immediately extends to additional odd degrees.  For instance, taking
\[
  D=\{3,5,7,9\},
  \qquad
  \sigma_d=(-1)^{(d-1)/2},
\]
keeps the same formula \eqref{eq:general-bm}.  A preliminary numerical search gives
\begin{align*}
  \eta&=0.12569605,&
  s_3&=0.34199778,&
  s_5&=0.05153822,\\
  s_7&=0.00698313,&
  s_9&=0.00090252.
\end{align*}
For the corresponding limiting model, the estimated value is
\[
  \gamma\approx0.88157525281,
  \qquad
  \KG\lesssim1.78180628572.
\]
This extension is not used in the main theorem.  It is included to indicate that the third/fifth scheme is not isolated: the same analytic and finite-transfer machinery applies to a broader family of Gaussianized Hermite-chaos averages.

\subsection{Effective dimensions}

Corollary~\ref{cor:finite-scheme} is qualitative: it proves the existence of sufficiently large finite length $N$, but it does not give a useful dimension bound.  For the Grothendieck constant as a mathematical constant, qualitative existence of a finite scheme is enough.  For an explicit algorithmic implementation, one should quantify the convergence $H_N\to H$ on the contour used in Theorem~\ref{thm:finite-transfer}.

The natural route is a collision expansion, by which we mean an expansion separating terms with distinct indices from terms in which some indices repeat.  For fixed degree $d$ and fixed $k$, the polynomial $\He_k(P_{d,N})$ has a leading distinct-index component
\[
  \sqrt{k!}\,N^{-k/2}
  \sum_{1\le i_1<\cdots<i_k\le N}
  \He_d(U_{d,i_1})\cdots \He_d(U_{d,i_k}),
\]
which is homogeneous of total Hermite degree $dk$ and has $L^2$-norm squared $(N)_k/N^k\to1$.  The remaining collision terms have vanishing $L^2$ mass for fixed $d,k$.  This explains at the coefficient level why a limiting Hermite mode of order $k$ contributes correlation power $t^{dk}$.  Making this expansion uniform to the required degree would produce explicit finite-dimensional estimates.


==> paper/finite_dim_realization.tex <==
\section{Finite-Dimensional Realization}
\label{sec:transfer}

This section is proves that finite schemes approximate the limiting $b$-series.  Coefficientwise convergence is true, but it is not strong enough to transfer the inverse-majorant condition, which is an infinite nonlinear condition on the inverse series.  We prove a stronger analytic statement.

\subsection{Locally uniform convergence of finite correlations}

Let $H_N$ denote the arcsine-normalized correlation function of the finite scheme $(f_N,g_N)$, in the standard-normal coordinates of Section~\ref{sec:scheme}:
\[
  H_N(t)={\pi\over2}\E[f_N(\calX)g_N(\calY_t)].
\]
Here $\calX,\calY_t\in\R^{2+|D|N}$ are standard Gaussian vectors with $\E[\calX_i\calY_{t,i}]=t$ coordinatewise.

\begin{proposition}[Local uniform convergence]\label{prop:loc-unif}
The functions $H_N$ extend holomorphically to $\D$, satisfy $|H_N(z)|\le\pi/2$ on $\D$, and converge locally uniformly on $\D$ to the limiting correlation $H$.  Consequently, if
\[
  H_N(z)=\sum_{m\ge1}b_{m,N}z^m,
  \qquad
  H(z)=\sum_{m\ge1}b_mz^m,
\]
then $b_{m,N}\to b_m$ for every fixed $m$.
\end{proposition}

\begin{proof}
For fixed $N$, expand $f_N$ and $g_N$ in the orthonormal tensor Hermite basis on $\R^{2+|D|N}$:
\[
  f_N=\sum_\alpha \widehat f_N(\alpha)\He_\alpha,
  \qquad
  g_N=\sum_\alpha \widehat g_N(\alpha)\He_\alpha.
\]
Mehler's formula gives, for real $t\in(-1,1)$,
\[
  {2\over\pi}H_N(t)=\sum_\alpha \widehat f_N(\alpha)\widehat g_N(\alpha)t^{|\alpha|}.
\]
The same series is absolutely convergent for $|z|<1$, since Cauchy-Schwarz gives
\begin{align*}
  \sum_\alpha |\widehat f_N(\alpha)\widehat g_N(\alpha)| |z|^{|\alpha|}
  &\le
  \left(\sum_\alpha |\widehat f_N(\alpha)|^2 |z|^{|\alpha|}\right)^{1/2}
  \left(\sum_\alpha |\widehat g_N(\alpha)|^2 |z|^{|\alpha|}\right)^{1/2}\\
  &\le \|f_N\|_2\|g_N\|_2=1.
\end{align*}
Thus $H_N$ is holomorphic on $\D$ and $|H_N(z)|\le \pi/2$.

We next identify the pointwise limit on the real interval.  Fix $t\in(-1,1)$.  For every degree $d\in D$, the Hermite covariance identity gives
\[
  \E[\He_d(U_{d,j})\He_d(U_{d,j}')]=t^d.
\]
The multivariate central limit theorem yields
\[
  \bigl(P_{d,N},P_{d,N}'\bigr)_{d\in D}
  \Rightarrow
  \bigl(R_d,R_d'\bigr)_{d\in D},
\]
where $(R_d,R_d')$ is a Gaussian pair with correlation $t^d$, and the pairs are independent over distinct $d$.  This convergence is joint with $(Z,Z',X,X')$, which are independent of the Hermite averages.

The limiting discontinuity set of the product of signs is contained in the union of the two threshold hypersurfaces
\begin{align*}
  z+\eta \He_3(x)+\sum_{d\in D}s_dr_d&=0,\\
  z'-\eta \He_3(x')+\sum_{d\in D}\sigma_ds_dr_d'&=0.
\end{align*}
This union has limiting probability zero: after conditioning on all variables except $Z$, the first threshold has probability zero because $Z$ has a density, and similarly for the second threshold using $Z'$.  The bounded continuous mapping theorem therefore gives $H_N(t)\to H(t)$ for every real $t\in(-1,1)$.

The family $\{H_N\}$ is locally bounded on $\D$ and converges pointwise on a set with an accumulation point.  Vitali's theorem gives locally uniform convergence on $\D$ to the unique holomorphic function agreeing with the real limiting correlation.  Coefficient convergence follows from Cauchy's formula.
\end{proof}

\begin{remark}
Proposition~\ref{prop:loc-unif} justifies the limiting coefficient formula as the fixed-degree limit of genuine finite-dimensional schemes.  But it does not by itself imply that the finite inverse series satisfy $\sum_n|A_{n,N}|\gamma^n\le1$.  Tail control for the inverse series requires the inverse-branch stability theorem below.
\end{remark}

\subsection{Analytic stability of inverse branches}

\begin{theorem}[Finite inverse-majorant transfer]\label{thm:finite-transfer}
Let $F_N,F\in\Hol(\D)$, assume $F_N\to F$ locally uniformly on $\D$, and assume $F_N(0)=F(0)=0$.  Suppose that $G$ is a holomorphic inverse branch of $F$ on a neighborhood of $\ol{D(0,R_0)}$, with values in $\D$:
\[
  F(G(\zeta))=\zeta,
  \qquad |\zeta|\le R_0.
\]
Write
\[
  G(\zeta)=\sum_{n\ge1}A_n\zeta^n.
\]
Let $0<\gamma<R_0$, and assume the strict majorant inequality
\[
  \sum_{n\ge1}|A_n|\gamma^n<1.
\]
Then, for all sufficiently large $N$, $F_N$ has a holomorphic inverse branch at the origin,
\[
  G_N(\zeta)=F_N^{-1}(\zeta)=\sum_{n\ge1}A_{n,N}\zeta^n,
\]
defined on a neighborhood of $\gamma\ol\D$, and
\[
  \sum_{n\ge1}|A_{n,N}|\gamma^n<1.
\]
Moreover $A_{n,N}\to A_n$ for every fixed $n$.
\end{theorem}

\begin{proof}
Choose nested radii
\[
  \gamma<\rho<r<R<R_0.
\]
Let
\[
  \Omega=G(D(0,R)).
\]
Since $G$ is a conformal inverse branch on a neighborhood of $\ol{D(0,R)}$, the boundary $\partial\Omega$ is the image of $|\zeta|=R$.  For $t\in\partial\Omega$, we have $|F(t)|=R$.  Therefore, for all $|\zeta|\le r$,
\[
  |F(t)-\zeta|\ge R-r,
  \qquad t\in\partial\Omega.
\]
The compact contour $\partial\Omega$ is contained in $\D$.  By locally uniform convergence, for all large $N$,
\[
  \sup_{t\in\partial\Omega}|F_N(t)-F(t)|<R-r.
\]
Rouche's theorem then implies that, for every $|\zeta|\le r$, the equations $F_N(t)=\zeta$ and $F(t)=\zeta$ have the same number of solutions in $\Omega$, counted with multiplicity.  The equation $F(t)=\zeta$ has exactly one solution in $\Omega$, namely $t=G(\zeta)$.  Hence $F_N(t)=\zeta$ also has exactly one solution in $\Omega$.  In particular, since $F_N(0)=0$, the zero at $0$ is simple, and these solutions define a holomorphic inverse branch $G_N$ on $D(0,r)$, with values in $\Omega$.

The inverse branches converge uniformly on $\ol{D(0,r)}$.  Indeed, by the argument-principle formula,
\[
  G_N(\zeta)= {1\over 2\pi i}\int_{\partial\Omega}
  {tF_N'(t)\over F_N(t)-\zeta}\,dt,
  \qquad |\zeta|\le r.
\]
The denominators are uniformly bounded away from zero on $\partial\Omega\times\ol{D(0,r)}$, and $F_N'\to F'$ uniformly on $\partial\Omega$.  Thus $G_N\to G$ uniformly on $\ol{D(0,r)}$, which implies fixed inverse-coefficient convergence.

It remains to control the tail.  Put
\[
  B=\sup_{t\in\ol\Omega}|t|<\infty.
\]
Since $G_N(D(0,r))\subseteq\Omega$, Cauchy's estimate on the circle $|\zeta|=\rho$ gives
\[
  |A_{n,N}|\le B\rho^{-n},
  \qquad n\ge1,
\]
for all large $N$.  Let
\[
  \delta=1-\sum_{n\ge1}|A_n|\gamma^n>0.
\]
Choose $M$ so large that
\[
  B\sum_{n>M}\left({\gamma\over\rho}\right)^n< {\delta\over3}.
\]
For all sufficiently large $N$, fixed-coefficient convergence gives
\[
  \sum_{n\le M}|A_{n,N}|\gamma^n
  \le \sum_{n\le M}|A_n|\gamma^n+{\delta\over3}.
\]
Therefore
\begin{align*}
  \sum_{n\ge1}|A_{n,N}|\gamma^n
  &\le \sum_{n\le M}|A_n|\gamma^n+{\delta\over3}
  +B\sum_{n>M}\left({\gamma\over\rho}\right)^n\\
  &< \sum_{n\ge1}|A_n|\gamma^n+{2\delta\over3}<1.
\end{align*}
\end{proof}

\begin{corollary}[Finite schemes from a limiting certificate]\label{cor:finite-scheme}
Assume the limiting correlation $H$ has a holomorphic inverse branch
\[
  G(\zeta)=H^{-1}(\zeta)=\sum_{n\ge1}A_n\zeta^n
\]
with values in $\D$ on a neighborhood of $\ol{D(0,R_0)}$.  Let $0<\gamma<R_0$, and suppose
\[
  \sum_{n\ge1}|A_n|\gamma^n<1.
\]
Then, for all sufficiently large lengths $N$, the genuine finite-dimensional scheme $(f_N,g_N)$ satisfies the inverse-majorant condition at radius $\gamma$.  Consequently
\[
  \KG\le {\pi\over2\gamma}.
\]
\end{corollary}

\begin{proof}
Apply Proposition~\ref{prop:loc-unif} and Theorem~\ref{thm:finite-transfer} with $F_N=H_N$ and $F=H$, then invoke Theorem~\ref{thm:krivine-criterion} for the finite scheme after the scaling convention stated at the start of Section~\ref{sec:scheme}.
\end{proof}

\begin{corollary}[Endpoint and margin]\label{cor:margin}
If the limiting inverse branch is holomorphic with values in $\D$ on a neighborhood of $\Gamma\ol\D$ and
\[
  \sum_{n\ge1}|A_n|\Gamma^n\le1,
\]
then every $\gamma<\Gamma$ transfers to all sufficiently high finite-dimensional schemes.  If the inequality at $\Gamma$ is strict and the same analytic neighborhood is available, then $\Gamma$ itself transfers.
\end{corollary}

\begin{proof}
For $\gamma<\Gamma$, the majorant is strict because $A_1\neq0$:
\[
  \sum_{n\ge1}|A_n|\gamma^n<\sum_{n\ge1}|A_n|\Gamma^n\le1.
\]
Apply Corollary~\ref{cor:finite-scheme}.  The strict endpoint case is the same argument with $\gamma=\Gamma$.
\end{proof}

